Online Anomalous Subtrajectory Detection on Road Networks with Deep Reinforcement Learning

Detecting anomalous trajectories has become an important task in many location-based applications. While many approaches have been proposed for this task, they suffer from various issues including (1) incapability of detecting anomalous subtrajectories, which are finer-grained anomalies in trajectory data, and/or (2) non-data driven, and/or (3) requirement of sufficient supervision labels which are costly to collect. In this paper, we propose a novel reinforcement learning based solution called RL4OASD, which avoids all aforementioned issues of existing approaches. RL4OASD involves two networks, one responsible for learning features of road networks and trajectories and the other responsible for detecting anomalous subtrajectories based on the learned features, and the two networks can be trained iteratively without labeled data. Extensive experiments are conducted on two real datasets, and the results show that our solution can significantly outperform the state-of-the-art methods (with 20-30% improvement) and is efficient for online detection (it takes less than 0.1ms to process each newly generated data point).

==> abstract.tex <==

\begin{abstract}
Detecting anomalous trajectory has become an important concern in many location-based applications. However, most of the existing studies for this problem can only give a vague judgement (e.g., an anomaly score) of whether a given trajectory is anomalous, fail at indicating which part of the trajectory is anomalous, i.e., detecting anomalous \textbf{sub}trajectory. Anomalous subtrajectory detection is very important for real-world applications that can more accurately locate and indicate the anomalousness in a trajectory, yet it is very challenging due to three challenges:
% In real-world applications, trajectories are usually long sequences with many subtrajectories. These methods are unable to accurately locate and measure the anomalousness in a trajectory anomaly, not to mention timely suggest corresponding action against it. 
% , which would be more informative and applicable for real-world location-based services. 
% Nevertheless, the anomalous subtrajectory detection problem is challenging to solve, due to
1) the complexity of subtrajectory modeling, 2) the lack of labeled data, and 3) the efficiency of detection. To tackle these challenges, we propose a novel reinforcement learning based solution, which is able to expressively learn the complexity mobility patterns behind subtrajectories with limited labeled data, and efficiently detect subtrajectory anomalies in an online manner. Extensive experiments are conducted on two real-world trajectory datasets with manually labeled test data, and the results show that our solution can significantly outperform the state-of-the-art methods and is efficient for online detection.

% 1) the variety and complexity of subtrajectory across different places, 2) the efficiency of online detection for a large number of subtrajectories, and 3) the measurement off anomalousness without labeled data.
% To this end,
% we propose a novel model, namely Gaussian Mixture Variational
% Sequence AutoEncoder (GM-VSAE), to tackle these challenges.
% Our GM-VSAE model is able to (1) capture complex sequential
% information enclosed in trajectories, (2) discover different types
% of normal routes from trajectories and represent them in a
% continuous latent space, and (3) support efficient online detection
% via trajectory generation. Our experiments on two real-world
% datasets demonstrate that GM-VSAE is more effective than the
% state-of-the-art baselines and is efficient for online anomalous
% trajectory detection.
\end{abstract}





==> abstract2.tex <==

\begin{abstract}
Detecting anomalous {\Comment{trajectories}} has become an important concern in many location-based applications. Most of the existing studies for this problem only give a vague judgement (e.g., an anomaly score) of whether a given trajectory is anomalous, but are not able to indicate which part of the trajectory is anomalous in a \textbf{timely manner}, i.e., detecting online anomalous \textbf{sub}trajectory. Anomalous subtrajectory detection is important for a number of real-world applications, e.g. for ladies going home late, elderly care, and child custody. The problem is challenging due to three issues:
% In real-world applications, trajectories are usually long sequences with many subtrajectories. These methods are unable to accurately locate and measure the anomalousness in a trajectory anomaly, not to mention timely suggest corresponding action against it. 
% , which would be more informative and applicable for real-world location-based services. 
% Nevertheless, the anomalous subtrajectory detection problem is challenging to solve, due to
1) the lack of labeled data, 2) the complex anomalous subtrajectory modelling,
% how to model anomalous subtrajectories more accurately, 
and 3) the efficiency requirement of online detection. 
To tackle these challenges, we propose a novel reinforcement learning based solution, which is able to expressively learn the characteristics of anomalous subtrajectories without labeled data, and efficiently detect subtrajectory anomalies in an online manner. Extensive experiments are conducted on two real-world trajectory datasets with manually labeled test data, and the results show that our solution can significantly outperform the state-of-the-art methods (with 20-30\% improvement) and is efficient for online detection (it takes less than 0.1ms to process each newly generated data point). \\\vspace{-0.1in}

% 1) the variety and complexity of subtrajectory across different places, 2) the efficiency of online detection for a large number of subtrajectories, and 3) the measurement off anomalousness without labeled data.
% To this end,
% we propose a novel model, namely Gaussian Mixture Variational
% Sequence AutoEncoder (GM-VSAE), to tackle these challenges.
% Our GM-VSAE model is able to (1) capture complex sequential
% information enclosed in trajectories, (2) discover different types
% of normal routes from trajectories and represent them in a
% continuous latent space, and (3) support efficient online detection
% via trajectory generation. Our experiments on two real-world
% datasets demonstrate that GM-VSAE is more effective than the
% state-of-the-art baselines and is efficient for online anomalous
% trajectory detection.
\end{abstract}






==> back_up_experiments.tex <==
\section{EXPERIMENTS}
\label{sec:experiment}
\subsection{Experimental Setup}
\label{sec:setup}
\noindent \textbf{Dataset.}
We collected a real-world billiards layouts dataset, which consists of more than 3000 break shots in around 94 international professional 9-ball games {\Comment played by 227 players. In the dataset, there are around 1200 (resp. 1400) billiards layouts with the label ``clear'' (resp. ``win'').} %The illegal cases of sinking the cue ball into a pocket are removed. 
Each layout contains several positions of balls that remain on the pool table after the break shot, and each position corresponds to $(x,y)$ coordinates captured by a professional sports analysis software Kinovea. We give more details on the dataset as follows.%~\cite{pan2021development}

When we collect data, a perspective grid provided by the software Kinovea is used on the closed surface of the table which is calibrated into a $200 \times 100$ coordinate system. The coordinates generally belong to the $[0, 200]$ range along the x-axis, and the $[0, 100]$ range along the y-axis, with the left bottom corner of the table being $(0,0)$. The information we collect includes the positions of balls that remain on the pool table after the break shot, the number of potted balls after the break shot, a binary tag indicating clear or not (clear if the player who performs the break shot pocketed all balls and thus win the game; unclear otherwise), win or not (in a 9-ball game, win if the player potted ball 9 into the pocket, not win otherwise),
and remarks. Remarks are used to capture some special situations, such as golden break, which means the ball 9 is potted into a pocket in the break shot; a foul shot, which means the shot is not making the first contact with the lowest numbered ball in the layout, and it is regarded as breaking the rule of competition. In addition, we provide the YouTube video link for each layout.
% , which can be found on YouTube. 
%record the source of the layout such as "2019 Men's Diamond Las Vegas Open" and provide video link,  We shall publish the dataset and the codes once the paper is accepted.

\noindent \textbf{Baseline.}
{\Comment To evaluate the effectiveness and efficiency of our BL2Vec, we compare it with the following baselines: %(1) EMD~\cite{rubner2000earth}, (2) Hausdorff~\cite{huttenlocher1993comparing}, (3) DTW~\cite{yi1998efficient}, (4) Frechet~\cite{alt1995computing}, (5) Peer Matching (PM), (6)DeepSets~\cite{zaheer2017deep}, (7) RepSet~\cite{skianis2020rep} and (8) WSSET~\cite{Arsomngern2021self} as discussed in Section~\ref{sec:related}.
}
\\
$\bullet$EMD~\cite{rubner2000earth}. The Earth Mover's Distance (EMD) is based on the idea of a transportation problem that measures the least amount of work needed to transform one set to another. %a well-known measurement for pointsets  Besides, EMD is widely used for various applications such as document classification, image retrieval, etc.
\\
$\bullet$Hausdorff~\cite{huttenlocher1993comparing}. Hausdorff distance is based on the idea of point-matching and computes the largest distance among all the distances from a point in one set to the nearest point in the other set.
\\
$\bullet$DTW~\cite{yi1998efficient} and Frechet~\cite{alt1995computing}. DTW and Frechet are two widely used similarity measurements for 
sequential data.
%trajectory/time series analysis. Specifically, Frechet is
%a metric, namely the distance is symmetric and satisfies the triangle inequality; however, DTW is not a metric, since it does not satisfy the triangle inequality.
%
To apply the measurements to billiards layouts, we model each layout as a sequence of locations, which corresponds to one cue ball followed by several object balls in ascending order of ball numbers.
\\
%{\color{blue}
$\bullet$Peer Matching (PM). {\ICDMComment We adopt a straightforward solution for measuring the similarity between two billiards layouts as the average of the distances between their balls matched based on the numbers}, e.g., ball 1 in one layout is matched to the ball 1 in another layout, and so on.
For those mismatched balls with different numbers, we align them in the ascending order of their numbers and match them accordingly.
%}
\\
$\bullet$DeepSets~\cite{zaheer2017deep}. DeepSets is used to generate pointsets representation in an unsupervised fashion. The main idea of DeepSets is to transform vectors
of points in a set into a new representation of the set. It aggregates the representations of vectors and then passes them to fully-connected layers to get the representation.
\\
$\bullet$RepSet~\cite{skianis2020rep}. RepSet is also used to generate the representations of pointsets. It adapts a bipartite matching idea by computing the correspondences between an input set and some generated hidden sets to get the set representation. Besides, RepSet captures the unordered nature of a set and can generate the same output for all possible permutations of points in the set.
\\
$\bullet$WSSET~\cite{Arsomngern2021self}. {\ICDMComment WSSET achieves the state-of-the-art performance on pointsets embedding}, which is an approximate version of EMD based on the deep metric learning framework and uses the EMD as a metric for inferring the positive and negative pairs. It generates the representations of pointsets, and these generated representations can be used for similarity search, classification tasks, etc.

\noindent \textbf{Parameter Setting.}
We set the cell size to be 15  (with the results of its effect shown later on) and thus we have 98 unique tokens for the BS features. For BP and BB features, we use the setting of $15^\circ$ and 10 for partitioning the angle range and distance range, respectively. {\ICDMComment We tried different settings, the results are similar and thus omitted.}
%
For each feature, we embed it to a 10-dimensional vector, and thus the representation dimension of the ball is $10*(1+4*6+2)=270$ (i.e., $K'=270$). Recall that for each ball, there is one token in the BS feature, four tokens in the BP feature with totally six pockets, and two tokens in the BB feature. {\ICDMComment We use a convolutional layer as $Net(\cdot)$ with 3 output channels. For each, it has 52 filters with varying sizes from $(1,K')$ to $(7,K')$.} Note that larger filters help capture the correlations between the balls. A ReLU function is applied after the convolutional layer and then a global max-pooling layer is employed to generate a 156-dimensional representation of the billiards layout  {\ICDMComment (i.e., $K=3 \times 56 = 156$).} {\Comment Additionally, in the training process, we randomly sample 70\% billiards layouts to generate training tuples and adopt Adam stochastic gradient descent with an initial learning rate of $0.00001$, and the remaining layouts are used for testing.} To avoid overfitting, we employ a L2 regularization term with $\lambda=0.001$ for $Net(\cdot)$. The margin in the triplet loss is set to {\ICDMComment $\delta = 1.0$ based on empirical findings.} {\ICDMComment For generating each $\mathcal{B}_+$ (resp. $\mathcal{B}_-$), we set both the noise rate and the drop rate to 0.2 (resp. 0.3) by default.} For parameters of baselines, we follow their settings in the original papers.

\noindent \textbf{Evaluation Metrics.}
We consider the following three tasks to evaluate the effectiveness.
(1) Similarity search, we report the {\ICDMComment Hitting Ratio for Top-10 ($HR@10$) and Mean Reciprocal Rank ($MRR$).} In particular, for a query billiards layout $\mathcal{B}_q$, if its positive version $\mathcal{B}_+$ is in the top-10 returned billiards layouts, then $HR@10$ is defined as $HR@10 = 1$, otherwise $HR@10 = 0$.
%
$MRR$ is defined as $MRR = \frac{1}{rank}$, where $rank$ denotes the rank of $\mathcal{B}_+$ in the database for its query billiards layout $\mathcal{B}_q$. The average results of $HR@10$ and $MRR$ over all queries are reported in the experiments. A higher $HR@10$ or $MRR$ indicates a better result.
%
(2) Classification, we report the average classification accuracy for the label of ``clear'' and ``not clear''. 
% "clear" or "not clear".
Classification accuracy is a widely used metric in the classification task. A higher accuracy indicates a better result.
%
(3) Clustering, we report two widely used metrics Adjusted Rand Index (ARI) and Adjusted Mutual Information (AMI) for clustering. %{\color{blue} ~\cite{rand1971objective} ~\cite{vinh2010information}
They measure the correlation between the predicted result and the ground truth. The ARI and AMI values lie in the range $[-1, 1]$. For ease of understanding, we normalize the values in the range of $[0,1]$.
%as a percentage value. %{\color{blue}
A higher ARI or AMI indicates a higher correspondence to the ground-truth.%}

\noindent \textbf{Evaluation Platform.}
All the methods are implemented in Python 3.8. The implementation of $BL2Vec$ is based on PyTorch 1.8.0. The experiments are conducted on a server with 10-cores of Intel(R) Core(TM) i9-9820X CPU @ 3.30GHz 64.0GB RAM and one Nvidia GeForce RTX 2080 GPU. {\Comment The datasets and codes can be downloaded via the link~\footnote{https://www.dropbox.com/sh/644aceaolfv4rky/AAAKhpY1yzrbq9-uo4Df3N0Oa?dl=0}.}

\begin{figure*}[h]
% \vspace*{-2mm}
% \hspace{-2mm}
%\hspace*{-.3cm}
\centering
\begin{tabular}{c c c c}
  \begin{minipage}{3.2cm}%5.5
    \includegraphics[width=17.2cm]{figures/legend}
   \end{minipage}
   \\
  \begin{minipage}{4.0cm}%5.5
    \includegraphics[width=4.3cm]{figures/hr_noise}
    \end{minipage}
    &
    \begin{minipage}{4cm}
    \includegraphics[width=4.3cm]{figures/mr_noise}
    \end{minipage}
    &
    \begin{minipage}{4cm}
    \includegraphics[width=4.3cm]{figures/hr_drop}
    \end{minipage}
    &
    \begin{minipage}{4cm}
    \includegraphics[width=4.3cm]{figures/mr_drop}
    \end{minipage}
    \\
    (a) Varying noise rate (HR@10)\hspace{-4mm}
    &
    (b) Varying noise rate (MRR)\hspace{-4mm}
    &
    (c) Varying drop rate (HR@10)\hspace{-4mm}
    &
    (d) Varying drop rate (MRR)\hspace{-4mm}
  % \begin{minipage}{0.43\linewidth}
	% \includegraphics[width=\linewidth]{figures/hr_noise}
  % \end{minipage}
  % &
  % \begin{minipage}{0.43\linewidth}
  %   \includegraphics[width=\linewidth]{figures/mr_noise}
  % \end{minipage}
  % \begin{minipage}{0.43\linewidth}
	% \includegraphics[width=\linewidth]{figures/hr_drop}
  % \end{minipage}
  % &
  % \begin{minipage}{0.43\linewidth}
  %   \includegraphics[width=\linewidth]{figures/mr_drop}
  % \end{minipage}
  % \\
  % (a) Varying noise rate (HR@10)
  % &
  % (b) Varying noise rate (MRR)
  % \\
  % \begin{minipage}{0.43\linewidth}
	% \includegraphics[width=\linewidth]{figures/hr_drop}
  % \end{minipage}
  % &
  % \begin{minipage}{0.43\linewidth}
  %   \includegraphics[width=\linewidth]{figures/mr_drop}
  % \end{minipage}
  % \\
  % (c) Varying drop rate (HR@10)
  % &
  % (d) Varying drop rate (MRR)
\end{tabular}
\vspace{-2mm}
%\setlength{\abovecaptionskip}{1pt}

\caption{Effectiveness evaluation with similarity search.}
\label{fig:effectiveness}
\vspace*{-5mm}
\end{figure*}

\subsection{Experimental Results}
\label{sec:effectiveness}

\begin{table}[]
\centering
\caption {Effectiveness evaluation with classification and clustering.}\label{tab:tasks}
\vspace*{-2mm}
\footnotesize{
\begin{tabular}{c|c|l|l|l|c|lcl}
\hline
\multirow{2}{*}{Tasks} & \multicolumn{4}{c|}{Classification} & \multicolumn{4}{c}{Clustring}                     \\ \cline{2-9}
                       & \multicolumn{4}{c|}{Accuracy (\%)}       & \multicolumn{2}{c}{ARI (\%)} & \multicolumn{2}{c}{AMI (\%)} \\ \hline
EMD                    & \multicolumn{4}{c|}{66.33}               & \multicolumn{2}{c}{52.15}    & \multicolumn{2}{c}{55.81}    \\
Hausdorff              & \multicolumn{4}{c|}{59.17}               & \multicolumn{2}{c}{51.68}    & \multicolumn{2}{c}{54.98}    \\
DTW                    & \multicolumn{4}{c|}{59.33}               & \multicolumn{2}{c}{50.12}    & \multicolumn{2}{c}{50.13}    \\
Frechet                & \multicolumn{4}{c|}{59.16}               & \multicolumn{2}{c}{50.16}    & \multicolumn{2}{c}{50.22}    \\
PM                        & \multicolumn{4}{c|}{54.24}               & \multicolumn{2}{c}{50.02}    & \multicolumn{2}{c}{50.32}    \\
DeepSets               & \multicolumn{4}{c|}{54.23}               & \multicolumn{2}{c}{49.50}    & \multicolumn{2}{c}{50.41}    \\
RepSet                 & \multicolumn{4}{c|}{58.99}               & \multicolumn{2}{c}{50.54}    & \multicolumn{2}{c}{50.72}    \\
WSSET                  & \multicolumn{4}{c|}{56.62}               & \multicolumn{2}{c}{49.12}    & \multicolumn{2}{c}{49.78}    \\
BL2Vec                 & \multicolumn{4}{c|}{\textbf{72.62}}               & \multicolumn{2}{c}{\textbf{61.94}}    & \multicolumn{2}{c}{\textbf{63.26}}    \\ \hline
\end{tabular}}
\vspace*{-6mm}
\end{table}
\noindent \textbf{(1) Effectiveness evaluation (similarity search).}
The lack of ground truth makes it a challenging problem to evaluate the similarity. To overcome this problem, we follow recent studies~\cite{Arsomngern2021self} which propose to use the $HR@10$ and $MRR$ to quantify the similarity evaluation via self-similarity comparison. Specifically, we randomly select 100 billiards layouts to form the query set (denoted as $Q$) and 500 billiards layouts as the target database (denoted as $D$), For each billiards layout $ \mathcal{B}_q \in Q$, we create its positive version denoted as $\mathcal{B}_+$ by introducing two types of noises. As discussed in Section~\ref{subsec:sample}, (1) we shift each ball along a random direction by a random distance, which is controlled by a noise rate; (2) we randomly delete some balls controlled by a drop rate and then add them at random locations. Then for each $\mathcal{B}_q$, we compute the rank of $\mathcal{B}_+$ in the database $D \cup \mathcal{B}_+$ using BL2Vec and other baselines. Ideally, $\mathcal{B}_+$ should be ranked at the top since $\mathcal{B}_+$ is generated from the $\mathcal{B}_q$.

Figure \ref{fig:effectiveness} (a) and (b) show the results of varying the noise rate from 0.2 to 0.4 when the drop rate is fixed to 0.2 in terms of
$HR@10$ and $MRR$. We can see that $BL2Vec$ is significantly better than the baselines in terms of $HR@10$ and $MRR$. For example, when applying 40\% noise, BL2Vec outperforms RepSet and DTW (the two best baselines) by 1.5 times and 4.7 times in terms of $HR@10$, respectively, and by more than 6.2 times and 13.3 times in terms of $MRR$, respectively. EMD and DeepSets perform the worst in most of the cases because EMD is based on the idea of point-matching and affected significantly by the noise;
DeepSets is developed for a set that has an unordered nature and therefore it is not suitable for measuring the similarity among billiards layouts, which are order sensitive. %In addition, compared with baselines, our BL2Vec is more robust to noise. For example, when the noise rate increases from 0.2 to 0.4, the $HR@10$ of BL2Vec only decreases by 15\%, while the values of DTW decrease by 80\%.
Figure \ref{fig:effectiveness} (c) and (d) show the results of varying the drop rate from 0.2 to 0.4 when the noise rate is fixed to 0.2 in terms of
$HR@10$ and $MRR$. BL2Vec still performs the best in terms of both metrics. For example, it outperforms RepSet, which performs best in baselines when the drop rate is 0.4, by more than 1.8 times (resp. 9.6 times) in terms of $HR@10$ (resp. $MRR$). %We also note that the performance of BL2Vec gets worse with a larger drop rate. This is because the drop rate may change the form of their relative locations, which affects the similarity.

\noindent \textbf{(2) Effectiveness evaluation (classification).}
Table \ref{tab:tasks} shows the results of different methods in the classification task for predicting the labels of ``clear" and ``not clear". Recall that ``clear" means the player who performs the break shot pocketed all balls and thus win the game, and ``not clear" means the otherwise case.
%
We train a k-nearest neighbour classifier (kNN) with $k = 10$ for this task and report the average accuracy on 500 billiards layouts. For BL2Vec, we fix the noise rate and drop rate to be 0.2 by default, and use the representations of billiards layouts for computing the distance in the KNN classifier, we do the same for DeepSets, RepSet and WSSET. For EMD, Hausdorff, DTW, Frechet and PM, we use their distances for the KNN classifier directly.
We observe BL2Vec outperforms all the baselines. For example, it outperforms EMD (the best baseline) by 9.5\%. The result indicates that the representation learned from BL2Vec is more useful for learning the target task.

\noindent \textbf{(3) Effectiveness evaluation (clustering).}
We further show the clustering task, which is to group billiards layouts belonging to the same family (i.e., ``clear" or ``not clear") into the same cluster. We use the K-means algorithm with $k = 2$ and report ARI and AMI on the
500 billiards layouts. The results are shown in Table~\ref{tab:tasks}. According to the results, BL2Vec also performs best.
For example, it outperforms EMD (the best baseline) by 18.8\% (resp. 13.3\%) in terms of ARI (resp. AMI). In addition, we observe other baselines have similar ARI and AMI, e.g., the values are between 49\% and 50\%. Similar to the classification task, the results indicate adopting the embeddings of BL2Vec for billiards layout clustering will yield superior performance.

\begin{table}[]
\centering
\caption {The effect of the cell size.}\label{tab:parameter}
\vspace*{-2mm}
\centering
\footnotesize{
\begin{tabular}{c|c|cc|c|l|l|l|c|lcl}
\hline
\multirow{2}{*}{Cell size} & \multirow{2}{*}{\#tokens} & \multicolumn{2}{c|}{Similarity} & \multicolumn{4}{c|}{Classification} & \multicolumn{4}{c}{Clustring}                     \\ \cline{3-12}
                           &                           & HR@10           & MRR           & \multicolumn{4}{c|}{Accuracy (\%)}       & \multicolumn{2}{c}{ARI (\%)} & \multicolumn{2}{c}{AMI (\%)} \\ \hline
10                         &    200                    &  0.92         & 0.240              & \multicolumn{4}{c|}{66.67}               & \multicolumn{2}{c}{52.25}    & \multicolumn{2}{c}{55.80}    \\
15                         &    98                     &  0.94         & 0.252         & \multicolumn{4}{c|}{\textbf{72.62}}               & \multicolumn{2}{c}{\textbf{61.94}}    & \multicolumn{2}{c}{\textbf{63.26}}    \\
20                         &    50                     & 0.95          &0.259          & \multicolumn{4}{c|}{67.33}               & \multicolumn{2}{c}{56.96}    & \multicolumn{2}{c}{58.25}    \\
25                         &    32                     &  0.96          &0.303              & \multicolumn{4}{c|}{70.14}               & \multicolumn{2}{c}{55.21}    & \multicolumn{2}{c}{57.37}    \\
30                         &    28                     &  \textbf{0.96}          &\textbf{0.306}            & \multicolumn{4}{c|}{68.72}               & \multicolumn{2}{c}{53.96}    & \multicolumn{2}{c}{56.28}    \\ \hline

\end{tabular}}
\vspace*{-6mm}
\end{table}

\noindent \textbf{(4) Effectiveness evaluation (parameter study).}
\label{sec:parameter}
We next evaluate the effect of the cell size on the effectiveness of similarity search, classification and clustering for BL2Vec.
Intuitively with the smaller cell size, it generates more tokens and provides a higher resolution of the pool table. However, with the smaller size, it reduces the robustness against the noise for the similarity search task. In Table \ref{tab:parameter}, we report the performance for the similarity search, classification and clustering. We notice that the performance of the similarity search becomes better as the cell size grows and this is in line with our intuition. In addition, we observe the smallest cell size of 10 leads to the worst performance, especially for classification and clustering, because the smallest cell size produces more tokens, which makes the model more difficult to train. In our experiments, we set the cell size to 15 because it provides better performance in general.

\begin{table}[]
\centering
\caption {Effectiveness evaluation with ablation study.}\label{tab:ablation}
\vspace*{-2mm}
\footnotesize{
\begin{tabular}{c|cc|c|l|l|l|c|lcl}
\hline
\multirow{2}{*}{Model} & \multicolumn{2}{c|}{Similarity} & \multicolumn{4}{c|}{Classification} & \multicolumn{4}{c}{Clustering}                     \\ \cline{2-11}
                       & HR@10           & MRR           & \multicolumn{4}{c|}{Accuracy (\%)}       & \multicolumn{2}{c}{ARI (\%)} & \multicolumn{2}{c}{AMI (\%)} \\ \hline
BL2Vec                 & \textbf{0.94}            & \textbf{0.252}              & \multicolumn{4}{c|}{\textbf{72.62}}               & \multicolumn{2}{c}{\textbf{61.94}}    & \multicolumn{2}{c}{\textbf{63.26}}    \\
w/o BS                 & 0.92            & 0.207              & \multicolumn{4}{c|}{62.42}               & \multicolumn{2}{c}{53.50}    & \multicolumn{2}{c}{59.25}    \\
w/o BP                 & 0.11            & 0.009              & \multicolumn{4}{c|}{51.08}               & \multicolumn{2}{c}{49.27}    & \multicolumn{2}{c}{50.18}    \\
w/o BB                 & 0.91            & 0.197              & \multicolumn{4}{c|}{69.52}               & \multicolumn{2}{c}{52.45}    & \multicolumn{2}{c}{61.73}    \\ 
w/o $Net(\cdot)$       &  0.40          & 0.078             & \multicolumn{4}{c|}{41.76}               & \multicolumn{2}{c}{50.38}    & \multicolumn{2}{c}{50.67}   \\ \hline
\end{tabular}}
%\vspace*{-2mm}
\end{table}

\begin{figure}
\begin{tabular}{c c}
\begin{minipage}{0.4\linewidth}
\centering
\includegraphics[width=\linewidth]{figures/running_time}
%\setlength{\abovecaptionskip}{1pt}
\vspace*{-5mm}
\caption{Scalability.}
\label{fig:efficiency}
\end{minipage}
&
\begin{minipage}{0.47\linewidth}
\centering
\includegraphics[width=\linewidth]{figures/user_study}
%\setlength{\abovecaptionskip}{0pt}
\vspace*{-5mm}
\caption{User study.}
\label{fig:userstudy}
\end{minipage}
\end{tabular}
\vspace*{-6mm}
\end{figure}


%\begin{figure}
%%\hspace*{-.3cm}
%\centering
%\begin{tabular}{c c}
%  \begin{minipage}{0.99\linewidth}
%	\includegraphics[width=\linewidth]{figures/running_time}
%  \end{minipage}
%\end{tabular}
%%\vspace{-2mm}
%%\setlength{\abovecaptionskip}{1pt}
%\caption{Efficiency evaluation.}
%\label{fig:efficiency}
%\end{figure}
\noindent \textbf{(5) Effectiveness evaluation (ablation study).}
\label{sec:ablation}
To show the importance of each component of the extracted features in our BL2Vec model, including Ball-self (BS), Ball-Pocket (BP) and Ball-Ball (BB), and {\ICDMComment the ability of CNN for capturing spatial features in $Net(\cdot)$}, we conduct an ablation experiment. We denote our BL2Vec model without BS, BP, BB and as w/o BS, w/o BP, w/o BB {\ICDMComment and w/o $Net(\cdot)$, respectively.} Table~\ref{tab:ablation} compares the different versions for similarity search, classification and clustering tasks. Overall, all these components help improve the effectiveness of the BL2Vec model and enable the model to achieve superior performance than baselines. A detailed discussion on the effectiveness of each component is given as follows.
%
(1) BS features can effectively capture the spatial information of each ball; if the features are omitted, the classification performance drops significantly by around 14\%. %{\color{blue}
(2) BP features capture the correlations between the ball and each pocket, and these are the unique characteristics in the billiards layout data. In addition, BP features are associated with the most tokens (i.e., $4 \times 6 =24$) in the total of 27 tokens to represent each ball as discussed in Section~\ref{subsec:feature_extraction}, and therefore the BP features contribute the most for all of the tasks. As expected, we observe that if the BP features are omitted, the performance of similarity search drops by 88\% (resp. 96\%) in terms of HR@10 (resp. MRR); that of classification drops by 30\% in terms of accuracy; that of clustering drops by 20\% (resp. 21\%) in terms of ARI (resp. AMI). (3) BB features capture the correlation between balls in the layout. The features also affect the overall performance. For example, if the BB features are omitted, the clustering performance drops a lot by around 15\% (resp. 2\%) in terms of ARI (resp. AMI). {\ICDMComment (4) the CNN in $Net(\cdot)$ can well capture the correlation of those spatial features (i.e., BS, BP and BB), and simply using the average of feature embeddings cannot lead to the superior performance, e.g., similarity search drops by 57.4\% (resp. 69.05\%) in terms of HR@10 (resp. MRR).}

% We also study our improvements on feature engineering of billiards layouts for the spatial data. Table \ref{tab:ablation} shows BL2Vec performance on three
% different conditions. Feature engineering of billiards layouts consists of three kinds of features. Firstly, we talk about BS features.
% It is positions of balls in each billiards layout, which are transformed into tokens by dividing cells on the pool table, which has been introduced in parameter study.
% From the table, we notice that if BS features are omitted, the performance of BL2Vec on accuracy and clustering are worse.
% We next talk about BP features. It is ball-to-pocket features. We know there are 6 pockets on the pool table. For each pocket, we use 4 features to
% represent features of the ball to it. These four features are a minimum value between the degree between the vector from the ball to the pocket and the eft cushion
% and the degree between the vector from the ball to the pocket and right cushion, the distance from a ball to a pocket, 0/1 to denote whether the pocket can be potted or not because
% if a ball whose number is larger than the ball lies in the path from the current ball with the smallest number on the billiards
% table to a pocket, we know the current ball cannot be potted to this pocket with the index is equal to 0, the index is equal to 1 otherwise, and the last feature is the pocket index from 0 to 5 namely 6 pockets on the pool table.
% Because there are 6 pockets on the poll table and the number of features from the current ball to each pocket are 4, there are 24 features represent the second kind of features belonging to BP (ball-to-pocket).
% From the table, we can notice that when these 24 features are omitted, the performance of BL2Vec in similarity, classification and clustering are worst, with HR@10 0.08, MRR 0.005, Accuracy 50.37, ARI 49.50 and AMI 49.65.
% The last kind of features are belonging to BB, which represents features from the former ball to the current ball. It consists of two features, namely the most possible pocket index which represents the most possible pocket the current ball can be potted and
% the degree between the vector from the former ball to the current ball and the vector from the current ball to the most possible pocket.
% We can see from the table that omitting this kind of features affects a little performance on similarity. Thus, we can see that BP features are the most important features for the BL2Vec.

\noindent \textbf{(6) Scalability.}
\label{sec:efficiency}
%In this part, we evaluate the efficiency of different methods for the billiards layout retrieval over 100 queries. 
{\ICDMComment 
To test scalability, we generate more layouts by adding noise on the original dataset.
}
Figure \ref{fig:efficiency} reports the average running time over 100 queries for computing the similarity between a query billiards layout and the billiards layouts when we vary the size of the target database {\ICDMComment from 10,000 layouts to 50,000 layouts.}
%
Clearly, EMD and Hausdorff perform extremely slow, which match their quadratic time complexity.
%
We observe the running time of DTW and Frechet is smaller than that of EMD and Hausdorff though all of them have the same time complexity. This is because DTW and Frechet compute the similarity via dynamic programming to find an
optimal pairwise point-matching.
%
%{\color{blue}
PM is faster than DTW and Frechet because it matches the balls peer-to-peer based on their numbers and the complexity is linear.%}
In addition, DeepSets, WSSET, Rapset and BL2Vec have a similar running time.
Specifically, they run up to 170 times faster than EMD and Hausdorff, 100 times faster than DTW and Frechet and 50 times faster than PM. Moreover, we notice that DeepSets, WSSET, Rapset and BL2Vec scale linearly with the dataset size and the disparity between them increases as the size of the target database grows. This is because all of the learning-based methods have linear time complexity to compute the similarity by embedding layouts to vectors, and the embedding process can also be done offline, which is consistent with their time complexities.
%the discussion in Section~\ref{subsec:complexity}.

\begin{figure*}
\centering
\begin{tabular}{c c c c c}
  \begin{minipage}{0.18\linewidth}
  \includegraphics[width=\linewidth]{figures/user/query_63_63}%
  \end{minipage}
  &
  \begin{minipage}{0.18\linewidth}
    \includegraphics[width=\linewidth]{figures/user/query_40_40}%
  \end{minipage}
  &
  \begin{minipage}{0.18\linewidth}
  \includegraphics[width=\linewidth]{figures/user/query_42_42}%
  \end{minipage}
  &
  \begin{minipage}{0.18\linewidth}
    \includegraphics[width=\linewidth]{figures/user/query_43_43}%
  \end{minipage}
  &
  \begin{minipage}{0.18\linewidth}
    \includegraphics[width=\linewidth]{figures/user/query_46_46}%
  \end{minipage}
  \\
  Q1
  &
  Q2
  &
  Q3
  &
  Q4
  &
  Q5
 % \\
%  \begin{minipage}{0.18\linewidth}
%  \includegraphics[width=\linewidth]{figures/user/query_50_50}%
%  \end{minipage}
%  &
%  \begin{minipage}{0.18\linewidth}
%    \includegraphics[width=\linewidth]{figures/user/query_16_16}%
%  \end{minipage}
%  &
%  \begin{minipage}{0.18\linewidth}
%  \includegraphics[width=\linewidth]{figures/user/query_82_82}%
%  \end{minipage}
%  &
%  \begin{minipage}{0.18\linewidth}
%    \includegraphics[width=\linewidth]{figures/user/query_78_78}%
%  \end{minipage}
%  &
%  \begin{minipage}{0.18\linewidth}
%    \includegraphics[width=\linewidth]{figures/user/query_84_84}%
%  \end{minipage}
%  \\
%  Q6
%  &
%  Q7
%  &
%  Q8
%  &
%  Q9
%  &
%  Q10
\end{tabular}
\vspace*{-3mm}
\caption{First five queries that are used for user study.}
\label{userstudy}
\vspace*{-2mm}
\end{figure*}

%\begin{figure}
%%\hspace*{-.3cm}
%\centering
%\begin{tabular}{c c}
%  \begin{minipage}{0.99\linewidth}
%	\includegraphics[width=\linewidth]{figures/user_study}
%  \end{minipage}
%\end{tabular}
%%\vspace{-2mm}
%%\setlength{\abovecaptionskip}{1pt}
%\caption{User study for billiards layout retrieval.}
%\label{fig:userstudy}
%\end{figure}

\begin{figure*}
\centering
\begin{tabular}{c c c c c}
  \begin{minipage}{0.18\linewidth}
  \includegraphics[width=\linewidth]{figures/user/dtw_63_0}%
  \end{minipage}
  &
  \begin{minipage}{0.18\linewidth}
    \includegraphics[width=\linewidth]{figures/user/dtw_40_0}%
  \end{minipage}
  &
  \begin{minipage}{0.18\linewidth}
  \includegraphics[width=\linewidth]{figures/user/dtw_42_0}%
  \end{minipage}
  &
  \begin{minipage}{0.18\linewidth}
    \includegraphics[width=\linewidth]{figures/user/dtw_43_0}%
  \end{minipage}
  &
  \begin{minipage}{0.18\linewidth}
    \includegraphics[width=\linewidth]{figures/user/dtw_46_0}%
  \end{minipage}
  \\
  DTW 1 (1/10)
  &
  DTW 2 (2/10)
  &
  DTW 3 (1/10)
  &
  DTW 4 (6/10)
  &
  DTW 5 (6/10)
  \\
  \begin{minipage}{0.18\linewidth}
  \includegraphics[width=\linewidth]{figures/user/dml_63_0}%
  \end{minipage}
  &
  \begin{minipage}{0.18\linewidth}
    \includegraphics[width=\linewidth]{figures/user/dml_40_0}%
  \end{minipage}
  &
  \begin{minipage}{0.18\linewidth}
  \includegraphics[width=\linewidth]{figures/user/dml_42_0}%
  \end{minipage}
  &
  \begin{minipage}{0.18\linewidth}
    \includegraphics[width=\linewidth]{figures/user/dml_43_0}%
  \end{minipage}
  &
  \begin{minipage}{0.18\linewidth}
    \includegraphics[width=\linewidth]{figures/user/dml_46_0}%
  \end{minipage}
  \\
  BL2Vec 1 (9/10)
  &
  BL2Vec 2 (8/10)
  &
  BL2Vec 3 (9/10)
  &
  BL2Vec 4 (4/10)
  &
  BL2Vec 5 (4/10)
  \\
\end{tabular}
\setlength{\abovecaptionskip}{1pt}
\caption{Top-1 billiards layouts for Q1-Q5 returned by DTW and BL2Vec, (1/10) means the 1 user supports this result among the total of 10 users.}
\label{top5}
\vspace*{-2mm}
\end{figure*}

%\begin{figure}
%\centering
%\begin{tabular}{c c c c c}
%  \begin{minipage}{0.18\linewidth}
%  \includegraphics[width=\linewidth]{figures/user/dtw_40_0}%-eps-converted-to
%  \end{minipage}
%  &
%  \begin{minipage}{0.18\linewidth}
%    \includegraphics[width=\linewidth]{figures/user/dtw_42_0}%-eps-converted-to
%  \end{minipage}
%  &
%  \begin{minipage}{0.18\linewidth}
%  \includegraphics[width=\linewidth]{figures/user/dtw_43_0}%-eps-converted-to
%  \end{minipage}
%  &
%  \begin{minipage}{0.18\linewidth}
%    \includegraphics[width=\linewidth]{figures/user/dtw_46_0}%-eps-converted-to
%  \end{minipage}
%  &
%  \begin{minipage}{0.18\linewidth}
%    \includegraphics[width=\linewidth]{figures/user/dtw_50_0}%-eps-converted-to
%  \end{minipage}
%  \\
%  DTW (2/10)
%  &
%  DTW (1/10)
%  &
%  DTW (6/10)
%  &
%  DTW (6/10)
%  &
%  DTW (0/10)
%  \\
%  \begin{minipage}{0.18\linewidth}
%  \includegraphics[width=\linewidth]{figures/user/dml_40_0}%-eps-converted-to
%  \end{minipage}
%  &
%  \begin{minipage}{0.18\linewidth}
%    \includegraphics[width=\linewidth]{figures/user/dml_42_0}%-eps-converted-to
%  \end{minipage}
%  &
%  \begin{minipage}{0.18\linewidth}
%  \includegraphics[width=\linewidth]{figures/user/dml_43_0}%-eps-converted-to
%  \end{minipage}
%  &
%  \begin{minipage}{0.18\linewidth}
%    \includegraphics[width=\linewidth]{figures/user/dml_46_0}%-eps-converted-to
%  \end{minipage}
%  &
%  \begin{minipage}{0.18\linewidth}
%    \includegraphics[width=\linewidth]{figures/user/dml_50_0}%-eps-converted-to
%  \end{minipage}
%  \\
%  BL2Vec (8/10)
%  &
%  BL2Vec (9/10)
%  &
%  BL2Vec (4/10)
%  &
%  BL2Vec (4/10)
%  &
%  BL2Vec (10/10)
%\end{tabular}
%\setlength{\abovecaptionskip}{1pt}
%\caption{Top-1 billiards layouts for Q2-Q6 returned by DTW and BL2Vec (from left to right).}
%\label{top1q2q6}
%\end{figure}

%\begin{figure*}
%\flushleft
%\begin{tabular}{c c c c}
%  \begin{minipage}{0.18\linewidth}
%  \includegraphics[width=\linewidth]{figures/user/dtw_16_0}%-eps-converted-to
%  \end{minipage}
%  &
%  \begin{minipage}{0.18\linewidth}
%    \includegraphics[width=\linewidth]{figures/user/dtw_82_0}%-eps-converted-to
%  \end{minipage}
%  &
%  \begin{minipage}{0.18\linewidth}
%  \includegraphics[width=\linewidth]{figures/user/dtw_78_0}%-eps-converted-to
%  \end{minipage}
%  &
%  \begin{minipage}{0.18\linewidth}
%    \includegraphics[width=\linewidth]{figures/user/dtw_84_0}%-eps-converted-to
%  \end{minipage}
%  \\
%  DTW (1/10)
%  &
%  DTW (1/10)
%  &
%  DTW (1/10)
%  &
%  DTW (0/10)
%  \\
%  \begin{minipage}{0.18\linewidth}
%  \includegraphics[width=\linewidth]{figures/user/dml_16_0}%-eps-converted-to
%  \end{minipage}
%  &
%  \begin{minipage}{0.18\linewidth}
%    \includegraphics[width=\linewidth]{figures/user/dml_82_0}%-eps-converted-to
%  \end{minipage}
%  &
%  \begin{minipage}{0.18\linewidth}
%  \includegraphics[width=\linewidth]{figures/user/dml_78_0}%-eps-converted-to
%  \end{minipage}
%  &
%  \begin{minipage}{0.18\linewidth}
%    \includegraphics[width=\linewidth]{figures/user/dml_84_0}%-eps-converted-to
%  \end{minipage}
%  \\
%  BL2Vec (9/10)
%  &
%  BL2Vec (9/10)
%  &
%  BL2Vec (9/10)
%  &
%  BL2Vec (10/10)
%\end{tabular}
%\setlength{\abovecaptionskip}{1pt}
%\begin{center}
%\caption{Top-1 billiards layouts for Q7-Q10 returned by DTW and BL2Vec (from left to right).}
%\label{top1q710}
%\end{center}
%\end{figure*}
%as shown in Figure~\ref{fig:effectiveness}
\noindent \textbf{(7) User study.} {\ICDMComment In general, DTW performs the best among all baselines in the similar billiards layout retrieval task}, we conduct a user study to compare the BL2Vec with DTW. We randomly select 10 billiards layouts as the queries as shown in Figure~\ref{userstudy} for the first five queries Q1 to Q5, and for each query in the query set, we use BL2Vec and DTW to retrieve Top-1 billiards layouts from the target database.
%
We invite ten volunteers with strong billiards knowledge to annotate the relevance of the retrieved results. More specifically, we firstly spent 15 minutes introducing the background to the volunteers so that they understand these queries. Then for each of 10 queries, the volunteers specify the more similar result from the Top-1 result retrieved by BL2Vec and the Top-1 result retrieved by DTW. Note that the volunteers do not know which result is returned by which method in advance. We report the scores of the ten queries for both methods in Figure~\ref{fig:userstudy}. We observe that our BL2Vec outperforms DTW with expert knowledge. In particular, BL2Vec outperforms DTW for 8 queries out of the total 10 queries. In addition, BL2Vec gets 81\% votes while DTW gets only 19\% votes. {\Comment We illustrate the Top-1 results of BL2Vec and DTW for the Q1 to Q5 in Figure~\ref{top5}. 
%, and the Top-1 results of BL2Vec and DTW for Q2 to Q10 in Figure~\ref{top1q2q6} and Figure~\ref{top1q710}, respectively. 
From these figures, we observe the layouts retrieved by BL2Vec match the queries very well. For example, we find that the overall layout of the TOP-1 result by BL2Vec is very similar to Q1. We also note taht DTW is slightly better than BL2Vec for Q4 and Q5 (i.e., by 2\% votes).
We believe this might be because the layouts returned by DTW have the locations of the balls more similar to those in the query layouts and this is perceived by the users. Nevertheless, with a closer check, the balls at similar locations in the layouts returned by DTW and the query layouts are of different numbers (i.e., colors) and thus they should be regarded be not that similar to each other. This illustrates DTW's drawback that it does not captures other information than the locations of layouts well.
% This is because the overall layouts returned by DTW are more similar to the queries; however, DTW falsely matches the balls, e.g., 9 balls in Q4, but the layout returned by DTW only has 7 balls and they are matched with different colors.
We omit the results for Q6 to Q10 due to the page limit.}

%, and the Top 2-5 results also maintain high consistency in the layouts. %{\color{blue}
%DTW is slightly better than BL2Vec for Q4 and Q5 (i.e., 2\% votes). This is because the overall layouts returned by DTW are more similar to the queries; however, DTW falsely matches the balls, e.g., 9 balls in Q4, but the layout returned by DTW only has 7 balls and they are matched with different colors.%}
%It indicates that the pairwise point-matching solution is not suitable for the billiards layout retrieval task. 

==> conclusion.tex <==
\section{CONCLUSION}
\label{sec:conclusion}
In this paper, we propose a novel deep reinforcement learning based solution called \texttt{RL4OASD} for online anomalous subtrajectory detection. \texttt{RL4OASD} incorporates the information of trajectory mobility and road network structure for detecting anomalies, it trains in a weakly supervised framework with noisy labels and can efficiently detect anomalous subtrajectories in an online manner. Experiments on two real-world taxi trajectory datasets demonstrate \texttt{RL4OASD} consistently outperforms existing algorithms, and runs comparably fast. In the future, we will explore other types of anomalous trajectories, such as temporally anomalous trajectories, or detecting anomalous trajectories in trajectory streams.

==> experiments.tex <==
\section{EXPERIMENTS}
\label{sec:experiment}
\subsection{Experimental Setup}
\label{sec:setup}


\noindent \textbf{Dataset.}
The experiments are conducted on two real-world taxi trajectory datasets from DiDi Chuxing~\footnote{https://outreach.didichuxing.com/research/opendata/en/}, namely \emph{Chengdu} and \emph{Xi'an}. All raw trajectories are preprocessed to map-matched trajectories via a popular map-matching algorithm~\cite{yang2018fast}, and the road networks of the two cities are obtained from OpenStreetMap~\footnote{https://www.openstreetmap.org/}.
%

\noindent \textbf{Ground Truth.} 
By following the previous works~\cite{zhang2011ibat,chen2013iboat, lv2017outlier}, we manually label the anomalous subtrajectories, and take the labeled subtrajectories as the ground truth for the evaluation.
%
Specifically, we randomly sample 200 SD-Pairs following the distribution of their traveled frequency in each dataset. For labeling subtrajectories, we illustrate all routes (i.e., map-matched trajectories) within each SD-Pair as shown in Figure~\ref{fig:casestudy}. We invite 5 participants and let them to identify whether the routes are anomalous or not based on the visualization. If one route is identified as the anomalous, we ask the volunteer to label which parts are responsible for its anomalousness. %{\Comment{In addition, we also double-check the trajectories to make sure the quality, and relabel some of them if necessary.}}
{\Comment{For quality control, we randomly pick 10\% trajectories, ask 5 other checkers to label these trajectories independently, adopt the majority voting to aggregate the labels, and compute the accuracy of the labels by the labelers against the aggregated ones by the checkers. The accuracy is 98.7\% for Chengdu and 94.3\% for Xi'an, which shows that our labeled datasets are with high accuracy.}}

{\Comment{Multiple trajectories may correspond to the same route and thus we have fewer routes than trajectories. We label 1,688 (resp. 1,057) routes, which correspond to 558,098 (resp. 163,027) raw trajectories before map-matching for Chengdu (resp. Xi'an). Among them, 1,436 (resp. 813) routes that correspond to 3,930 (resp. 2,368) raw trajectories are identified as the anomalous for Chengdu (resp. Xi'an), where the anomalous ratios for Chengdu and Xi'an are estimated as $3,930/558,098=0.7\%$ and $2,368/163,027=1.5\%$, respectively. The statistics of the two datasets are reported in Table~\ref{tab:dataset}.}} 

\begin{table}[]
\setlength{\tabcolsep}{4pt}
\centering
\caption{Dataset statistics.}
\vspace*{-2mm}
\begin{tabular}{lll}
\hline
Dataset             & Chengdu       & Xi'an         \\ \hline
\# of trajectories      & 677,492       & 373,054       \\
\# of segments          & 4,885         & 5,052         \\
\# of intersections     & 12,446        & 13,660        \\
\# of labeled routes  & 1,688/558,098 & 1,057/163,027 \\
\# of anomalous routes & 1,436/3,930   & 813/2,368     \\
Anomalous ratio     & 0.7\%         & 1.5\%         \\ \hline
\end{tabular}
\label{tab:dataset}
\vspace*{-2mm}
\end{table}

\noindent \textbf{Baseline.}
We review the literature thoroughly, and identify the following baselines for the online detection problem, including IBOAT~\cite{chen2013iboat}, DBTOD~\cite{wu2017fast}, GM-VSAE~\cite{liu2020online}, SD-VSAE~\cite{liu2020online}, SAE~\cite{malhotra2016lstm}, VSAE~\cite{kingma2013auto} and CTSS~\cite{zhang2020continuous}. The detailed description of these algorithms is discussed in Section~\ref{sec:related}. For SAE and VSAE, they are adapted from GM-VSAE, where SAE replaces the encoder and decoder structure in GM-VSAE with a traditional Seq2Seq model, which aims to minimize a reconstruction error, and the reconstruction error is further used to define the anomaly score. VSAE replaces the Gaussian mixture distribution of the latent route representations in GM-VSAE with a Gaussian distribution.

\if 0
\\
$\bullet$. IBOAT is a isolation-based method for detecting anomalous trajectories online by identifying which parts of a detected trajectory can be separated from others.
\\
$\bullet$. DBTOD is based on a probabilistic model to detect online anomalous trajectories via modeling the driving behavior from historical trajectories. For modeling the driving behavior, it takes some related features into account, including historical average speed, road level and turning angle.
\\
$\bullet$. GM-VSAE is a learning-based model to detect online anomalous trajectories via the generation scheme, by modeling a Gaussian mixture distribution into a sequential autoencoder structure.
\\
$\bullet$. SD-VSAE is a fast version of GM-VSAE. It replaces the encoder part of GM-VSAE with a distillation network (i.e., SD-network) to support efficient online detection.
\\
$\bullet$. SAE and VSAE are two adapted versions of GM-VSAE. In particular, SAE is a traditional Seq2Seq based learning model by minimizing the reconstruction error for the generation. VSAE is based on a traditional VAE structure, 
\\
$\bullet$. CTSS is the state-of-the-art method proposed for online detour detection. It continues to monitor an online detour by extending the partial trajectory to the destination and applies the Frechet distance to measure the trajectory similarity with a selected normal route.
\fi

\begin{table*}[]
\caption{Effectiveness comparison with existing baselines.}
\vspace{-2mm}
%\small
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|}
\hline
Mathods           & \multicolumn{5}{c|}{Chengdu} & \multicolumn{5}{c|}{Xi'an} \\ \hline
Trajectory Length & G1    & G2    & G3    & G4  &Overall & G1    & G2   & G3   & G4  &Overall \\ \hline
IBOAT~\cite{chen2013iboat}             &0.426       &0.431       &0.406       &0.590  &0.431   &0.424       &0.467      &0.487      &0.503  &0.472    \\ \hline
DBTOD~\cite{wu2017fast}             &0.523       &0.531       &0.515       &0.669  &0.530    &0.519       &0.448      &0.441      &0.483 &0.433     \\ \hline
GM-VSAE~\cite{liu2020online}           &0.375       &0.493       &0.504       &0.658  &0.451    &0.371       &0.464      &0.498      &0.521 &0.467     \\ \hline
SD-VSAE~\cite{liu2020online}           &0.373       &0.491       &0.498       &0.637  &0.448    &0.373       &0.459      &0.478      &0.507 &0.458    \\ \hline
SAE~\cite{malhotra2016lstm}               &0.375       &0.492       &0.499       &0.658  &0.450    &0.372       &0.460      &0.479      &0.517 &0.461     \\ \hline
VSAE~\cite{kingma2013auto}              &0.374       &0.492       &0.504       &0.656  &0.450   &0.369       &0.461      &0.487      &0.520  &0.463    \\ \hline
CTSS~\cite{zhang2020continuous}              &0.730       &0.708       &0.625       &0.741  &0.706   &0.657       &0.637      &0.636      &0.672  & 0.658   \\ \hline
\textbf{RL4OASD}           &\textbf{0.888}       &\textbf{0.892}       &\textbf{0.725}       &\textbf{0.774} & \textbf{0.854}     &\textbf{0.964}       &\textbf{0.864}      &\textbf{0.809}     &\textbf{0.844}  &\textbf{0.857}    \\ \hline
\end{tabular}
\label{tab:baselines}
\vspace*{-3mm}
\end{table*}

\begin{table}[ht]
\setlength{\tabcolsep}{4pt}
\centering
\caption{Impacts of parameter $\alpha$ for \texttt{RL4OASD}.}
\vspace*{-2mm}
\begin{tabular}{|c|c|c|c|c|c|c|}
\hline
Parameter & $\alpha=0.3$ & $\alpha=0.4$ & $\alpha=0.5$ & $\alpha=0.6$ & $\alpha=0.7$ \\ \hline
$F_1$-score &0.844 &0.845 &\textbf{0.849} &0.846 &0.845 \\ \hline
\end{tabular}
\label{tab:alpha}
\vspace*{-2mm}
\end{table}

\begin{table}[ht]
\setlength{\tabcolsep}{4pt}
\centering
\caption{Impacts of parameter $\delta$ for \texttt{RL4OASD}.}
\vspace*{-2mm}
\begin{tabular}{|c|c|c|c|c|c|c|}
\hline
Parameter & $\delta=0.1$ & $\delta=0.2$ & $\delta=0.3$ & $\delta=0.4$ & $\delta=0.5$ \\ \hline
$F_1$-score &0.647 &0.834 &0.846 &\textbf{0.849} &0.847 \\ \hline
\end{tabular}
\label{tab:delta}
\vspace*{-2mm}
\end{table}

\begin{table}[ht]
\setlength{\tabcolsep}{4pt}
\centering
\caption{Impacts of parameter $D$ for \texttt{RL4OASD}.}
\vspace*{-2mm}
\begin{tabular}{|c|c|c|c|c|c|c|c|}
\hline
Parameter & $D=0$ & $D=2$ & $D=4$ & $D=6$ & $D=8$ & $D=10$ \\ \hline
$F_1$-score &0.737 &0.763 &0.812 &0.833 &\textbf{0.849} &0.852\\ \hline
\end{tabular}
\label{tab:D}
\vspace*{-2mm}
\end{table}

\noindent \textbf{Parameter Setting.} In RSRNet, we embed the TCF and NRF features into the 128-dimensional vectors, and use the LSTM with 128 hidden units to implement the RSRNet. To train RSRNet, we construct noisy labels in 24 time slots with one hour granularity via empirical studies. The parameter $\alpha$ and $\delta$ are set to 0.5 and 0.4 by default. In ASDNet, the dimension of label vectors $\mathbf{v}(e_{i}.l)$ is 128. The policy network is implemented with a single-layer feedforward neural network, and the softmax function is adopted as the activation function. The delay parameter $D$ is set to 8 by default. By empirical findings, the learning rates for RSRNet and ASDNet are set to 0.01 and 0.001, respectively. For baselines, we follow their strategies in the original papers.

\noindent \textbf{Evaluation Metrics.}
{\Comment{To verify the results of subtrajectory detection, we adapt the evaluation metric $F_1$-score proposed for Named Entity Recognition (NER)~\cite{li2020survey,li2021effective}.
This is inspired by the fact that our task corresponds to one of tagging subsequences of a sequence, which is similar to NER, which tags phrases (i.e., subsequences) of a sentence (sequence).

The intuition is that we take the anomalous subtrajectories as entities in NER task. Specifically, (1) let $C_{g,i}$ denote a manually labeled anomalous subtrajectory $i$ in the ground truth set $C_g$, and $C_{o,i}$ denotes the corresponding subtrajectory $i$ in the set $C_o$, which is returned by a detection method. We employ Jaccard to measure the ratio of intersection over union of the road segments between $C_{g,i}$ and $C_{o,i}$, that is 
\begin{align*}
\mathcal{J}_i(C_{g,i},C_{o,i}) &= \frac{|C_{g,i} \cap C_{o,i}|}{|C_{g,i} \cup C_{o,i}|}.
\end{align*}
(2) We then measure the similarity between $C_{g}$ and $C_{o}$ by aggregating the Jaccard $\mathcal{J}_i(C_{g,i},C_{o,i})$, that is 
\begin{align*}
\mathcal{J}(C_g, C_o) &= \sum_{i=1}^{|C_g|} \mathcal{J}_i(C_{g,i},C_{o,i}).
\end{align*}
(3) Finally, we define the precision and recall by following~\cite{li2020survey,li2021effective}, and compute the $F_1$-score accordingly.
\begin{align*}
\text{Precision} &= \frac{\mathcal{J}(C_g, C_o)}{|C_o|}, \quad \text{Recall} = \frac{\mathcal{J}(C_g, C_o)}{|C_g|},\\
F_{1} &= 2\times\frac{\text{Precision}\times\text{Recall}}{\text{Precision}+\text{Recall}}.
\end{align*}
}}

\if 0
{\Comment{To verify the results of subtrajectory detection, we adapt the evaluation metric $F_1$-score proposed for Named Entity Recognition (NER)~\cite{li2020survey,li2021effective}. 
The intuition is that we take the anomalous subtrajectories as entities in NER task, and define the precision and recall accordingly.
\begin{align*}
\text{Precision} = \frac{\mathcal{J}(C_o, C_g)}{|C_o|}, &\quad \text{Recall} = \frac{\mathcal{J}(C_o, C_g)}{|C_g|}\\
\mathcal{J}(C_o, C_g) &= \sum_{i=1}^{|C_g|} \frac{|C_{o,i} \cap C_{g,i}|}{|C_{o,i} \cup C_{g,i}|},
\end{align*}
where $C_o$ denotes a set of outputted anomalous subtrajectories by a detection method and $C_g$ denotes a set of ground truth anomalous subtrajectories via manually labeling. 
%
$\mathcal{J}(C_o, C_g)$ denotes the Jaccard index, which measures the ratio of intersection over union of the two sets $C_o$ and $C_g$.
%
To compute $\mathcal{J}(C_o, C_g)$, we first align the anomalous subtrajectories in $C_o$ and $C_g$ according to their corresponding trajectory ids. For the subtrajectories that cannot be aligned, we simply discard them. For each aligned pair $i$ in $C_o$ and $C_g$ (i.e., $C_{o,i}$ and $C_{g,i}$), we compute their Jaccard's as the size of the intersection divided by the size of the union of the road segments in $C_{o,i}$ and $C_{g,i}$, then we take the summation of Jaccard's of all pairs as $\mathcal{J}(C_o, C_g)$. Finally, the $F_1$-score is defined as
\begin{align*}
F_{1} = 2\times\frac{\text{Precision}\times\text{Recall}}{\text{Precision}+\text{Recall}}.
\end{align*}
}}
\fi
%
We notice the existing solutions~\cite{chen2013iboat,wu2017fast,liu2020online,zhang2020continuous} output an anomaly score on each point in a detected trajectory. To support this for subtrajectory detection, we turn their thresholds of the anomaly scores in a development set (i.e, a set of 100 trajectories with manual labels), and for each turned threshold, the anomalous subtrajectories $C_o$ is identified as those road segments, whose anomaly scores are larger than the threshold. and the threshold that is associated with the highest $F_1$-score is selected for experiments.
%
For \texttt{RL4OASD}, it naturally outputs the anomalous subtrajectories, and we can compute its $F_1$-score based on the defined precision and recall directly.

\noindent \textbf{Evaluation Platform.}
We implement \texttt{RL4OASD} and other baselines in Python 3.6 and Tensorflow 1.8.0. 
The experiments are conducted on a server with 10-cores of Intel(R) Core(TM) i9-9820X CPU @ 3.30GHz 64.0GB RAM and one Nvidia GeForce RTX 2080 GPU. The labeled datasets and codes can be downloaded via the link~\footnote{https://www.dropbox.com/sh/imix3otoep49v0g/AACQLPpgA0jMdTg7LV-GdL70a?dl=0} to reproduce our work.

 

\subsection{Experimental Results}
\label{sec:effectiveness}

\noindent \textbf{(1) Effectiveness evaluation (comparison with existing baselines).}
We study the anomalous subtrajectory detection with our labeled datasets. In Table~\ref{tab:baselines}, we report the effectiveness in terms of different trajectory lengths, e.g., we manually partition the Chengdu dataset into four groups, i.e., G1, G2, G3 and G4, such that the lengths in a groups are $G1<15$, $15 \leq G2 < 30$, $30 \leq G3 <45$ and $G4 \geq 45$. In addition, we also report the overall effectiveness in whole datasets. The results clearly show that \texttt{RL4OASD} consistently outperforms baselines in terms of different settings. For example, it outperforms the best baseline (i.e., CTSS) for around 21\% (resp. 30\%) in Chengdu (resp. Xi'an) in terms of the overall effectiveness, which verifies its data-driven nature.

% \begin{table}[ht]
% \setlength{\tabcolsep}{4pt}
% \centering
% \caption{Impacts of time granularity (hours) for \texttt{RL4OASD}.}
% \vspace*{-2mm}
% \begin{tabular}{|c|c|c|c|c|c|c|}
% \hline
% Parameter & 1 hr & 2 hrs  & 3 hrs & 4 hrs & 5 hrs \\ \hline
% $F_1$-score & & & & & \\ \hline
% \end{tabular}
% \label{tab:parameterL}
% \vspace*{-2mm}
% \end{table}


\begin{table}[ht]
\setlength{\tabcolsep}{4pt}
\centering
\caption{Ablation study for \texttt{RL4OASD}.}
\vspace*{-2mm}
\begin{tabular}{|c|c|}
\hline
Effectiveness           & $F_1$-score  \\ \hline
RL4OASD           &\textbf{0.854}         \\ \hline
w/o noisy labels & 0.626         \\ \hline
w/o road segment embeddings &  0.828       \\ \hline
w/o RNEE  & 0.816    \\ \hline
w/o local reward  &0.850         \\ \hline
w/o global reward  &0.849         \\ \hline
%\begin{tabular}[c]{@{}c@{}}0.811 \\(degrade 9.6\% in efficiency)\end{tabular}
\end{tabular}
\label{tab:ablation}
\vspace*{-2mm}
\end{table}

\begin{figure}[h]
\hspace{-.8cm}
\centering
\begin{tabular}{c}
  \begin{minipage}{0.93\linewidth}%5.5
    \includegraphics[width=1.02\linewidth]{figures/overall_efficiency_legend.pdf}
   \end{minipage}
   \\
  \begin{minipage}{0.93\linewidth}%5.5
    \includegraphics[width=1.02\linewidth]{figures/overall_efficiency_new.pdf}
  \end{minipage}
\end{tabular}
\vspace*{-3mm}
\caption{Overall detection efficiency.}
\label{fig:overall_efficiency}
\vspace*{-4mm}
\end{figure}

\begin{figure}[h]
	\hspace{-.8cm}
	\centering
	\begin{tabular}{c c}
		\begin{minipage}{3.7cm}
			\includegraphics[width=3.9cm]{figures/traj_length_chengdu_2.pdf}
		\end{minipage}
		&
		\begin{minipage}{3.7cm}
			\includegraphics[width=3.9cm]{figures/traj_length_xian_2.pdf}
		\end{minipage}
		\\
		(a) Chengdu
		&
		(b) Xi'an
	\end{tabular}
	\vspace*{-3mm}
	\caption{Efficiency with varying trajectory lengths.}\label{fig:length}
	\vspace{-4mm}
\end{figure}

\begin{figure*}
\centering
\begin{tabular}{c c c c c}
  \begin{minipage}{0.22\linewidth}
  \includegraphics[width=\linewidth]{figures/ground-1000-180-20-choose.pdf}%
  \end{minipage}
  &
  \begin{minipage}{0.22\linewidth}
    \includegraphics[width=\linewidth]{figures/ground-1000-180-28-choose.pdf}%
  \end{minipage}
  &
  \begin{minipage}{0.22\linewidth}
  \includegraphics[width=\linewidth]{figures/ground-453-4471-1-choose.pdf}%
  \end{minipage}
  &
  \begin{minipage}{0.22\linewidth}
    \includegraphics[width=\linewidth]{figures/ground-1000-3447-2-choose.pdf}%
  \end{minipage}
  \\
  (a) GT-1
  &
  (b) GT-2
  &
  (c) GT-3
  &
  (d) GT-4
  \\
 \begin{minipage}{0.22\linewidth}
 \includegraphics[width=\linewidth]{figures/ctss-1000-180-11-choose.pdf}%
 \end{minipage}
 &
 \begin{minipage}{0.22\linewidth}
    \includegraphics[width=\linewidth]{figures/ctss-1000-180-17-choose.pdf}%
 \end{minipage}
 &
 \begin{minipage}{0.22\linewidth}
 \includegraphics[width=\linewidth]{figures/ctss-453-4471-1-choose.pdf}%
 \end{minipage}
 &
 \begin{minipage}{0.22\linewidth}
    \includegraphics[width=\linewidth]{figures/ctss-1000-3447-0-choose.pdf}%
 \end{minipage}
 \\
  (e) CTSS, $F_1$=0.792
  &
  (f) CTSS, $F_1$=0.621
  &
  (g) CTSS, $F_1$=0.0
  &
  (h) CTSS, $F_1$=1.0
 \\
 \begin{minipage}{0.22\linewidth}
 \includegraphics[width=\linewidth]{figures/rl-1000-180-20-choose.pdf}%
 \end{minipage}
 &
 \begin{minipage}{0.22\linewidth}
    \includegraphics[width=\linewidth]{figures/rl-1000-180-28-choose.pdf}%
 \end{minipage}
 &
 \begin{minipage}{0.22\linewidth}
 \includegraphics[width=\linewidth]{figures/rl-453-4471-1-choose.pdf}%
 \end{minipage}
 &
 \begin{minipage}{0.22\linewidth}
    \includegraphics[width=\linewidth]{figures/rl-1000-3447-2-choose.pdf}%
 \end{minipage}
 \\
  (i) \texttt{RL4OASD}, $F_1$=1.0
  &
  (j) \texttt{RL4OASD}, $F_1$=1.0
  &
  (k) \texttt{RL4OASD}, $F_1$=1.0
  &
  (l) \texttt{RL4OASD}, $F_1$=1.0
\end{tabular}
\vspace*{-3mm}
\caption{Case study on Chengdu, blue lines: the normal routes traveled by most of trajectories; red dashed lines: the routes with anomalous subtrajectories (i.e., detours); red points: the intersections on road networks; green lines: the detected detours by Ground Truth (GT), CTSS and \texttt{RL4OASD}.}
\label{fig:casestudy}
\vspace*{-2mm}
\end{figure*}

%\noindent \textbf{(2) Effectiveness evaluation (varying parameter time slots).}

\noindent \textbf{(2) Effectiveness evaluation (varying parameter $\alpha$).} Table~\ref{tab:alpha} shows the effects of varying parameter $\alpha$ for constructing noisy labels for training \texttt{RL4OASD}. Intuitively, both smaller or larger $\alpha$ will affect the quality of noisy labels, and lead to the model performance degrades. We study the parameter in the labeled Chengdu dataset, and we observe its performance becomes better as $\alpha$ increases, and drops as the $\alpha$ further increases.

\noindent \textbf{(3) Effectiveness evaluation (varying parameter $\delta$).}
In Table~\ref{tab:delta}, we further study the effects of varying parameter $\delta$, where the $\delta$ controls the number of normal routes that will be selected for constructing normal route features. With a smaller $\delta$, many existing anomalous routes in the datasets will be falsely selected. With a larger $\delta$, only a few normal routes will be considered, e.g., when $\delta$ is set to 0.5, only one route (i.e., the most frequent 
route) will be selected as the normal route. As expected, a moderate $\delta$ provides the best effectiveness.

\noindent \textbf{(4) Effectiveness evaluation (varying parameter $D$).}
Parameter $D$ controls the number of road segments in the delaying mechanism in order to form longer subtrajectories instead of short fragments. The results of varying $D$ are reported in Table~\ref{tab:D}. We observe the model performance improves as $D$ grows, since a larger $D$ provides better continuity of detected subtrajectories. However, with a larger $D$, the capability of the model to detect multiple anomalous subtrajectories will degrade, which is as expected.

\noindent \textbf{(5) Effectiveness evaluation (ablation study).}
{\Comment{
We conduct an ablation study to show the effects of some important components in \texttt{RL4OASD}, including (1) noisy labels, (2) pre-trained road segment embeddings, (3) Road Network Enhanced Environment (RNEE), (4) local reward and (5) global reward. 
In particular, for (1), we replace the noisy labels with random labels;
for (2), we randomly initialize the embeddings of road segments to replace the pre-trained embeddings provided by Toast~\cite{chen2021robust}; for (3), we drop the RNEE, and the model needs to take the action at each road segment without guided by road networks; for (4), we drop the local reward, which encourages the continuity of refined labels; for (5), we drop the global reward, which provides some feedback indicating the quality of refined labels.
%for (4), we compute the global reward (i.e., $F_1$-score) in a development set with refined labels provided by ASDNet to replace manual labels. 
In Table~\ref{tab:ablation}, we observe each component benefits the overall effectiveness, where the noisy labels contribute quite much, because it provides a necessary warm-start before the training. With random labels, the model converges to a local optimum and it is difficult to obtain further optimization. In addition, with the RNEE, we notice an effectiveness improvement of around 5\%, since it simplifies the cases of making decisions and the model becomes easier to train. In addition, we notice an efficiency improvement of around 9\% of RNEE, because it saves the time of taking actions via neural networks.}}

\noindent \textbf{(6) Efficiency evaluation (overall detection).}
Figure~\ref{fig:overall_efficiency} reports the online detection efficiency in terms of average running time per point. We observe DBTOD runs the fastest on both datasets, because it is a light model with cheaper feature engineering efforts for a binary classification problem on detecting whether an anomaly is contained in a trajectory. CTSS runs the slowest since it involves discrete Frechet distance to compute the deviation between a detected trajectory and a given reference trajectory, which suffers from quadratic time complexity. Overall, \texttt{RL4OASD} runs reasonably fast and would meet the practical needs, e.g., it takes less than 1ms to process each point, which is much faster than the practical sampling rate of trajectory data.

\noindent \textbf{(7) Efficiency evaluation (detection scalability).}
Further, we study the scalability for detecting ongoing trajectories in terms of different trajectory lengths. In Figure~\ref{fig:length}, we report the average running time per trajectory on both datasets. In general, we notice CTSS performs the worst, and its disparity between other baselines becomes larger as the trajectory length increases. \texttt{RL4OASD} scales well with the trajectory length grows, and it is faster than most of the baselines for long trajectories. This is because it involves the graph structure of road networks for labeling road segments, and the time of taking actions is saved accordingly.

\noindent \textbf{(8) Case study.} In Figure~\ref{fig:casestudy}, we investigate four detour cases in Chengdu dataset, including the case of two detours, the long detour, the short detour and no detour in a detected trajectory. We visualize the detours with the green lines labeled by human, CTSS and \texttt{RL4OASD}, where we choose CTSS for comparison, since it shows the best effectiveness among baselines. The results clearly show that \texttt{RL4OASD} can accurately identify detours and the returned detours are more in line with human intuition, which demonstrates its capability for real applications.

==> introduction.tex <==

\section{INTRODUCTION}
\label{sec:introduction}

Trajectories, i.e., sequences of GPS points that tracks moving subjects (e.g., vehicles) on urban space, are being generated with our daily travel at an unprecedented speed. Trajectory data usually contain rich information about human mobility and urban transportation, and thus can be leveraged to empower various location-based services (LBS), e.g., urban planning and ride-hailing. 
% The availability of large-scale urban trajectories have
% revolutionized the methodology we investigate human mobility and urban transportation,
% As a result, mining frequent mobility patterns from trajectories has been extensively researched, and has been empowering many novel location-based services, such as location prediction.
% and many novel location-based services (LBS), such as location prediction, have been empowered by mining massive trajectories. 
% As such, trajectory data has 
% been utilized as an indispensable information source that empowers various location-based services (LBS), such as urban planning and ride-hailing. 
% With its widespread applications, 
With its ubiquity, 
% detecting vehicles that follows unusual mobility patterns, i.e., 
\emph{anomalous trajectory detection} has become an important concern. It reveals whether a moving object is spatially following a normal route during its travel, which is beneficial in many scenarios. For example, the managers of a transportation system can discover local traffic issues from crowded trajectory anomalies. A ride-hailing company can prevent and punish malicious overcharging via discovering unusual trajectory detour. 

% Motivated by this, 
In recent years, many approaches for anomalous trajectory detection have been proposed, while most of them aim to discriminate whether a given trajectory is anomalous,
i.e., following normal routes between two locations. They fail to answer a more critical and meaningful question: \textbf{Which part of a trajectory (i.e., subtrajectory) is anomalous?}
% In recent years, discovering anomalous behaviors in trajectory data has become an indispensable pathway that leads to continual improvement of downstream LBS. For example, the managers of a transportation system can discover potential traffic issues from accumulated trajectory anomalies in a local area. A taxi company can prevent and punish malicious overcharging via discovering trajectory detour. As such, the problem of \emph{anomalous trajectory detection} is being increasingly popular, and various approaches has been proposed. 
% However, existing studies still have obvious flaws to be employed in real-world applications, as an important question remains unanswered:
% However, to employ anomalous trajectory detection in real-world applications, existing studies still fail at answering one important question:
% cannot be accurately answered with most of the existing methods:
% \textbf{Which part of a trajectory (i.e., subtrajectory) is anomalous?} 
In real-world applications, trajectories are usually long sequences with many subtrajectories. Identifying anomalous subtrajectories is a necessity to accurately locate and indicate the anomalousness, which is crucial for the corresponding actions to be timely taken.
% , e.g., 
For example, a ride-haling company can take different measures based on where the detour is occurred and how long it lasts. 
% Unfortunately, most of the exiting studies can only output an anomalous score w.r.t. the entire trajectory, not to mention showing the anomalous subtrajectory that could be more insightful.
However, the anomalous subtrajectory detection problem is non-trivial to solve, due to three challenges:
% Motivated by this, we study the problem of anomalous subtrajectory detection in this paper, where three major challenges need to be tackled:
% Motivated by this, we propose a novel solution for anomalous subtrajectory detection, focus on answering the aforementioned question. However, solving this problem faces three major challenges:

% To bridge this gap, we study the problem of anomalous \emph{subtrajectory} detection, which focus on identifying the anomalous segment (i.e., subtrajectory) of a given trajectory. Nevertheless, to be applied to real-world applications, solving this problem faces non-trivial challenges:
% , which has the following challenges:
% Nevertheless, existing studies might not be fully applicable for real-world application, due to the following challenges:

\begin{itemize}[leftmargin=*]
    \item \textbf{Subtrajectory modeling}. The detection of anomalous subtrajectory heavily relies on understanding the mobility patterns of subtrajectories. This is a challenging task, as the complexity and variety of subtrajectories across different places can hardly be modeled by simple heuristics. Moreover, the mobility on urban space usually happens on road networks, which would have a significant impact on the appearance of subtrajectory anomalies and make the problem even more challenging.
    \item \textbf{Lack of labeled data}. Worst still, the modeling of normal and anomalous mobility patterns cannot depend on labeled data in this problem. Specifically, the anomalousness is extremely hard to be defined by simple rules, while manually labeling large-scale subtrajectories costs unaffordable human effort. This obstructs some straightforward data-intensive methods to be applied for this problem.
%     The key of trajectory anomaly
% detection is to effectively discover and represent the normal
% routes of trajectories. This is challenging because the normal
% routes of trajectories may vary across different places due
% to the complexity of transportation systems, and thus are
% difficult to be predefined and represented. Also, the sequential
% correlation between different segments of a normal route
% should also be considered, as it is imporatnt for detecting
% route-switching anomalies as shown in Figure 1.
    \item \textbf{Efficient online detection}. As trajectories are often generated at a very high speed, detection efficiency is also a central concern. Nevertheless, the number of subtrajectoies is several orders of magnitude larger than the number of trajectories. 
    % , which makes most of the previous studies infeasible to be adopted.
    Conventional offline detection methods that often need to enumerate all the subtrajectories are clearly infeasible. To avoid this, an optimal solution must enable \emph{online detection}, where the anomalousness can be revealed while a trajectory is being generated.
\end{itemize}
To this end, we propose a novel reinforcement learning based solution in this paper to tackle these challenges.
% Overall, our solution 1) employs deep neural networks to learn the mobility patterns of subtrajectories, 2) uses reinforcement learning techniques learn to label anomalous trajectories with limited supervision, and 3) conduct efficient online detection.
For the first challenge, we propose Road Segment Representation Network (SRNet), which exploits road network representation learning and deep sequence modeling techniques that jointly model the mobility pattern underlying subtrajectories. For the second challenge, we propose Anomalous Subtrajectory Detection Network (ASDNet), which is a policy network that is tailored for the detection of subtrajectories on road networks. ASDNet can be trained jointly with SRNet, in a weakly supervised manner using noisy labeled data. The two networks can mutually refine each other, where SRNet can provide expressive sequential information behind trajectories for ASDNet to detect, and ASDNet can offer supervision for SRNet to better learn the mobility patterns.
% It can sequentially detect the anomalousness of trajectory segments, and provide supervision for SRNet to learn the mobility patterns that can discriminate subtrajectory anomalies. 
For the third challenge, we propose a novel detection algorithm, namely RL4OASD, which leverages the learned policy and enables online detection of anomalous subtrajectories. 
% Overall, our proposed solution is able to expressively learn the complexity mobility patterns behind subtrajectories with limited labeled data, and efficiently detect subtrajectory anomalies in an online manner. 
Our contributions can be summarized as follows:
\begin{itemize}
    \item We propose the first deep reinforcement learning based solution to learn the mobility patterns of subtrajectories. The proposed model 1) integrates the information of trajectory mobility and road network structure, and 2) can be trained with limited labeled data.
    \item We propose a novel detection paradigm based on the learned policy, which allows the anomalous subtrajectory detection to be efficiently conducted in an online manner.
    \item We conduct extensive experiments on two real-world trajectory datasets with manually-labeled test data. We compare our proposed solution with various baselines, and the results show that our solution can significantly outperform the state-of-the-art methods and is efficient for online anomalous subtrajectory detection.
\end{itemize}

\noindent\textbf{22 Nov-Cheng: 1. The first challenge is not clear to me - some more elaborations are needed; 2. Some more details of the proposed model (e.g., intuition, how it solves the issues, novel ideas) are desired; In its current form, this part is too brief; 3. Some references are expected throughout the introduction (some of them have been marked as Overleaf comments).}

==> introduction2.tex <==
\section{INTRODUCTION}
\label{sec:introduction}
% 1. emphasis this problem important
% 2. important (linking to application and motivation)
% 3. this problem is hard to solve-->challenges. 
% 4. insight of the paper (how to solve.)


With the proliferation of tracking facilities involving mobile phones and tracking technologies involving GPS, a large amount of \emph{trajectory} data is being generated by moving objects. Such large amount of trajectory data provides us a chance to investigate rich information contained in them. Existing studies have mined the traffic patterns~\cite{lippi2010collective}, how to operate the taxis via a good pattern~\cite{li2011hunting, liu2010uncovering}, and the hot locations of the cities~\cite{chang2010context, zheng2009mining} from the trajectory data, which helps taxis drivers pick up passengers in a high probability and helps passengers save waiting time. 



\begin{figure}
  \centering
  \includegraphics[width=0.8\linewidth, height=0.5\linewidth]{figures/example}
  \caption{$T_1$, $T_2$ and $T_3$ are three map-matched trajectories under $e_1$ (source) and $e_{10}$ (destination). %Assuming the starting travel times of $T_1$, $T_2$ and $T_3$ are 9:00, 17:00, and 9:10, and thus $T_1$ and $T_3$ are in the same group (denoted by Group-1) because they are within the same time slot with one hour granularity, and $T_2$ is in the other group (denoted by Group-2).
  }
  \label{fig:example}
  \vspace{-5mm}
\end{figure}

An \emph{outlier} is an object that is different from or inconsistent with the remaining objects~\cite{han2006concepts}. In our context, a trajectory outlier or an anomalous trajectory refers to a trajectory that is different from the majority trajectories for a given source and destination~\cite{chen2011real, chen2013iboat} which can be described as occurring sparsely comparing the majority trajectories for a given source and destination. For the problem of detecting anomalous trajectories, each trajectory has a source and destination pair, put it differently, SD pair in the following context. We present an example in figure~\ref{fig:example}. We note that there are three map-matched trajectories from $S$ to the destination $D$. We note that the trajectory $T_3$ is anomalous with respect to the SD pair $<S, D>$ (i.e., $<e_1, e_{10}>$) since it does not follow the normal route followed by the trajectory $T_1$ and $T_2$, which is different from the majority trajectories following the same route representing with blue colour and green colour from $e_1$ to $e_{10}$. As mentioned before, detecting anomalous trajectories has attracted much attention and many approaches~\cite{zhang2020continuous, liu2020online,zhang2011ibat, chen2013iboat, wu2017fast} have been proposed for it, while most of them aim to discriminate whether a target trajectory is anomalous or not and fail to solve \textbf{which part of a trajectory (i.e., subtrajectory) is anomalous?}, which is a non-trivial and meaningful problem. We give an application to present the importance and motivation of detecting anomalous \textbf{sub}trajectories. 

\emph{Example:} In order to overcharge on a certain trip from a passenger and earn unusual money, some taxi drivers deliberately perform unnecessary detours, while passengers usually fail to find out in time, especially for those who are not familiar with routes of cities. Real-time anomalous trajectory detection makes it possible for passengers to detect whether the route is normal or anomalous taken by drivers timely and helps taxi companies to monitor fraud behaviours of dishonest drivers. This could improve the quality of taxi services. There are currently three studies to detect anomalous subtrajectories.~\citet{lee2008trajectory} proposes to partition the trajectories and detect the anomalous subtrajectories by computing the distance of each segment in a detected trajectory to the segments in other trajectories, which is offline and cannot detect the anomalous subtrajectories in real-time manner. ~\citet{chen2013iboat} proposes to detect anomalous subtrajectories in online manner with the isolation-based method, which aims to check which parts of a detected trajectory that can be isolated from the reference (i.e., normal) trajectories with the same source and destination routes. ~\citet{zhang2020continuous} proposes to monitor the trajectory similarity based on discrete Frechet distance between a given reference route and the current partial route at each timestamp. If the deviation threshold exceeds a given threshold at any timestamp, and the system alerts that an outlier event of detouring is detected. These studies are hand-crafted heuristic with many predefined parameters (e.g., the deviation threshold) for detecting anomalous subtrajectories and time-consuming. 


Therefore, detecting anomalous subtrajectories effectively via online manner is a non-trival task and there are the following challenging issues:

\vspace{-\topsep}
% [leftmargin=*]
\begin{itemize}[leftmargin=*]

\item \textbf{Lack of labelled data.} The anomalousness is extremely hard to be defined by simple rules, while manually labeling large-scale subtrajectories costs unaffordable human effort. This obstructs some straightforward data-intensive methods to be applied for this problem. {\color{blue}{For example, ~\citet{chen2013iboat} propose to detect anomalous subtrajectories in online manner with the isolation-based method on a small manually dataset with 9 SD pairs with the average number little over 1000 for each SD pair. Put it differently, the manually test set in~\cite{chen2013iboat} is so small that the evaluation results cannot reflect the performance accurately and directly}}. 
\item \textbf{Subtrajectory modeling}. {\Comment{The detection of anomalous subtrajectories relies heavily on modeling the characteristics involving complexity, variety, and the uniqueness, of subtrajectories on different routes effectively and efficiently}}, which is a challenging task and hardly handled by manually defined heuristic parameters. Moreover, the mobility on urban space usually happens on road networks, which would have a significant impact on the appearance of subtrajectory anomalies and make the problem even more challenging. {\Comment{Also, predefined heuristic parameters of modeling subtrajectories are hardly adaptive to different applications. As we mention before, a small manually dataset with the anomalous rate is 5.1\%, which is largely higher than the anomalous rate of datasets in this paper (Chengdu:0.7\% and Xi'an: 1.5\%) is utilized in experiments in~\cite{chen2013iboat}. According to the experiment results (Table $\uppercase\expandafter{\romannumeral2}$) in ~\cite{chen2013iboat}, iBOAT can achieve a good performance on detecting anomalous subtrajectopries. Nevertheless, we adapt it to our datasets with \textbf{1,688} (resp.\textbf{1,057}) \emph{SD pairs}, which corresponds to \textbf{558,098} (resp. \textbf{163,027}) raw trajectories before map-matching for Chengdu (resp. Xi’an). The performance of iBOAT proposed in ~\cite{chen2013iboat} is around 40\% lower than our method RL4OASD.
% on the whole manually labelled test datasets of Chengdu and Xi'an. 
Thus, heuristic methods are hardly adaptive to different applications such as the varied anomalous rate, the varied datasize and so on.}}
\item \textbf{Efficient online detection}. As trajectories are often generated at a very high speed, detection efficiency is also a central concern. For example, taxi trajectories involving 790 million GPS points~\cite{yuan2011driving, yuan2010t} are generated in Beijing in 3 months. {\Comment{The average time interval of sampling is 3.1 minutes per point and the average distance of two consecutively sampling points is around 600 meters. There are 4.96 million trajectories after data preprocessing~\cite{yuan2011driving, yuan2010t}}}. In addition, the number of subtrajectories is several orders of magnitude larger than the number of trajectories. For example, there are over {\color{red}{20 million}} subtrajectories with respect to 4.96 million trajectories~\cite{yuan2011driving, yuan2010t} after map-matching~\cite{yang2018fast}. Thus, conventional offline detection methods that often need to enumerate all the subtrajectories are clearly infeasible. To avoid this, an optimal solution must enable \emph{online detection}, where the anomalousness can be revealed while a trajectory is being generated.

% there is a paper using non-labelled data and achieve good results, but then if we increase the dataset size, it's performance drops a bit, I think we should include this point in the introduction


% The detection of anomalous subtrajectory heavily relies on understanding the mobility patterns of subtrajectories. This is a challenging task, as the complexity and variety of subtrajectories across different places can hardly be modeled by simple heuristics. Moreover, the mobility on urban space usually happens on road networks, which would have a significant impact on the appearance of subtrajectory anomalies and make the problem even more challenging.

\end{itemize}
\vspace{-\topsep}


\noindent In this paper, {\Comment{we propose a novel reinforcement learning based solution RL4OASD to address above three challenges. RL4OASD consists of three parts, namely data preprocessing, RSRNet and ASDNet. \emph{\textbf{First}}, we obtain map-matched trajectories via map-matching the raw trajectories on road networks during data preprocessing period. The map-matched trajectory is in the form of a sequence of road segments. We then design a noisy labeling method to label each road segment as 0 representing normal and 1 otherwise, by counting each transition frequency from historical trajectories. \textbf{During training process}, the noisy labels are used to train the Road Segment Representation Network (RSRNet). Also, in order to improve the effectiveness of RL4OASD, we model the detecting anomalous subtrajectories as a Markov decision process~\cite{puterman2014markov} named Anomalous Subtrajectory Detection Network (ASDNet). And ASDNet can be trained jointly with SRNet, in a weakly supervised manner using noisy labeled data. The two networks can mutually refine each other, where SRNet can provide expressive sequential information behind trajectories for ASDNet to detect, and ASDNet can offer supervision for SRNet to better learn the characteristics of subtrajectories. \textbf{During test period}, RL4OASD perform testing on \textbf{manually labelled test data}. In this way, we address the first challenge effectively.  
\emph{\textbf{Second}}, SRNet, which exploits road network representation learning and deep sequence modeling techniques that jointly model the \emph{characteristics} underlying subtrajectories, which addresses the second challenge. 
\emph{\textbf{Third}}, a novel detection algorithm, namely RL4OASD, which leverages the learned policy and enables online detection of anomalous subtrajectories, which addresses the third challenge.}}
% \vspace{-\topsep}
% \begin{itemize}[leftmargin=*]
% \item {\color{blue}{\textbf{}

% In RSRNet, we infer the normal routes behind a detected trajectory and train the embeddings of road segments of the trajectory. Those embeddings are fed into the Anomalous Subtrajectory Detection Network (ASDNet) as the state, to provide observations for labeling anomalous subtrajectories. We implement the RSRNet with RNN, which is able to capture the sequential information of trajectories (Section 4.3). In ASDNet, we build a road network enhanced environment for
% labeling each road segment as normal or not. The task is modeled as a Markov decision process [25], whose policies are learned via a policy gradient method [26] (Section 4.4). Note that the ASDNet outputs refined labels of road segments,
% which are further used to train RSRNet again, and then RSRNet provides better observations for ASDNet to train better policies.
 
% For the second challenge, we propose Anomalous Subtrajectory Detection Network (ASDNet), which is a policy network that is tailored for the detection of subtrajectories on road networks. ASDNet can be trained jointly with SRNet, in a weakly supervised manner using noisy labeled data. The two networks can mutually refine each other, where SRNet can provide expressive sequential information behind trajectories for ASDNet to detect, and ASDNet can offer supervision for SRNet to better learn the mobility patterns.


% \textbf{Setting noise labels and ASDNet is proposed to refined noise labels during training period}. 
% We firstly calculate the transition probability of each route segment after map-matching for each $<S,D>$ pair. We then set a threshold and if the probability of the route segment $r_i$ is larger than the threshold, we labelled the route segment $r_i$ as 0 otherwise as 1. In this way, we obtain the noise labels. Then we propose Anomalous Subtrajectory Detection Network (ASDNet), which is a policy network that is tailored for the detection of subtrajectories on road networks. ASDNet can be trained jointly with SRNet, in a weakly supervised manner using \textbf{noisy labelled data}. The two networks can mutually refine each other, where SRNet can provide expressive sequential information behind trajectories for ASDNet to detect, and ASDNet can offer supervision for SRNet to better learn the mobility patterns. For testing, we \textbf{manulaly labelled} totally label \textbf{1,688} (resp. \textbf{1,057}) unique routes, which correspond to \textbf{558,098} (resp. \textbf{163,027}) raw trajectories before map-matching for Chengdu (resp. Xi’an). 

% \item \textbf{}
% For the third challenge, we propose a novel detection algorithm, namely RL4OASD, which leverages the learned policy and enables online detection of anomalous subtrajectories. 
% % \textbf{Learned policy of RL4OASD for detecting anomalous subtrajectories effectively and efficiently}. 
% % In order to detect anomalous subtrajectories efficiently via an online manner, we propose a novel detection algorithm, namely RL4OASD, which leverages the learned policy during training process and enables online detection of anomalous subtrajectories effectively and efficiently.
% \item \textbf{} For the first challenge, we propose Road Segment Representation Network (SRNet), which exploits road network representation learning and deep sequence modeling techniques that jointly model the mobility pattern underlying subtrajectories.     }}
% \end{itemize}
% \vspace{-\topsep}

\noindent Our contributions can be summarized as follows:
\vspace{-\topsep}
\begin{itemize}[leftmargin=*]
    \item We propose the first deep reinforcement learning based solution to detect anomalous subtrajectories. The
    % information of trajectory
    proposed model 1) integrates the {\color{blue}{characteristics of subtrajectories}} and road network structure, and 2) can be trained with limited labeled data.
    \item We propose a novel detection paradigm based on the learned policy, which allows the anomalous subtrajectory detection to be efficiently conducted in an online manner.
    \item We conduct extensive experiments on two real-world trajectory datasets with \textbf{manually-labelled test data}. We compare our proposed solution with various baselines, and the results show that our solution can significantly outperform the state-of-the-art methods and is efficient for online anomalous subtrajectory detection.
\end{itemize}
\vspace{-\topsep}



% 1. emphasis this problem important
% 2. important (linking to application and motivation)
% 3. this problem is hard to solve-->challenges. 
% 4. insight of the paper (how to solve.)



















































==> introduction3.tex <==
\section{INTRODUCTION}
\label{sec:introduction}
% 1. emphasis this problem important
% 2. important (linking to application and motivation)
% 3. this problem is hard to solve-->challenges. 
% 4. insight of the paper (how to solve.)


With the proliferation of tracking facilities involving mobile phones and tracking technologies involving GPS, a large amount of \emph{trajectory} data is being generated by moving objects. Such a large amount of trajectory data provides us with a chance to investigate rich information contained in them. {\Comment{Existing studies have mined the traffic patterns~\cite{lippi2010collective}, co-movement patterns~\cite{fan2016general,tritsarolis2021online}, trajectory similarity search~\cite{tritsarolis2021online, tiakas2006trajectory, pelekis2007similarity} and next location prediction~\cite{yang2017neural}.}}
% how to operate the taxis via a good pattern~\cite{li2011hunting, liu2010uncovering}, and the hot locations of the cities~\cite{chang2010context, zheng2009mining} from the trajectory data, which helps taxis drivers pick up passengers in a high probability and helps passengers save waiting time. 



\begin{figure}
  \centering
  \includegraphics[width=0.8\linewidth, height=0.5\linewidth]{figures/example}
  \caption{$T_1$, $T_2$ and $T_3$ are three map-matched trajectories under $e_1$ (source) and $e_{10}$ (destination). %Assuming the starting travel times of $T_1$, $T_2$ and $T_3$ are 9:00, 17:00, and 9:10, and thus $T_1$ and $T_3$ are in the same group (denoted by Group-1) because they are within the same time slot with one hour granularity, and $T_2$ is in the other group (denoted by Group-2).
  }
  \label{fig:example}
  \vspace{-5mm}
\end{figure}


An \emph{outlier} is an object that is different from or inconsistent with the remaining objects~\cite{han2006concepts}. In our context, a trajectory outlier or an anomalous trajectory refers to a trajectory that is different from the majority trajectories for a given source and destination~\cite{chen2011real, chen2013iboat} which can be described as occurring sparsely comparing the majority trajectories for a given source and destination. For the problem of detecting anomalous trajectories, each trajectory has a source and destination pair, put it differently, SD pair in the following context. We present an example in figure~\ref{fig:example}. We note that there are three map-matched trajectories from $S$ to the destination $D$. We note that the trajectory $T_3$ is anomalous with respect to the SD pair $<S, D>$ (i.e., $<e_1, e_{10}>$) since it does not follow the normal route followed by the trajectory $T_1$ and $T_2$, which is different from the majority trajectories following the same route representing with blue colour and green colour from $e_1$ to $e_{10}$. As mentioned before, detecting anomalous trajectories has attracted much attention and many approaches~\cite{zhang2020continuous, liu2020online,zhang2011ibat, chen2013iboat, wu2017fast} have been proposed for it, while most of them aim to discriminate whether a target trajectory is anomalous or not and fail to solve \textbf{which part of a trajectory (i.e., subtrajectory) is anomalous?}, which is a non-trivial and meaningful problem. In real-world applications, trajectories are usually long sequences with many subtrajectories. Identifying anomalous subtrajectories is a necessity to accurately locate and indicate the anomalousness, which is crucial for the corresponding actions to be timely taken.
For example, a ride-haling company can take different measures based on where the detour is occurred and how long it lasts.
% We give an application to present the importance and motivation of detecting anomalous \textbf{sub}trajectories. 


% \emph{Example:} In order to overcharge on a certain trip from a passenger and earn unusual money, some taxi drivers deliberately perform unnecessary detours, while passengers usually fail to find out in time, especially for those who are not familiar with routes of cities. Real-time anomalous trajectory detection makes it possible for passengers to detect whether the route is normal or anomalous taken by drivers timely and helps taxi companies to monitor fraud behaviours of dishonest drivers. This could improve the quality of taxi services.

% There are currently three studies to detect anomalous subtrajectories.~\citet{lee2008trajectory} proposes to partition the trajectories and detect the anomalous subtrajectories by computing the distance of each segment in a detected trajectory to the segments in other trajectories, which is offline and cannot detect the anomalous subtrajectories in real-time manner. ~\citet{chen2013iboat} proposes to detect anomalous subtrajectories in online manner with the isolation-based method, which aims to check which parts of a detected trajectory that can be isolated from the reference (i.e., normal) trajectories with the same source and destination routes. ~\citet{zhang2020continuous} proposes to monitor the trajectory similarity based on discrete Frechet distance between a given reference route and the current partial route at each timestamp. If the deviation threshold exceeds a given threshold at any timestamp, and the system alerts that an outlier event of detouring is detected. These studies are hand-crafted heuristic with many predefined parameters (e.g., the deviation threshold) for detecting anomalous subtrajectories and time-consuming. 


Therefore, detecting anomalous subtrajectories effectively via online manner is a non-trival task and there are the following challenging issues:

\vspace{-\topsep}
% [leftmargin=*]
\begin{itemize}[leftmargin=*]

\item \textbf{Lack of labelled data.} The anomalousness is extremely hard to be defined by simple rules, while manually labeling large-scale subtrajectories costs unaffordable human effort. This obstructs some straightforward data-intensive methods to be applied for this problem. {\color{blue}{For example, ~\citet{chen2013iboat} propose to detect anomalous subtrajectories in an online manner with the isolation-based method on a small manually dataset with 9 SD pairs and there are about 1000 trajectories for each SD pair.% with the average length little over 1000 for each SD pair. 
Put it differently, the manually test set in~\cite{chen2013iboat} is so small that the evaluation results cannot reflect the performance accurately and directly}}. 
\item \textbf{Subtrajectory modeling}. {\Comment{The detection of anomalous subtrajectories relies heavily on modeling the characteristics involving complexity, variety, and the uniqueness, of subtrajectories on different routes effectively and efficiently}}, which is a challenging task and hardly handled by manually defined heuristic parameters. Moreover, the mobility on urban space usually happens on road networks, which would have a significant impact on the appearance of subtrajectory anomalies and make the problem even more challenging. {\Comment{Also, predefined heuristic parameters of modeling subtrajectories are hardly adaptive to different applications. As shown in our experiments, we utilize iBOAT on our datasets with \textbf{1,688} ( resp.\textbf{1,057}) \emph{SD pairs}, which corresponds to \textbf{558,098} (resp. \textbf{163,027}) raw trajectories for Chengdu (resp. Xi’an). The performance of iBOAT proposed in ~\cite{chen2013iboat} is around 40\% lower than our method RL4OASD. Thus, heuristic methods are hardly adaptive to different applications such as the varied datasize, the varied anomalous rate and so on.}}


% As we mention before, a small manually dataset with the anomalous rate is 5.1\%, which is largely higher than the anomalous rate of datasets in this paper (Chengdu:0.7\% and Xi'an: 1.5\%) is utilized in experiments in~\cite{chen2013iboat}. According to the experiment results (Table $\uppercase\expandafter{\romannumeral2}$) in ~\cite{chen2013iboat}, iBOAT can achieve a good performance on detecting anomalous subtrajectopries. Nevertheless, we adapt it to our datasets with \textbf{1,688} (resp.\textbf{1,057}) \emph{SD pairs}, which corresponds to \textbf{558,098} (resp. \textbf{163,027}) raw trajectories before map-matching for Chengdu (resp. Xi’an). The performance of iBOAT proposed in ~\cite{chen2013iboat} is around 40\% lower than our method RL4OASD.
% on the whole manually labelled test datasets of Chengdu and Xi'an. 

\item \textbf{Efficient online detection}. As trajectories are often generated at a very high speed, detection efficiency is also a central concern. For example, taxi trajectories involving 790 million GPS points~\cite{yuan2011driving, yuan2010t} are generated in Beijing in 3 months. {\Comment{There are 4.96 million trajectories generated in 3 months after data preprocessing~\cite{yuan2011driving, yuan2010t}}}. In addition, the number of subtrajectories is several orders of magnitude larger than the number of trajectories. For example, there are over {\color{red}{20 million}} subtrajectories with respect to 4.96 million trajectories~\cite{yuan2011driving, yuan2010t} after map-matching~\cite{yang2018fast}. Thus, an optimal solution must enable \emph{online detection}, where the anomalousness can be revealed while a trajectory is being generated.
% Thus, conventional offline detection methods that often need to enumerate all the subtrajectories are clearly infeasible. 


% The average time interval of sampling is 3.1 minutes per point and the average distance of two consecutively sampling points is around 600 meters. 


% there is a paper using non-labelled data and achieve good results, but then if we increase the dataset size, it's performance drops a bit, I think we should include this point in the introduction


% The detection of anomalous subtrajectory heavily relies on understanding the mobility patterns of subtrajectories. This is a challenging task, as the complexity and variety of subtrajectories across different places can hardly be modeled by simple heuristics. Moreover, the mobility on urban space usually happens on road networks, which would have a significant impact on the appearance of subtrajectory anomalies and make the problem even more challenging.

\end{itemize}
\vspace{-\topsep}


\noindent However, existing studies fail to solve three above challenges.~\citet{lee2008trajectory} proposes to partition the trajectories and detect the anomalous subtrajectories by computing the distance of each segment in a detected trajectory to the segments in other trajectories, which is offline and cannot detect the anomalous subtrajectories in real-time manner. ~\citet{chen2013iboat} proposes to detect anomalous subtrajectories in online manner with the isolation-based method, which aims to check which parts of a detected trajectory that can be isolated from the reference (i.e., normal) trajectories with the same source and destination routes, which fail to generalize in many real applications. ~\citet{zhang2020continuous} proposes to monitor the trajectory similarity based on discrete Frechet distance between a given reference route and the current partial route at each timestamp. If the deviation threshold exceeds a given threshold at any timestamp, and the system alerts that an outlier event of detouring is detected, which fail to slove the second challenge. These studies are hand-crafted heuristic with many predefined parameters (e.g., the deviation threshold) for detecting anomalous subtrajectories and time-consuming, and faile to solve above challenges.


\noindent In this paper, {\Comment{we propose a novel reinforcement learning based solution RL4OASD to address above three challenges. RL4OASD consists of three parts, namely data preprocessing, RSRNet and ASDNet. \emph{\textbf{First}}, we obtain map-matched trajectories via map-matching the raw trajectories on road networks during data preprocessing period. The map-matched trajectory is in the form of a sequence of road segments. We then design a noisy labeling method to label each road segment as 0 representing normal and 1 otherwise, by counting each transition frequency from historical trajectories. \textbf{During training process}, the noisy labels are used to train the Road Segment Representation Network (RSRNet). Also, in order to improve the effectiveness of RL4OASD, we model the detecting anomalous subtrajectories as a Markov decision process~\cite{puterman2014markov} named Anomalous Subtrajectory Detection Network (ASDNet). And ASDNet can be trained jointly with SRNet, in a weakly supervised manner using noisy labeled data. The two networks can mutually refine each other, where SRNet can provide expressive sequential information behind trajectories for ASDNet to detect, and ASDNet can offer supervision for SRNet to better learn the characteristics of subtrajectories. \textbf{During test period}, RL4OASD perform testing on \textbf{manually labelled test data}. In this way, we address the first challenge effectively.  
\emph{\textbf{Second}}, SRNet, which exploits road network representation learning and deep sequence modeling techniques that jointly model the \emph{characteristics} underlying subtrajectories, which addresses the second challenge. 
\emph{\textbf{Third}}, a novel detection algorithm, namely RL4OASD, which leverages the learned policy and enables online detection of anomalous subtrajectories, which addresses the third challenge.}}
% \vspace{-\topsep}
% \begin{itemize}[leftmargin=*]
% \item {\color{blue}{\textbf{}

% In RSRNet, we infer the normal routes behind a detected trajectory and train the embeddings of road segments of the trajectory. Those embeddings are fed into the Anomalous Subtrajectory Detection Network (ASDNet) as the state, to provide observations for labeling anomalous subtrajectories. We implement the RSRNet with RNN, which is able to capture the sequential information of trajectories (Section 4.3). In ASDNet, we build a road network enhanced environment for
% labeling each road segment as normal or not. The task is modeled as a Markov decision process [25], whose policies are learned via a policy gradient method [26] (Section 4.4). Note that the ASDNet outputs refined labels of road segments,
% which are further used to train RSRNet again, and then RSRNet provides better observations for ASDNet to train better policies.
 
% For the second challenge, we propose Anomalous Subtrajectory Detection Network (ASDNet), which is a policy network that is tailored for the detection of subtrajectories on road networks. ASDNet can be trained jointly with SRNet, in a weakly supervised manner using noisy labeled data. The two networks can mutually refine each other, where SRNet can provide expressive sequential information behind trajectories for ASDNet to detect, and ASDNet can offer supervision for SRNet to better learn the mobility patterns.


% \textbf{Setting noise labels and ASDNet is proposed to refined noise labels during training period}. 
% We firstly calculate the transition probability of each route segment after map-matching for each $<S,D>$ pair. We then set a threshold and if the probability of the route segment $r_i$ is larger than the threshold, we labelled the route segment $r_i$ as 0 otherwise as 1. In this way, we obtain the noise labels. Then we propose Anomalous Subtrajectory Detection Network (ASDNet), which is a policy network that is tailored for the detection of subtrajectories on road networks. ASDNet can be trained jointly with SRNet, in a weakly supervised manner using \textbf{noisy labelled data}. The two networks can mutually refine each other, where SRNet can provide expressive sequential information behind trajectories for ASDNet to detect, and ASDNet can offer supervision for SRNet to better learn the mobility patterns. For testing, we \textbf{manulaly labelled} totally label \textbf{1,688} (resp. \textbf{1,057}) unique routes, which correspond to \textbf{558,098} (resp. \textbf{163,027}) raw trajectories before map-matching for Chengdu (resp. Xi’an). 

% \item \textbf{}
% For the third challenge, we propose a novel detection algorithm, namely RL4OASD, which leverages the learned policy and enables online detection of anomalous subtrajectories. 
% % \textbf{Learned policy of RL4OASD for detecting anomalous subtrajectories effectively and efficiently}. 
% % In order to detect anomalous subtrajectories efficiently via an online manner, we propose a novel detection algorithm, namely RL4OASD, which leverages the learned policy during training process and enables online detection of anomalous subtrajectories effectively and efficiently.
% \item \textbf{} For the first challenge, we propose Road Segment Representation Network (SRNet), which exploits road network representation learning and deep sequence modeling techniques that jointly model the mobility pattern underlying subtrajectories.     }}
% \end{itemize}
% \vspace{-\topsep}

\noindent Our contributions can be summarized as follows:
\vspace{-\topsep}
\begin{itemize}[leftmargin=*]
    \item We propose the first deep reinforcement learning based solution to detect anomalous subtrajectories. The
    % information of trajectory
    proposed model 1) integrates the {\color{blue}{characteristics of subtrajectories}} and road network structure, and 2) can be trained with limited labeled data.
    \item We propose a novel detection paradigm based on the learned policy, which allows the anomalous subtrajectory detection to be efficiently conducted in an online manner.
    \item We conduct extensive experiments on two real-world trajectory datasets with \textbf{manually-labelled test data}. We compare our proposed solution with various baselines, and the results show that our solution can significantly outperform the state-of-the-art methods and is efficient for online anomalous subtrajectory detection.
\end{itemize}
\vspace{-\topsep}



% 1. emphasis this problem important
% 2. important (linking to application and motivation)
% 3. this problem is hard to solve-->challenges. 
% 4. insight of the paper (how to solve.)



















































==> introduction4.tex <==
\section{INTRODUCTION}
\label{sec:introduction}
% 1. emphasis this problem important
% 2. important (linking to application and motivation)
% 3. this problem is hard to solve-->challenges. 
% 4. insight of the paper (how to solve.)

With the advancement of mobile computing and geographical positioning techniques, massive spatial trajectory data is being generated by various moving objects (\eg, people, vehicles) in spatial spaces, such as GPS devices and smart phones. Such collected trajectory data records the mobility traces of moving objects at different timestamps, which reflects the diverse mobility patterns of objects. Accurate spatial trajectory data analysis serves as the key technical component for a wide spectrum of spatial-temporal applications, including intelligent transportation~\cite{yuan2021effective}, location-based recommendation service~\cite{feng2020hme}, pandemic tracking~\cite{seemann2020tracking}, and criminal prevention for public safety~\cite{2018deepcrime}.

% With the proliferation of tracking facilities involving mobile phones and tracking technologies involving GPS, a large amount of \emph{trajectory} data is being generated by moving objects. These trajectory datasets provide us an opportunity to identify important information for useful location-based applications. Existing studies on such datasets have attempted to solve many problems including: mining the traffic patterns~\cite{lippi2010collective}, identifying co-movement objects~\cite{fan2016general,tritsarolis2021online}, conducting trajectory similarity search~\cite{tritsarolis2021online, tiakas2006trajectory, pelekis2007similarity} and predicting the next location of a moving object~\cite{yang2017neural}.

% how to operate the taxis via a good pattern~\cite{li2011hunting, liu2010uncovering}, and the hot locations of the cities~\cite{chang2010context, zheng2009mining} from the trajectory data, which helps taxis drivers pick up passengers in a high probability and helps passengers save waiting time.

Among various trajectory mining applications, detecting anomalous trajectories plays a vital role in many practical urban scenarios. For example, the real-time vehicle trajectory detection is beneficial for better traffic management by identifying the traffic anomalies (\eg, traffic jam and accidents) beforehand~\cite{yuan2018hetero}. Additionally, studying the mobility behaviors of humans for discovering their anomalous trajectories is helpful for predicting spatial event outliers (\eg, civil unrest and pandemic outbreaks)~\cite{ning2019spatio}. In such context, a trajectory anomaly refers to a trajectory which does not show the normal mobility patterns and deviates from the majority of the trajectories with the same source and destination~\cite{chen2011real, chen2013iboat}.

An \emph{anomaly} is an object that is different from or inconsistent with the remaining objects~\cite{han2006concepts}. In our context, a trajectory anomaly or an anomalous trajectory refers to a trajectory that is different from the majority of the trajectories with the same source and destination~\cite{chen2011real, chen2013iboat}.
% which can be described as occurring sparsely when compared to the majority trajectories for a given source and destination. 
Recently, detecting anomalous trajectories has attracted much attention, and many approaches~(\eg, \cite{zhang2020continuous, liu2020online,zhang2011ibat, chen2013iboat, wu2017fast}) have been proposed for solving this problem.
In the following, we assume that each trajectory has a source and destination pair, referred as an SD pair. Consider the example in Figure~\ref{fig:example}. There are three trajectories from the source $S  (e_1)$ to the destination $D (e_{10})$. The trajectory $T_3$ (the red one) is considered as anomalous with respect to the SD pair $<S, D>$ if the majority of the trajectories with the same SD pair follow either $T_1$ (the blue one) or $T_2$ (the green one). Most of the existing approaches{\Revision{~\cite{chen2013iboat,zhang2020continuous,wu2017fast,liu2020online}}} are designed to decide whether a target trajectory is anomalous or not, but they are not able to provide information of \textbf{which part of the trajectory (\emph{subtrajectory}) is anomalous in a timely manner}, which is critical for a number of real-world applications. For instance, a ride-hailing company could immediately spot a driver when the trajectory starts to deviate from a normal route, or provide an alert to a passenger. Other potential applications include elderly care, especially for those who suffer from Alzheimer or child custody in countries with high kidnapping rates. {\Revision{For example, many seniors require constant monitoring to support their daily life, but such care is expensive, and generally processes in an automatic way by monitoring anomalies that occur in their trajectories. When they go outside and some anomalies are detected (e.g., taking a wrong bus), if their families could be notified in time with the accurate mobile localization, immediate and possible lifesaving actions can be taken accordingly. In addition, the subtrajectory detection enables the detection in a finer-grained way than the conventional trajectory anomaly detection task, i.e., it reveals which parts are responsible for the anomalies. This would be helpful for taking prompt and accurate actions against the anomalies in real-world scenarios.}}

\begin{figure}
  \centering
  \includegraphics[width=0.68\linewidth]{figures/example2}
  \caption{$T_1$, $T_2$ and $T_3$ are three trajectories from the same source $e_1$ to the same destination $e_{10}$. %Assuming the starting travel times of $T_1$, $T_2$ and $T_3$ are 9:00, 17:00, and 9:10, and thus $T_1$ and $T_3$ are in the same group (denoted by Group-1) because they are within the same time slot with one hour granularity, and $T_2$ is in the other group (denoted by Group-2).
  }
  \label{fig:example}
  \vspace{-5mm}
\end{figure}
%The trajectories are usually long sequences with many subtrajectories. Identifying anomalous subtrajectories is a necessity to accurately locate and indicate the anomalousness, which is crucial for the corresponding actions to be timely taken.
%For example, a ride-haling company can take different measures based on where the detour is occurred and how long it lasts.
% We give an application to present the importance and motivation of detecting anomalous \textbf{sub}trajectories. 

% \emph{Example:} In order to overcharge on a certain trip from a passenger and earn unusual money, some taxi drivers deliberately perform unnecessary detours, while passengers usually fail to find out in time, especially for those who are not familiar with routes of cities. Real-time anomalous trajectory detection makes it possible for passengers to detect whether the route is normal or anomalous taken by drivers timely and helps taxi companies to monitor fraud behaviours of dishonest drivers. This could improve the quality of taxi services.

% There are currently three studies to detect anomalous subtrajectories.~\citet{lee2008trajectory} proposes to partition the trajectories and detect the anomalous subtrajectories by computing the distance of each segment in a detected trajectory to the segments in other trajectories, which is offline and cannot detect the anomalous subtrajectories in real-time manner. ~\citet{chen2013iboat} proposes to detect anomalous subtrajectories in online manner with the isolation-based method, which aims to check which parts of a detected trajectory that can be isolated from the reference (i.e., normal) trajectories with the same source and destination routes. ~\citet{zhang2020continuous} proposes to monitor the trajectory similarity based on discrete Frechet distance between a given reference route and the current partial route at each timestamp. If the deviation threshold exceeds a given threshold at any timestamp, and the system alerts that an outlier event of detouring is detected. These studies are hand-crafted heuristic with many predefined parameters (e.g., the deviation threshold) for detecting anomalous subtrajectories and time-consuming. 

Detecting anomalous subtrajectories effectively in a timely (online) manner is a non-trivial task with the following challenging issues:
% \vspace{5pt}
% \vspace{-\topsep}
% % [leftmargin=*]
% \begin{itemize}[leftmargin=*]
% \item 

(1) \textbf{Lack of labeled data.} 
%The anomalousness is hard to define by simple rules,
{\Revision{It is challenging to capture anomalous information behind trajectories without labeled data, and the anomalousness is hard to define by simple rules due to variable and complex traffic condition.}} Yet, manually labeling large-scale subtrajectories would cost unaffordable human effort. This obstructs some straightforward data-intensive methods to be applied for this problem. As far as we know, 
{\Comment{the only manually labeled dataset available (used in Chen et al.~\cite{chen2013iboat}) contains only 9 SD pairs with about 1,000}} trajectories. Using a small dataset cannot provide accurate information on the performance of an approach in a real application. 
%propose to detect anomalous subtrajectories in an online manner with the isolation-based method on a small manually dataset with 9 SD pairs and there are about 1000 trajectories for each SD pair.% with the average length little over 1000 for each SD pair. 
%Put it differently, the manually test set in~\cite{chen2013iboat} is so small that the evaluation results cannot reflect the performance accurately and directly}}. 
% \vspace{5pt}
% \item 

{\Revision{(2) \textbf{Complex subtrajectory modeling.} Existing approaches for modeling anomalous subtrajectories follow one of the following strategies. The first approach~\cite{chen2013iboat} is to use some manually defined parameters to isolate an anomalous subtrajectory. It maintains an adaptive window of the latest incoming GPS points to compare against normal trajectories, where the normal trajectories are supported by the majority of the trajectories within an SD pair. When a new point arrives, it will be added to the window as long as the support of the subtrajectory in the window is larger than a pre-defined threshold; otherwise, the adaptive window is reduced to contain only the latest point, and the process continues. However, the threshold is hard to set appropriately, and not general enough to cover all possible situations or adaptive to different road conditions.
%
The second approach~\cite{zhang2020continuous} is to use a density-based method. It follows some pre-defined rules to partition all trajectories within an SD pair into many subtrajectories, and the anomalous subtrajectories are recognized via computing the distance of each subtrajectory in a detected trajectory to the subtrajectories in other trajectories. It is clear that the detection needs to go through the whole trajectory, and cannot be done in an online manner. The most promising approach is the learning-based method~\cite{liu2020online, wu2017fast}, however, all proposed learning-based methods can only be applied to answer whether a given trajectory is anomalous or not but cannot detect anomalous subtrajectories. A possible reason is due to the lack of labeled data for anomalous subtrajectories.}}

\if 0
(2) \textbf{Complex subtrajectory modeling.} Existing approaches for modeling anomalous subtrajectories follow one of the following strategies. The first approach~\cite{chen2013iboat} is to use a set of manually defined parameters to characterize an anomalous subtrajectory. Due to the limited amount of labeled data, a fixed set of parameters is not general enough to cover all possible situations or adaptive to different road conditions. The second approach~\cite{zhang2020continuous} is to use a distance-based measure to differentiate anomalous trajectories from normal ones, i.e., when the deviation of the current partial route from a normal route exceeds a certain threshold, it reports a detouring event. First, the threshold is hard to set appropriately. Second, this is an indirect measure for anomalous subtrajectories. {\Revision{This method detects anomalous trajectories via calculating the trajectory similarity by discrete Frechet distance between a given reference route and the current partial route at each timestamp. Thus, the method is time-consuming and it is not clear whether the detection can be done in a timely manner.}} The most promising approach is the learning-based method~\cite{liu2020online, wu2017fast}, however, all proposed learning-based methods can only be applied to answer whether a given trajectory is anomalous or not but cannot detect anomalous subtrajectories. A possible reason is due to the lack of labeled data for anomalous subtrajectories.
\fi
%  is either based on heuristics, i.e., a large number of manually set parameters,   relies heavily on modeling the characteristics involving complexity, variety, and the uniqueness, of subtrajectories on different routes effectively and efficiently, which is a challenging task and hardly handled by manually defined heuristic parameters. Moreover, the mobility on urban space usually happens on road networks, which would have a significant impact on the appearance of subtrajectory anomalies and make the problem even more challenging. Also, predefined heuristic parameters of modeling subtrajectories are hardly adaptive to different applications. As shown in our experiments, we utilize iBOAT on our datasets with \textbf{1,688} ( resp.\textbf{1,057}) \emph{SD pairs}, which corresponds to \textbf{558,098} (resp. \textbf{163,027}) raw trajectories for Chengdu (resp. Xi’an). The performance of iBOAT proposed in ~\cite{chen2013iboat} is around 40\% lower than our method \texttt{RL4OASD}. Thus, heuristic methods are hardly adaptive to different applications such as the varied datasize, the varied anomalous rate and so on.
% As we mention before, a small manually dataset with the anomalous rate is 5.1\%, which is largely higher than the anomalous rate of datasets in this paper (Chengdu:0.7\% and Xi'an: 1.5\%) is utilized in experiments in~\cite{chen2013iboat}. According to the experiment results (Table $\uppercase\expandafter{\romannumeral2}$) in ~\cite{chen2013iboat}, iBOAT can achieve a good performance on detecting anomalous subtrajectopries. Nevertheless, we adapt it to our datasets with \textbf{1,688} (resp.\textbf{1,057}) \emph{SD pairs}, which corresponds to \textbf{558,098} (resp. \textbf{163,027}) raw trajectories before map-matching for Chengdu (resp. Xi’an). The performance of iBOAT proposed in ~\cite{chen2013iboat} is around 40\% lower than our method \texttt{RL4OASD}.
% on the whole manually labelled test datasets of Chengdu and Xi'an. 
% \vspace{5pt}
% \item 

(3) \textbf{Efficient online detection requirement.} Trajectories can be generated at a very high speed, and thus detection efficiency is a major concern. 
% For example, taxi trajectories with 790 million GPS points, involving about 5 million trajectories, can be generated in Beijing in 3 months~\cite{yuan2011driving, yuan2010t}. 
The number of subtrajectories is usually several orders of magnitude larger than the number of trajectories. In our example, there are over 1 billion subtrajectories corresponding to the 5 million trajectories. It is important to have a solution that can conduct \emph{online detection}, where the anomalousness can be revealed while a trajectory is being generated.

{\Revision{(4)  \textbf{Concept drift of anomalous trajectories.} 
The concept of anomalous trajectory might drift over time. For example, due to some varying traffic condition (e.g., some accident), the trajectory might gradually deviate from a normal route, and the concept of ``normal'' and ``anomalous'' is changed accordingly. Therefore, it is desirable to handle these changes and incorporate them into the model.}}
%There are 4.96 million trajectories generated in 3 months after data preprocessing~\cite{yuan2011driving, yuan2010t}. In addition, the number of subtrajectories is several orders of magnitude larger than the number of trajectories. For example, there are over {\color{red}{20 million}} subtrajectories with respect to 4.96 million trajectories~\cite{yuan2011driving, yuan2010t} after map-matching~\cite{yang2018fast}. Thus, an optimal solution must enable \emph{online detection}, where the anomalousness can be revealed while a trajectory is being generated.
% Thus, conventional offline detection methods that often need to enumerate all the subtrajectories are clearly infeasible. 


% The average time interval of sampling is 3.1 minutes per point and the average distance of two consecutively sampling points is around 600 meters. 


% there is a paper using non-labelled data and achieve good results, but then if we increase the dataset size, it's performance drops a bit, I think we should include this point in the introduction


% The detection of anomalous subtrajectory heavily relies on understanding the mobility patterns of subtrajectories. This is a challenging task, as the complexity and variety of subtrajectories across different places can hardly be modeled by simple heuristics. Moreover, the mobility on urban space usually happens on road networks, which would have a significant impact on the appearance of subtrajectory anomalies and make the problem even more challenging.

%\end{itemize}

%\vspace{-\topsep}
%\vspace{5pt}
%\noindent 
In summary, existing studies cannot address the aforementioned challenges simultaneously (more details of these studies can be found in Section~\ref{sec:related}). %
%However, existing studies fail to solve three above challenges.~\citet{lee2008trajectory} proposes to partition the trajectories and detect the anomalous subtrajectories by computing the distance of each segment in a detected trajectory to the segments in other trajectories, which is offline and cannot detect the anomalous subtrajectories in real-time manner. ~\citet{chen2013iboat} proposes to detect anomalous subtrajectories in online manner with the isolation-based method, which aims to check which parts of a detected trajectory that can be isolated from the reference (i.e., normal) trajectories with the same source and destination routes, which fail to generalize in many real applications. ~\citet{zhang2020continuous} proposes to monitor the trajectory similarity based on discrete Frechet distance between a given reference route and the current partial route at each timestamp. If the deviation threshold exceeds a given threshold at any timestamp, and the system alerts that an outlier event of detouring is detected, which fail to slove the second challenge. These studies are hand-crafted heuristic with many predefined parameters (e.g., the deviation threshold) for detecting anomalous subtrajectories and time-consuming, and faile to solve above challenges.
Therefore, in this paper, we propose a novel reinforcement learning based solution \texttt{RL4OASD} to address the challenges. \texttt{RL4OASD} consists of three parts, namely the data preprocessing, Road Segment Representation Network (RSRNet) and Anomalous Subtrajectory Detection Network (ASDNet). First, we obtain map-matched trajectories via map-matching the raw trajectories (GPS points) on road networks. The map-matched trajectory is in the form of a sequence of road segments. We then design a \emph{noisy labeling method} to label each road segment as 0 representing normal and 1 otherwise automatically, by counting each transition frequency from historical trajectories. {\Revision{This is the first step to address the challenge of the lack of labeled data, where the noisy labels are used to pre-train RSRNet as a warm-start, which outputs the road segment feature representations behind trajectories. Then, we model the detecting anomalous subtrajectories as a Markov Decision Process (MDP)~\cite{puterman2014markov} via ASDNet. 
%
Here, ASDNet is trained jointly with RSRNet in a weakly supervised manner. Specifically, the two networks can mutually refine each other, where RSRNet provides the representations for ASDNet to detect anomalies, and ASDNet refines the noisy labels using the current policy learned from MDP, and offers supervision of the refined labels for RSRNet to train 
better representations.}}
We emphasize that the noisy labels only provide some prior knowledge to address the cold-start problem of training the proposed model, but are not used to train the model as in a supervised paradigm.
%
During the testing period, \texttt{RL4OASD} performs testing on manually labeled test data. In this way, we do not require labeled data during training and hence we address the first challenge effectively.  

Second, RSRNet, which exploits road network representation learning and deep sequence modeling techniques that jointly model the \emph{characteristics} underlying subtrajectories, which addresses the second challenge. 
Third, a novel detection algorithm, which leverages the learned policy and enables online detection of anomalous subtrajectories, which addresses the third challenge. {\Revision{Fourth, our model can easily incorporate online learning strategy using the latest trajectory data to fine-tune the model, which addresses the fourth challenge.
}}

%\vspace{-\topsep}
% \begin{itemize}[leftmargin=*]
% \item {\color{blue}{\textbf{}
% In RSRNet, we infer the normal routes behind a detected trajectory and train the embeddings of road segments of the trajectory. Those embeddings are fed into the Anomalous Subtrajectory Detection Network (ASDNet) as the state, to provide observations for labeling anomalous subtrajectories. We implement the RSRNet with RNN, which is able to capture the sequential information of trajectories (Section 4.3). In ASDNet, we build a road network enhanced environment for
% labeling each road segment as normal or not. The task is modeled as a Markov decision process [25], whose policies are learned via a policy gradient method [26] (Section 4.4). Note that the ASDNet outputs refined labels of road segments,
% which are further used to train RSRNet again, and then RSRNet provides better observations for ASDNet to train better policies.
% For the second challenge, we propose Anomalous Subtrajectory Detection Network (ASDNet), which is a policy network that is tailored for the detection of subtrajectories on road networks. ASDNet can be trained jointly with RSRNet, in a weakly supervised manner using noisy labeled data. The two networks can mutually refine each other, where RSRNet can provide expressive sequential information behind trajectories for ASDNet to detect, and ASDNet can offer supervision for RSRNet to better learn the mobility patterns.
% \textbf{Setting noise labels and ASDNet is proposed to refined noise labels during training period}. 
% We firstly calculate the transition probability of each route segment after map-matching for each $<S,D>$ pair. We then set a threshold and if the probability of the route segment $r_i$ is larger than the threshold, we labelled the route segment $r_i$ as 0 otherwise as 1. In this way, we obtain the noise labels. Then we propose Anomalous Subtrajectory Detection Network (ASDNet), which is a policy network that is tailored for the detection of subtrajectories on road networks. ASDNet can be trained jointly with RSRNet, in a weakly supervised manner using \textbf{noisy labelled data}. The two networks can mutually refine each other, where RSRNet can provide expressive sequential information behind trajectories for ASDNet to detect, and ASDNet can offer supervision for RSRNet to better learn the mobility patterns. For testing, we \textbf{manulaly labelled} totally label \textbf{1,688} (resp. \textbf{1,057}) unique routes, which correspond to \textbf{558,098} (resp. \textbf{163,027}) raw trajectories before map-matching for Chengdu (resp. Xi’an). 
% \item \textbf{}
% For the third challenge, we propose a novel detection algorithm, namely \texttt{RL4OASD}, which leverages the learned policy and enables online detection of anomalous subtrajectories. 
% % \textbf{Learned policy of \texttt{RL4OASD} for detecting anomalous subtrajectories effectively and efficiently}. 
% % In order to detect anomalous subtrajectories efficiently via an online manner, we propose a novel detection algorithm, namely \texttt{RL4OASD}, which leverages the learned policy during training process and enables online detection of anomalous subtrajectories effectively and efficiently.
% \item \textbf{} For the first challenge, we propose Road Segment Representation Network (RSRNet), which exploits road network representation learning and deep sequence modeling techniques that jointly model the mobility pattern underlying subtrajectories.     }}
% \end{itemize}
% \vspace{-\topsep}
Our contributions can be summarized as follows.
\begin{itemize}
    \item We propose the first deep reinforcement learning based solution to detect anomalous subtrajectories. The proposed model 1) can be trained without labeled data, 2) integrates techniques of road network representation learning (RSRNet) and deep reinforcement learning (ASDNet) to model the characteristics of subtrajectories, 3) 
    %\item We propose a novel detection paradigm based on the learned policy, which 
    allows the anomalous subtrajectory detection to be efficiently conducted in an online manner, {\Revision{and 4) handles the concept drift of anomalous trajectories.}}
    \item We conduct extensive experiments on two real-world trajectory datasets with manually labeled test data. We compare our proposed solution with various baselines, and the results show that our solution effectively and efficiently, i.e., it can significantly outperform the state-of-the-art methods (with 20-30\% improvement compared to the best existing approach) and is efficient for online anomalous subtrajectory detection (it takes less than 0.1ms to process each newly generated data point).
    \item {\Revision{The manually labeled test data is publicly accessible via the link~\footnote{https://www.dropbox.com/sh/imix3otoep49v0g/AACQLPpgA0jMdTg7LV-GdL70a?dl=0}.
    }}
\end{itemize}

The rest of paper is organized as follows. We review the literature in Section~\ref{sec:related}. We provide the problem definition in Section~\ref{sec:problem}. We present our \texttt{RL4OASD} model in Section~\ref{sec:method}. We demonstrate the experimental results in Section~\ref{sec:experiment}, and finally we conclude this paper in Section~\ref{sec:conclusion}.

% 1. emphasis this problem important
% 2. important (linking to application and motivation)
% 3. this problem is hard to solve-->challenges. 
% 4. insight of the paper (how to solve.)



















































==> method.tex <==
\section{METHODOLOGY}
\label{sec:method}

\subsection{Overview of \texttt{RL4OASD}}
To discover the anomalous subtrajectories from an ongoing trajectory, we explore a reinforcement learning based method within a weakly supervised framework called RL4OASD. We illustrate the overall architecture of RL4OASD in Figure~\ref{fig:rl4oasd}. It includes three components and we discuss them as follows.

In data preprocessing, we obtain map-matched trajectories via map-matching the raw trajectories on road networks. The map-matched trajectory is in the form of a sequence of road segments, which can be represented its travel route. We then design a noisy labeling method to label each road segment as 0 representing normal and 1 otherwise, by counting each transition frequency from historical trajectories. The noisy labels are then used to train the Road Segment Representation Network (RSRNet) in a weakly supervised manner (Section~\ref{sec:weakly}). 

In RSRNet, we infer the normal routes behind a detected trajectory and train the embeddings of road segments of the trajectory. Those embeddings are fed into the Anomalous Subtrajectory Detection  Network (ASDNet) as the state, to provide observations for labeling anomalous subtrajectories. We implement the RSRNet with RNN, which is able to capture the sequential information of trajectories (Section~\ref{sec:RSRNet}).

In ASDNet, we build a road network enhanced environment for labeling each road segment as normal or not. The task is modeled as a \emph{Markov decision process}~\cite{puterman2014markov}, whose policies are learned via a policy gradient method~\cite{silver2014deterministic} (Section~\ref{sec:ASDNet}). 

Note that the ASDNet outputs refined labels of road segments, which are further used to train RSRNet again, and then RSRNet provides better observations for ASDNet to train better policies. The process iterates and we call the resulting algorithm combined RSRNet and ASDNet as RL4OASD (Section~\ref{sec:RL4OASD}).

\subsection{Data Preprocessing for Noisy Labels}\
\label{sec:weakly}
Our RL4OASD model consists of two networks (i.e., RSRNet and ASDNet), where RSRNet is essentially to capture the features of each road segment. However, labeled data (i.e., the labeled anomalous subtrajectories in a detected trajectory) is usually not available in the datasets, which makes it a challenge to learn good representations. To overcome this, we explore the network training in a weakly supervised setting (i.e., using noisy labels), and take the spatial and temporal factors into consideration. More specifically, the process includes four steps. \underline{Step-1}: we group historical trajectories in a dataset wrt different SD-Pairs and time slots. Here, we have 24 time slots if we partition one day with one hour granularity, and we say a trajectory falls into a time slot if its starting travel time is within the slot. e.g., in Figure~\ref{fig:example}, we have three map-matched trajectories $T_1$, $T_2$ and $T_3$ under the source $e_1$ and destination $e_10$. Assuming the starting travel times of $T_1$, $T_2$ and $T_3$ are 9:00, 17:00, and 9:10, respectively. Therefore, $T_1$ and $T_3$ are in the same group (denoted by Group-1) because they are within the same time slot with one hour granularity, and $T_2$ is in the other group (denoted by Group-2).
%
\underline{Step-2}: we then capture the fraction of transitions wrt all trajectories in each group, e.g., in Group-1 (i.e., $T_1$ and $T_3$), suppose that there are 9 trajectories traveling the same route as $T_1$ and only one trajectory traveling traveling route as $T_3$, the fraction of transition $<e_1,e_2>$ is calculated by $1/10=0.1$ since it appears only once in all 10 trajectories.
%
\begin{figure}
  \centering
  \includegraphics[width=0.8\linewidth, height=0.5\linewidth]{figures/example}
  \caption{$T_1$, $T_2$ and $T_3$ are three map-matched trajectories under $e_1$ (source) and $e_{10}$ (destination). %Assuming the starting travel times of $T_1$, $T_2$ and $T_3$ are 9:00, 17:00, and 9:10, and thus $T_1$ and $T_3$ are in the same group (denoted by Group-1) because they are within the same time slot with one hour granularity, and $T_2$ is in the other group (denoted by Group-2).
  }
  \label{fig:example}
  \vspace{-5mm}
\end{figure}

\underline{Step-3}: for each trajectory, we refer to the group it belongs to
and map it to a sequence of transition fractions wrt each road segment. e.g., for a trajectory traveling the route as $T_3$, its mapped sequence is $<1.0,0.1,0.1,0.1,0.1,0.1,0.1,0.1,1.0>$. Note that the fractions on the source (i.e., $e_1$) and the destination (i.e., $e_1$) are set to 1.0 since the two road segments are definitely traveled within its group.
%
\underline{Step-4}: the noisy labels can be obtained with a threshold is given, denoted by $\alpha$, e.g., the noisy labels of $T_3$ is $<0,1,1,1,1,1,1,1,0>$ given $alpha=0.1$, where 0 denotes a normal road segment, whose fraction is larger than $\alpha$ meaning that the road segment is frequently traveled, and 1 otherwise. 
%
The noisy labels are then used in the training of RSRNet. Compared with manually labeling~\cite{zhang2011ibat,chen2013iboat, lv2017outlier}, such noisy labels can be obtained more easily.

\subsection{Road Segment Representation Network (RSRNet)}
\label{sec:RSRNet}
RSRNet aims to provide representations of road segments as the state for the MDP in ASDNet. To design RSRNet, we adopt LSTM~\cite{hochreiter1997long} structure, which accepts trajectories with different lengths and captures the sequential information behind trajectories. In addition, we embed two types of features into representations, one is to capture the traffic context on road networks, and the other one is to capture the normal routes for a given SD-Pair. 

\noindent \textbf{Traffic Context Feature (TCF).} A map-matched trajectory corresponds to a sequence of road segments and each road segment is naturally in the form of the token (i.e., the road segment id). We pre-train each road segment in the embedding layer of RSRNet as a vector, which embeds traffic context features (e.g., driving speed, trip duration, road type) into it. To do this, we employ Toast~\cite{chen2021robust} to learn road segments, which is the state-of-the-art road network representation learning model to support road segment based applications. The learned road segment representations will be used to initialize the embedding
layer in RSRNet, and those embeddings can still be further optimized with the model training. Other road network representation models~\cite{jepsen2019graph,wang2019learning} are also applicable for the task.

\noindent \textbf{Normal Route Feature (NRF).} Given an SD-Pair in a time slot, we first infer the normal routes within it. Intuitively, the normal trajectories are often followed the same route. If a trajectory contains some road segments that are rarely traveled by others, and it probably contains anomalies. Therefore, we infer a route as the normal route by calculating the fraction of the trajectories passing through the route wrt all trajectories within its SD-Pair. The inferring is controlled with a threshold (denoted by $\delta$), i.e., a route is inferred as the normal if the fraction is larger than the threshold, vice versa.
%
For example, given $\delta=0.4$, recall that the Group-1 with the trajectory $T_1$ (appearing 9 times) and $T_3$ (appearing 1 time) in Figure~\ref{fig:example}, we infer $T_1$ as the normal route, because its fraction ($9/10=0.9$) is larger than the threshold $\delta$.
%
Based on the inferred normal routes, we then extract the features of a detected trajectory. For example, given a detected trajectory followed the route as $T_3$, we partition the trajectory into a sequence of transitions, and we detect whether a road segment in a detected trajectory is normal (i.e., 0) if the transition on that road segment occurs in the inferred normal routes; 1 otherwise. For example, the extracted normal features of $T_3$ is $<0,1,1,1,1,1,1,1,0>$, where the feature on the road segment $e_2$ is 0 since the transition $<e_1,e_2>$ does not occur in the normal route $T_1$. Note that the source and destination road segments are always denoted by 0 (i.e., normal) in the extracted features. After obtaining the normal route features on road segments, we embed them via an embedding layer, and the embedded vectors are then fed into the model.

\noindent \textbf{Training RSRNet.} Figure~\ref{fig:rl4oasd} illustrates the architecture of RSRNet. In particular, given a sequence of embedded traffic context features $\mathbf{x_i}^{tcf}$ ($1 \leq i \leq n$), where $n$ denotes the trajectory length, and the LSTM obtains the hidden states $\mathbf{h_i}$ at each road segment, accordingly. We then concatenate $\mathbf{h_i}$ with the embedding of normal route feature $\mathbf{x_i}^{nrf}$, denoted by $\mathbf{z}_i=[\mathbf{h}_i;\mathbf{x}_i^{nrf}]$. RSRNet is trained using the noisy labels, and we adopt cross-entropy loss to train RSRNet between the predicted label $\hat{y}_i$ based on the $\mathbf{z}_i$ and the noisy label $y_i$, i.e., $\mathcal{L}=\frac{1}{n}\sum_{i=1}^{n}\mathcal{H}(y_i,\hat{y}_i)$, where $\mathcal{H}$ denotes the cross-entropy operator. The trained $\mathbf{z}_i$ is then fed into ASDNet as the state representation in ASDNet.
%, and the parameters in RSRNet will be optimized during the joint training of RSRNet and ASDNet.

\subsection{Anomalous Subtrajectory Detection Network (ASDNet)}
\label{sec:ASDNet}
We implement ASDNet with reinforcement learning (RL). Consider the task of online anomalous subtrajectory detection is to sequentially scan an ongoing trajectory and for each road segment, it decides whether an anomaly happened at that position. This motivates us to model the process as an MDP, involving actions, states, transitions
and rewards. In addition, we utilize the graph structure of a road network to build an environment for conducting the MDP, which helps the anomaly detection as discussed below.

\noindent \textbf{Road Network Enhanced Environment (RNEE).} Consider a transition $<e_{i-1},e_i>$ ($1 < i \leq n$) between two road segments $e_{i-1}$ and $e_i$. Based on the graph structure of road networks, we denote the out degree and in degree on a road segment $e_{i}$ as $e_{i}.out$, $e_{i}.in$. We then label each road segment as normal (i.e.,0) or abnormal (i.e., 1), denoted by $e_{i}.l$, according to the following four lemmas.

\begin{lemma}
\label{lemma:1}
Given $e_{i-1}.out=1$ and $e_{i}.in=1$, we have $e_{i}.l=e_{i-1}.l$.
\end{lemma}
\begin{proof}
The transition is smooth without any road turns can be involved, and thus the labels on $e_{i-1}$ and $e_{i}$ maintain the same.
\end{proof}

\begin{lemma}
\label{lemma:2}
Given $e_{i-1}.out=1$ and $e_{i}.in>1$, we have $e_{i}.l=0$, if $e_{i-1}.l=0$.
\end{lemma}
\begin{proof}
This can be proved by contradiction. Suppose $e_{i}.l=1$ when $e_{i-1}.l=0$, it implies that an anomaly happened on the road segment $e_{i}$, whose movement do not follow the normal road, denoted by $e'_{i}$. This contradicts the fact that $e_{i-1}.out=1$. Hence, the lemma holds.
\end{proof}

\begin{lemma}
\label{lemma:3}
Given $e_{i-1}.out>1$ and $e_{i}.in=1$, we have $e_{i}.l=1$, if $e_{i-1}.l=1$.
\end{lemma}
\begin{proof}
We also prove it by contradiction. Suppose $e_{i}.l=0$ when $e_{i-1}.l=1$, it indicates that an anomaly finished on the road segment $e_{i}$, which is definitely associated with a normal road $e'_{i-1}$ that is traveled. This contradicts the fact that $e_{i}.in=1$. Hence, the lemma holds. 
\end{proof}

\begin{lemma}
\label{lemma:4}
Given $e_{i-1}.out>1$ and $e_{i}.in>1$, $e_{i-1}.l$ and $e_{i}.l$ are arbitrary, i.e., $e_{i}.l=e_{i-1}.l$ or $e_{i}.l \neq e_{i-1}.l$.
\end{lemma}
\begin{proof}
The lemma directly follows the observation.
\end{proof}

We build an environment for conducting the MDP, where a decision for labeling a road segment is deterministic in one of three cases: (1) $e_{i-1}.out=1$, $e_{i}.in=1$ (Lemma~\ref{lemma:1});
(2) $e_{i-1}.out=1$, $e_{i}.in>1$ and $e_{i-1}.l=0$ (Lemma~\ref{lemma:2}); (3) $e_{i-1}.out>1$, $e_{i}.in=1$ and $e_{i-1}.l=1$ (Lemma~\ref{lemma:3}). In other cases, it makes a decision via the model.
%
As we can see many decisions have been replaced by the lemma~\ref{lemma:1}, \ref{lemma:2} and \ref{lemma:3}, and it brings at least two advantages. First, the efficiency is improved since the time of constructing states and taking actions at some road segments is saved via checking the light lemmas. Second, as many cases have been pruned with deterministic decisions, the RL model is lightly to train for tackling the otherwise cases, and some potential wrong decisions can therefore be avoided. Based on the road network enhanced environment, we define the MDP as follows.

\noindent \textbf{Actions.} We denote an action of the MDP by $a$, which is to label each road segment as normal or not. Note that an anomalous subtrajectory boundary can be identified when the labels of two adjacent road segments are different, and the action is only conducted by the RL model when a decision is required based on the road network enhanced environment.

\noindent \textbf{States.} The state $\mathbf{s}_i$ ($1 < i \leq n$) is represented by the concatenation of $\mathbf{z}_i$ and $\mathbf{v}(e_{i-1}.l)$, i.e., $\mathbf{s}_i=[\mathbf{z}_i;\mathbf{v}(e_{i-1}.l)]$, where $\mathbf{z}_i$ is obtained from RSRNet and $\mathbf{v}(e_{i-1}.l)$ denotes the vector of the label on the previous road segment $e_{i-1}.l$ via a embedding layer, whose parameter is learnable in ASDNet. The rationale for the state design is to capture the features from three aspects, i.e., traffic context, normal routes and the previous label.

\noindent \textbf{Transitions.} We take an action $a$ to produce a label on a road segment at a state $\mathbf{s}$, it then would label the next road segment. There are two cases: (1) the labeling is deterministic at the next road segment based on the derived lemmas above. In this case, the process continues for the next; otherwise, (2) we construct a new state $\mathbf{s}'$, which corresponds to the next state of $\mathbf{s}$, to output an action via the RL model.

\noindent \textbf{Rewards.} We design the reward in terms of two aspects. One is called \emph{local reward}, which aims to capture the local continuity of labels of road segments. The rationale is that normal road segments or anomalous road segments are usually continued for several times. Intuitively, the labels would not be changed frequently. The other one is called \emph{global reward}. During the training, we check the model performance based on the task of online anomalous subtrajectory detection (OASD). We take the model performance (i.e., $F_1$-score) as a signal to guide the training.

The local reward is an intermediate reward, which encourages the continuity of the labels on road segments. It is defined as $r_i^{local}=\text{sign}(e_{i-1}.l=e_{i}.l)\text{cos}(\mathbf{z}_{i-1},\mathbf{z}_{i})$, where the $\text{sign}(e_{i-1}.l=e_{i}.l)$ returns 1 if the condition $e_{i-1}.l=e_{i}.l$ is true and -1 otherwise; $\text{cos}(\mathbf{z}_{i-1},\mathbf{z}_{i})$ denotes the consine similarity between $\mathbf{z}_{i-1}$ and $\mathbf{z}_{i}$, which are obtained from SRNet.

The global reward is obtained based on the OASD task. To do this, we manually label a development dataset for around 100 trajectories (more details for the manually labeling are presented in Section~\ref{sec:setup}), and we evaluate the model performance within the development dataset in terms of the $F_1$-score metric (more details regarding the evaluation metric are presented in Section~\ref{sec:setup}). We evaluate the model performance during the training, and take the returned $F_1$-score as the global reward, denoted by $r^{global}$. We use this reward as a long-term reward, which is calculated when all road segments on a trajectory are labeled, 

Then, the expected cumulative reward for a trajectory is defined as $R_n=\frac{1}{n-1}\sum_{i=2}^{n}r_i^{local}+r^{global}$.

\noindent \textbf{Policy Learning on the MDP.} 
The core problem of an MDP is to learn a policy, which guides an agent to choose actions based on the constructed states such that the cumulative reward is maximal. We learn the policy via a policy gradient method~\cite{silver2014deterministic}, called the REINFORCE algorithm~\cite{williams1992simple}. To be specific, let $\pi_{\theta}(a|\mathbf{s})$ denote a stochastic policy, which is used to sample an action $a$ for a given state $\mathbf{s}$ via a neural network, whose parameters are denoted by $\theta$. Then, the gradients wrt the network parameters $\theta$ are estimated as $\nabla_{\theta}J(\theta) = \sum_{i=2}^{n}R_n\nabla_{\theta}\ln\pi_{\theta}(a_i|s_i)$, which can be optimized using an optimizer (e.g., Adam stochastic gradient descent).

\noindent \textbf{Joint Training of RSRNet and ASDNet.} We jointly train the two networks (e.g., RSRNet and ASDNet). First, we map raw trajectories on road networks and generate noisy labels as explained in Section~\ref{sec:weakly}. Then, we randomly sample 200 trajectories to pre-train the RSRNet and ASDNet, separately. The pre-training provides a warm-start for the two networks. 
%
During the training, we randomly sample 10,000 trajectories, and for each trajectory, we generate 5 epochs to iteratively train the RSRNet and ASDNet. In particular, we apply the learned policy from ASDNet to 
refine the noisy labels, and the refined labels are used to train the RSRNet to obtain the better representation $\mathbf{z}_i$ on each road segment. Then, $\mathbf{z}_i$ is used to construct the state to learn better policy in ASDNet. Since the learned policy can further refine the labels, and the two networks are jointly trained with the best model is chosen during the process.

\subsection{The RL4OASD Algorithm}
\label{sec:RL4OASD}
Our \texttt{RL4OASD} algorithm is based on the learned policy for detecting anomalous subtrajectories. The process is presented in Algorithm~\ref{alg:rl4oasd}. Specifically, \texttt{RL4OASD} accepts an ongoing trajectory in an online fashion for labeling each road segment as the normal (i.e., 0) or not (i.e., 1) (lines 1-12). It first labels the source or destination road segment as normal by definitions (lines 2-3). It then validates the three deterministic cases according to Lemma \ref{lemma:1}, \ref{lemma:2} or \ref{lemma:3}. If so, it labels the current road segment with the label on the previous road segment (lines 4-5). If not, it 
constructs a state via calling RSRNet (lines 7-8), and samples an action to label the road segment based on the learned policy in ASDNet (lines 9-10). Finally, it returns the anomalous subtrajectories which involve the abnormal labels (i.e., 1) on the road segments.

We further develop a technique (called labeling with delay) for boosting the effectiveness. \texttt{RL4OASD} forms an anomalous subtrajectory whenever its boundary is identified, i.e., the boundary is identified at $e_{i-1}$ if $e_{i-1}.l = 1$ and $e_{i}.l=0$. Intuitively, it looks a bit rush to form an anomalous subtrajectory and may produce many short fragments from a detected trajectory. Therefore, we consider a delay mechanism, which is to scan $D$ more road segments that follow $e_{i-1}$, and we form a subtrajectory by extending its boundary to the last one with label 1 if that road segment is contained among those $D$ road segments. It could be verified the labeling with delay does not incur much time cost, and offer a better continuity to avoid forming too many fragments instead.

\begin{algorithm}[t!]
	\caption{The \texttt{RL4OASD} algorithm}
	\label{alg:rl4oasd}
		\KwIn{
		A map-matched trajectory $T = <e_1, e_2, ..., e_n>$ which is inputted in an online manner}
		\KwOut{
		The anomalous subtrajectories}
        \For{$i=1,2,...,n$}{
			\uIf{$i=1$ \textbf{or} $i=n$}{
			$e_{i}.l \leftarrow 0$;
			}
            \uElseIf{Lemma \ref{lemma:1}, \ref{lemma:2} or \ref{lemma:3} is valid}{
			$e_{i}.l \leftarrow e_{i-1}.l$;
			}
           \Else{
           Call RSRNet for obtaining a representation $\mathbf{z}_{i}$;\\
		   Construct a state $\mathbf{s}_i=[\mathbf{z}_i;\mathbf{v}(e_{i-1}.l)]$;\\
		   Sample an action (i.e., 0 or 1), $a_i \sim \pi_{\theta}(a|s)$;\\
		   $e_{i}.l \leftarrow a_i$;\\
        }

}
\textbf{Return} anomalous subtrajectories consisting of the road segments with the label 1;\\
\end{algorithm}

\noindent \textbf{Time complexity.} The time complexity of the \texttt{RL4OASD} algorithm is $O(n)$, where $n$ denotes the length of a detected trajectory. The time is dominated by two networks, i.e., RSRNet and ASDNet. We analyze them as follows. In RSRNet, the time cost of one road segment consists of (1) that of obtaining embeddings of TCF and NRF, which are both $O(1)$ and (2) that of obtaining the $\mathbf{z}$ via a classic LSTM cell, which is $O(1)$. In ASDNet, the time cost of one road segment consists of (1) that of constructing a state, where the part $\mathbf{z}$ has been computed in RSRNet and the part $\mathbf{v}(e.l)$ is obtained via an embedding layer, which is $O(1)$ and (2) that of sampling an action via the learned policy, which is $O(1)$. As we can see in Algorithm~\ref{alg:rl4oasd}, the two networks are called at most $n$ times. Therefore, the time complexity of the \texttt{RL4OASD} is $O(n)\times O(1)=O(n)$. We note that the $O(n)$ time complexity maintains the current best time complexity as those of existing algorithms~\cite{chen2013iboat,wu2017fast,liu2020online} for the trajectory or subtrajectory detection task, and can largely meet practical needs for online scenarios as shown in our experiments.

==> method2.tex <==
\section{METHODOLOGY}
\label{sec:method}

\subsection{Overview of \texttt{RL4OASD}}
To discover the anomalous subtrajectories from an ongoing trajectory, we explore a reinforcement learning based method within a weakly supervised framework called RL4OASD. We illustrate the overall architecture of RL4OASD in Figure~\ref{fig:rl4oasd}. It includes three components and we discuss them as follows.

In data preprocessing, we obtain map-matched trajectories via map-matching the raw trajectories on road networks. The map-matched trajectory is in the form of a sequence of road segments, which can be represented its travel route. We then design a noisy labeling method to label each road segment as 0 representing normal and 1 otherwise, by counting each transition frequency from historical trajectories. The noisy labels are then used to train the Road Segment Representation Network (RSRNet) in a weakly supervised manner (Section~\ref{sec:weakly}). 

In RSRNet, we infer the normal routes behind a detected trajectory and train the embeddings of road segments of the trajectory. Those embeddings are fed into the Anomalous Subtrajectory Detection  Network (ASDNet) as the state, to provide observations for labeling anomalous subtrajectories. We implement the RSRNet with RNN, which is able to capture the sequential information of trajectories (Section~\ref{sec:RSRNet}).

In ASDNet, we build a road network enhanced environment for labeling each road segment as normal or not. The task is modeled as a \emph{Markov decision process}~\cite{puterman2014markov}, whose policies are learned via a policy gradient method~\cite{silver2014deterministic} (Section~\ref{sec:ASDNet}). 

Note that the ASDNet outputs refined labels of road segments, which are further used to train RSRNet again, and then RSRNet provides better observations for ASDNet to train better policies. The process iterates and we call the resulting algorithm combined RSRNet and ASDNet as RL4OASD (Section~\ref{sec:RL4OASD}).

\noindent\textbf{19 Nov-Cheng: Comments on the overview description. 1. It could be a bit difficult to follow (since it assumes an ``author'' angle over the overview, but not a ``reader'' one; 2. It does not explain clearly why we design the method in the way it is (weak supersion + reinforcement learning) and how it is superior over existing solutions. This part needs to revised further.}


\noindent\textbf{19 Nov-Cheng: Comments on the overview figure. 1: The figure looks too small; 2. it does not show how $x^{nrf}$ features are obtained; 3. it does not show the linkage from z variables from RSRNet to those in ASDNet; 4. it does not show how the 0/1 lables used for constructing states in ASDNet are obtained; 5. RNN could be better changed to LSTM? 6. could we also reflect the iterative training process with this figure?}

\subsection{Data Preprocessing for Noisy Labels}\
\label{sec:weakly}
Our RL4OASD model consists of two networks (i.e., RSRNet and ASDNet), where RSRNet is essentially to capture the features of each road segment. However, labeled data (i.e., the labeled anomalous subtrajectories in a detected trajectory) is usually not available in the datasets, which makes it a challenge to learn good representations. To overcome this, we explore the network training in a weakly supervised setting (i.e., using noisy labels), and take the spatial and temporal factors into consideration. More specifically, the process includes four steps. \underline{Step-1}: we group historical trajectories in a dataset wrt different SD-Pairs and time slots. Here, we have 24 time slots if we partition one day with one hour granularity, and we say a trajectory falls into a time slot if its starting travel time is within the slot. e.g., in Figure~\ref{fig:example}, we have three map-matched trajectories $T_1$, $T_2$ and $T_3$ under the source $e_1$ and destination $e_{10}$. Assuming the starting travel times of $T_1$, $T_2$ and $T_3$ are 9:00, 17:00, and 9:10, respectively. Therefore, $T_1$ and $T_3$ are in the same group (denoted by Group-1) because they are within the same time slot with one hour granularity, and $T_2$ is in the other group (denoted by Group-2).
%
\underline{Step-2}: we then capture the fraction of transitions wrt all trajectories in each group, e.g., in Group-1 (i.e., $T_1$ and $T_3$), suppose that there are 9 trajectories traveling the same route as $T_1$ and only one trajectory traveling traveling route as $T_3$, the fraction of transition $<e_1,e_2>$ is calculated by $1/10=0.1$ since it appears only once in all 10 trajectories.
%

% \begin{figure}
%   \centering
%   \includegraphics[width=0.8\linewidth, height=0.5\linewidth]{figures/example}
%   \caption{$T_1$, $T_2$ and $T_3$ are three map-matched trajectories under $e_1$ (source) and $e_{10}$ (destination). %Assuming the starting travel times of $T_1$, $T_2$ and $T_3$ are 9:00, 17:00, and 9:10, and thus $T_1$ and $T_3$ are in the same group (denoted by Group-1) because they are within the same time slot with one hour granularity, and $T_2$ is in the other group (denoted by Group-2).
%   }
%   \label{fig:example}
%   \vspace{-5mm}
% \end{figure}



\underline{Step-3}: for each trajectory, we refer to the group it belongs to
and map it to a sequence of transition fractions wrt each road segment. e.g., for a trajectory traveling the route as $T_3$, its mapped sequence is $<1.0,0.1,0.1,0.1,0.1,0.1,0.1,0.1,1.0>$. Note that the fractions on the source (i.e., $e_1$) and the destination (i.e., $e_1$) are set to 1.0 since the two road segments are definitely traveled within its group.
%
\underline{Step-4}: the noisy labels can be obtained with a threshold is given, denoted by $\alpha$, e.g., the noisy labels of $T_3$ is $<0,1,1,1,1,1,1,1,0>$ given $alpha=0.1$, where 0 denotes a normal road segment, whose fraction is larger than $\alpha$ meaning that the road segment is frequently traveled, and 1 otherwise. 
%
The noisy labels are then used in the training of RSRNet. Compared with manually labeling~\cite{zhang2011ibat,chen2013iboat, lv2017outlier}, such noisy labels can be obtained more easily.


\noindent\textbf{19 Nov-Cheng: Comments on the noisy labelling part. 1: It mentions that capturing the road segment features without labels is challenging, which I don't agree. For example, self/un-supverised learning is widely used to learn representations, e.g., we can simply use the Toast method. My understanding is that noisy labelling is simply to provide some initialized labels to start with; 2: To show the benefits of this component, some ablation study (e.g., by replacing the noisy labels with random labels) could be conducted. 3: The description of Step-3 is not clear enough and need to be revised further (e.g., sometimes, the fractions are defined for transitions, and some other times, they are for road segments);}


\subsection{Road Segment Representation Network (RSRNet)}
\label{sec:RSRNet}
RSRNet aims to provide representations of road segments as the state for the MDP in ASDNet. To design RSRNet, we adopt LSTM~\cite{hochreiter1997long} structure, which accepts trajectories with different lengths and captures the sequential information behind trajectories. In addition, we embed two types of features into representations, one is to capture the traffic context on road networks, and the other one is to capture the normal routes for a given SD-Pair. 

\noindent \textbf{Traffic Context Feature (TCF).} A map-matched trajectory corresponds to a sequence of road segments and each road segment is naturally in the form of the token (i.e., the road segment id). We pre-train each road segment in the embedding layer of RSRNet as a vector, which embeds traffic context features (e.g., driving speed, trip duration, road type) into it. To do this, we employ Toast~\cite{chen2021robust} to learn road segments, which is the state-of-the-art road network representation learning model to support road segment based applications. The learned road segment representations will be used to initialize the embedding
layer in RSRNet, and those embeddings can still be further optimized with the model training. Other road network representation models~\cite{jepsen2019graph,wang2019learning} are also applicable for the task.

\noindent \textbf{Normal Route Feature (NRF).} Given an SD-Pair in a time slot, we first infer the normal routes within it. Intuitively, the normal trajectories are often followed the same route. If a trajectory contains some road segments that are rarely traveled by others, and it probably contains anomalies. Therefore, we infer a route as the normal route by calculating the fraction of the trajectories passing through the route wrt all trajectories within its SD-Pair. The inferring is controlled with a threshold (denoted by $\delta$), i.e., a route is inferred as the normal if the fraction is larger than the threshold, vice versa.
%
For example, given $\delta=0.4$, recall that the Group-1 with the trajectory $T_1$ (appearing 9 times) and $T_3$ (appearing 1 time) in Figure~\ref{fig:example}, we infer $T_1$ as the normal route, because its fraction ($9/10=0.9$) is larger than the threshold $\delta$.
%
Based on the inferred normal routes, we then extract the features of a detected trajectory. For example, given a detected trajectory followed the route as $T_3$, we partition the trajectory into a sequence of transitions, and we detect whether a road segment in a detected trajectory is normal (i.e., 0) if the transition on that road segment occurs in the inferred normal routes; 1 otherwise. For example, the extracted normal features of $T_3$ is $<0,1,1,1,1,1,1,1,0>$, where the feature on the road segment $e_2$ is 0 since the transition $<e_1,e_2>$ does not occur in the normal route $T_1$. Note that the source and destination road segments are always denoted by 0 (i.e., normal) in the extracted features. After obtaining the normal route features on road segments, we embed them via an embedding layer, and the embedded vectors are then fed into the model.

\noindent \textbf{Training RSRNet.} Figure~\ref{fig:rl4oasd} illustrates the architecture of RSRNet. In particular, given a sequence of embedded traffic context features $\mathbf{x_i}^{tcf}$ ($1 \leq i \leq n$), where $n$ denotes the trajectory length, and the LSTM obtains the hidden states $\mathbf{h_i}$ at each road segment, accordingly. We then concatenate $\mathbf{h_i}$ with the embedding of normal route feature $\mathbf{x_i}^{nrf}$, denoted by $\mathbf{z}_i=[\mathbf{h}_i;\mathbf{x}_i^{nrf}]$. RSRNet is trained using the noisy labels, and we adopt cross-entropy loss to train RSRNet between the predicted label $\hat{y}_i$ based on the $\mathbf{z}_i$ and the noisy label $y_i$, i.e., $\mathcal{L}=\frac{1}{n}\sum_{i=1}^{n}\mathcal{H}(y_i,\hat{y}_i)$, where $\mathcal{H}$ denotes the cross-entropy operator. The trained $\mathbf{z}_i$ is then fed into ASDNet as the state representation in ASDNet.
%, and the parameters in RSRNet will be optimized during the joint training of RSRNet and ASDNet.

\noindent\textbf{22 Nov-Cheng: Comments on RSRNet. 1. The part of defining fractions and using a threshold $\delta$ looks quite similar to the part in the noisy labelling part. I understand that they are different, the former at the route level and the latter at the road segment level. Readers may wonder why not use these features as noisy labels or vice versa. These issues should be clearly addressed/explained; 2. It is not clear how $x^{nrf}$ features are embedded; 3. It needs to be explained why not let the embeddings of $x^{nrf}$ go through the RNN network;}

\subsection{Anomalous Subtrajectory Detection Network (ASDNet)}
\label{sec:ASDNet}
We implement ASDNet with reinforcement learning (RL). Consider the task of online anomalous subtrajectory detection is to sequentially scan an ongoing trajectory and for each road segment, it decides whether an anomaly happened at that position. This motivates us to model the process as an MDP, involving actions, states, transitions
and rewards. In addition, we utilize the graph structure of a road network to build an environment for conducting the MDP, which helps the anomaly detection as discussed below.

\noindent \textbf{Road Network Enhanced Environment (RNEE).} Consider a transition $<e_{i-1},e_i>$ ($1 < i \leq n$) between two road segments $e_{i-1}$ and $e_i$. Based on the graph structure of road networks, we denote the out degree and in degree on a road segment $e_{i}$ as $e_{i}.out$, $e_{i}.in$. We then label each road segment as normal (i.e.,0) or abnormal (i.e., 1), denoted by $e_{i}.l$, according to the following four lemmas.

\begin{lemma}
\label{lemma:1}
Given $e_{i-1}.out=1$ and $e_{i}.in=1$, we have $e_{i}.l=e_{i-1}.l$.
\end{lemma}
\begin{proof}
The transition is smooth without any road turns can be involved, and thus the labels on $e_{i-1}$ and $e_{i}$ maintain the same.
\end{proof}

\begin{lemma}
\label{lemma:2}
Given $e_{i-1}.out=1$ and $e_{i}.in>1$, we have $e_{i}.l=0$, if $e_{i-1}.l=0$.
\end{lemma}
\begin{proof}
This can be proved by contradiction. Suppose $e_{i}.l=1$ when $e_{i-1}.l=0$, it implies that an anomaly happened on the road segment $e_{i}$, whose movement do not follow the normal road, denoted by $e'_{i}$. This contradicts the fact that $e_{i-1}.out=1$. Hence, the lemma holds.
\end{proof}

\begin{lemma}
\label{lemma:3}
Given $e_{i-1}.out>1$ and $e_{i}.in=1$, we have $e_{i}.l=1$, if $e_{i-1}.l=1$.
\end{lemma}
\begin{proof}
We also prove it by contradiction. Suppose $e_{i}.l=0$ when $e_{i-1}.l=1$, it indicates that an anomaly finished on the road segment $e_{i}$, which is definitely associated with a normal road $e'_{i-1}$ that is traveled. This contradicts the fact that $e_{i}.in=1$. Hence, the lemma holds. 
\end{proof}

\begin{lemma}
\label{lemma:4}
Given $e_{i-1}.out>1$ and $e_{i}.in>1$, $e_{i-1}.l$ and $e_{i}.l$ are arbitrary, i.e., $e_{i}.l=e_{i-1}.l$ or $e_{i}.l \neq e_{i-1}.l$.
\end{lemma}
\begin{proof}
The lemma directly follows the observation.
\end{proof}

We build an environment for conducting the MDP, where a decision for labeling a road segment is deterministic in one of three cases: (1) $e_{i-1}.out=1$, $e_{i}.in=1$ (Lemma~\ref{lemma:1});
(2) $e_{i-1}.out=1$, $e_{i}.in>1$ and $e_{i-1}.l=0$ (Lemma~\ref{lemma:2}); (3) $e_{i-1}.out>1$, $e_{i}.in=1$ and $e_{i-1}.l=1$ (Lemma~\ref{lemma:3}). In other cases, it makes a decision via the model.
%
As we can see many decisions have been replaced by the lemma~\ref{lemma:1}, \ref{lemma:2} and \ref{lemma:3}, and it brings at least two advantages. First, the efficiency is improved since the time of constructing states and taking actions at some road segments is saved via checking the light lemmas. Second, as many cases have been pruned with deterministic decisions, the RL model is lightly to train for tackling the otherwise cases, and some potential wrong decisions can therefore be avoided. Based on the road network enhanced environment, we define the MDP as follows.

\noindent \textbf{Actions.} We denote an action of the MDP by $a$, which is to label each road segment as normal or not. Note that an anomalous subtrajectory boundary can be identified when the labels of two adjacent road segments are different, and the action is only conducted by the RL model when a decision is required based on the road network enhanced environment.

\noindent \textbf{States.} The state $\mathbf{s}_i$ ($1 < i \leq n$) is represented by the concatenation of $\mathbf{z}_i$ and $\mathbf{v}(e_{i-1}.l)$, i.e., $\mathbf{s}_i=[\mathbf{z}_i;\mathbf{v}(e_{i-1}.l)]$, where $\mathbf{z}_i$ is obtained from RSRNet and $\mathbf{v}(e_{i-1}.l)$ denotes the vector of the label on the previous road segment $e_{i-1}.l$ via a embedding layer, whose parameter is learnable in ASDNet. The rationale for the state design is to capture the features from three aspects, i.e., traffic context, normal routes and the previous label.

\noindent \textbf{Transitions.} We take an action $a$ to produce a label on a road segment at a state $\mathbf{s}$, it then would label the next road segment. There are two cases: (1) the labeling is deterministic at the next road segment based on the derived lemmas above. In this case, the process continues for the next; otherwise, (2) we construct a new state $\mathbf{s}'$, which corresponds to the next state of $\mathbf{s}$, to output an action via the RL model.

\noindent \textbf{Rewards.} We design the reward in terms of two aspects. One is called \emph{local reward}, which aims to capture the local continuity of labels of road segments. The rationale is that normal road segments or anomalous road segments are usually continued for several times. Intuitively, the labels would not be changed frequently. The other one is called \emph{global reward}. During the training, we check the model performance based on the task of online anomalous subtrajectory detection (OASD). We take the model performance (i.e., $F_1$-score) as a signal to guide the training.

The local reward is an intermediate reward, which encourages the continuity of the labels on road segments. It is defined as $r_i^{local}=\text{sign}(e_{i-1}.l=e_{i}.l)\text{cos}(\mathbf{z}_{i-1},\mathbf{z}_{i})$, where the $\text{sign}(e_{i-1}.l=e_{i}.l)$ returns 1 if the condition $e_{i-1}.l=e_{i}.l$ is true and -1 otherwise; $\text{cos}(\mathbf{z}_{i-1},\mathbf{z}_{i})$ denotes the consine similarity between $\mathbf{z}_{i-1}$ and $\mathbf{z}_{i}$, which are obtained from SRNet.

The global reward is obtained based on the OASD task. To do this, we manually label a development dataset for around 100 trajectories (more details for the manually labeling are presented in Section~\ref{sec:setup}), and we evaluate the model performance within the development dataset in terms of the $F_1$-score metric (more details regarding the evaluation metric are presented in Section~\ref{sec:setup}). We evaluate the model performance during the training, and take the returned $F_1$-score as the global reward, denoted by $r^{global}$. We use this reward as a long-term reward, which is calculated when all road segments on a trajectory are labeled, 

Then, the expected cumulative reward for a trajectory is defined as $R_n=\frac{1}{n-1}\sum_{i=2}^{n}r_i^{local}+r^{global}$.

\noindent \textbf{Policy Learning on the MDP.} 
The core problem of an MDP is to learn a policy, which guides an agent to choose actions based on the constructed states such that the cumulative reward is maximal. We learn the policy via a policy gradient method~\cite{silver2014deterministic}, called the REINFORCE algorithm~\cite{williams1992simple}. To be specific, let $\pi_{\theta}(a|\mathbf{s})$ denote a stochastic policy, which is used to sample an action $a$ for a given state $\mathbf{s}$ via a neural network, whose parameters are denoted by $\theta$. Then, the gradients wrt the network parameters $\theta$ are estimated as $\nabla_{\theta}J(\theta) = \sum_{i=2}^{n}R_n\nabla_{\theta}\ln\pi_{\theta}(a_i|s_i)$, which can be optimized using an optimizer (e.g., Adam stochastic gradient descent).

\noindent \textbf{Joint Training of RSRNet and ASDNet.} We jointly train the two networks (e.g., RSRNet and ASDNet). First, we map raw trajectories on road networks and generate noisy labels as explained in Section~\ref{sec:weakly}. Then, we randomly sample 200 trajectories to pre-train the RSRNet and ASDNet, separately. The pre-training provides a warm-start for the two networks. 
%
During the training, we randomly sample 10,000 trajectories, and for each trajectory, we generate 5 epochs to iteratively train the RSRNet and ASDNet. In particular, we apply the learned policy from ASDNet to 
refine the noisy labels, and the refined labels are used to train the RSRNet to obtain the better representation $\mathbf{z}_i$ on each road segment. Then, $\mathbf{z}_i$ is used to construct the state to learn better policy in ASDNet. Since the learned policy can further refine the labels, and the two networks are jointly trained with the best model is chosen during the process.

\noindent\textbf{22 Nov-Cheng: Comment on the RNEE. It is not that interesting/technicallly novel as it may look to be. I suggest: (1) we do NOT call them lemmas (they are rules but not lemmas that are always correct); (2) we less emphasize this technique (e.g., we treat it similarly as we do the "delay" technique - after all, they are simple rules). To me, the first case could be easily excluded by preprocessing the road networks so that junctions with degree = 2 are dropped and I don't think we have many instances of case 2 and 3 in the real data (you may collect the statistics); (3) we summarize the intuition behind the rules and avoid presenting them rule by rule with 4 cases - I belive they share some intuition; (4) with this change, this section and the pseudo-code need to be adjusted accordingly; (5) same as the "delay technique", we can do some ablation sutdy on the technique based on the rules;}

\noindent\textbf{22 Nov-Cheng: Comments on other parts of the section: 1. For transitions, my understanding is that in either case, we need re-compute the next state? In its current writing, it looks that in the first case, we don't re-compute the state; 2. For local reward, the intuition should be better explained (e.g., why we use the cosine term); 3. For the global reward, it will immediately trigger that we use extra information that is not available for existing solutions. In fact, based on the experimental results (ablation study), even we drop this global reward, we still achieve the best results. How about we target the setting with no labelled data at all? 4. For the joint training, it is not clear how the pre-training works exactly? Why is it necessary?}

\subsection{The RL4OASD Algorithm}
\label{sec:RL4OASD}
Our \texttt{RL4OASD} algorithm is based on the learned policy for detecting anomalous subtrajectories. The process is presented in Algorithm~\ref{alg:rl4oasd}. Specifically, \texttt{RL4OASD} accepts an ongoing trajectory in an online fashion for labeling each road segment as the normal (i.e., 0) or not (i.e., 1) (lines 1-12). It first labels the source or destination road segment as normal by definitions (lines 2-3). It then validates the three deterministic cases according to Lemma \ref{lemma:1}, \ref{lemma:2} or \ref{lemma:3}. If so, it labels the current road segment with the label on the previous road segment (lines 4-5). If not, it 
constructs a state via calling RSRNet (lines 7-8), and samples an action to label the road segment based on the learned policy in ASDNet (lines 9-10). Finally, it returns the anomalous subtrajectories which involve the abnormal labels (i.e., 1) on the road segments.

We further develop a technique (called labeling with delay) for boosting the effectiveness. \texttt{RL4OASD} forms an anomalous subtrajectory whenever its boundary is identified, i.e., the boundary is identified at $e_{i-1}$ if $e_{i-1}.l = 1$ and $e_{i}.l=0$. Intuitively, it looks a bit rush to form an anomalous subtrajectory and may produce many short fragments from a detected trajectory. Therefore, we consider a delay mechanism, which is to scan $D$ more road segments that follow $e_{i-1}$, and we form a subtrajectory by extending its boundary to the last one with label 1 if that road segment is contained among those $D$ road segments. It could be verified the labeling with delay does not incur much time cost, and offer a better continuity to avoid forming too many fragments instead.

\begin{algorithm}[t!]
	\caption{The \texttt{RL4OASD} algorithm}
	\label{alg:rl4oasd}
		\KwIn{
		A map-matched trajectory $T = <e_1, e_2, ..., e_n>$ which is inputted in an online manner}
		\KwOut{
		The anomalous subtrajectories}
        \For{$i=1,2,...,n$}{
			\uIf{$i=1$ \textbf{or} $i=n$}{
			$e_{i}.l \leftarrow 0$;
			}
            \uElseIf{Lemma \ref{lemma:1}, \ref{lemma:2} or \ref{lemma:3} is valid}{
			$e_{i}.l \leftarrow e_{i-1}.l$;
			}
           \Else{
           Call RSRNet for obtaining a representation $\mathbf{z}_{i}$;\\
		   Construct a state $\mathbf{s}_i=[\mathbf{z}_i;\mathbf{v}(e_{i-1}.l)]$;\\
		   Sample an action (i.e., 0 or 1), $a_i \sim \pi_{\theta}(a|s)$;\\
		   $e_{i}.l \leftarrow a_i$;\\
        }

}
\textbf{Return} anomalous subtrajectories consisting of the road segments with the label 1;\\
\end{algorithm}

\noindent \textbf{Time complexity.} The time complexity of the \texttt{RL4OASD} algorithm is $O(n)$, where $n$ denotes the length of a detected trajectory. The time is dominated by two networks, i.e., RSRNet and ASDNet. We analyze them as follows. In RSRNet, the time cost of one road segment consists of (1) that of obtaining embeddings of TCF and NRF, which are both $O(1)$ and (2) that of obtaining the $\mathbf{z}$ via a classic LSTM cell, which is $O(1)$. In ASDNet, the time cost of one road segment consists of (1) that of constructing a state, where the part $\mathbf{z}$ has been computed in RSRNet and the part $\mathbf{v}(e.l)$ is obtained via an embedding layer, which is $O(1)$ and (2) that of sampling an action via the learned policy, which is $O(1)$. As we can see in Algorithm~\ref{alg:rl4oasd}, the two networks are called at most $n$ times. Therefore, the time complexity of the \texttt{RL4OASD} is $O(n)\times O(1)=O(n)$. We note that the $O(n)$ time complexity maintains the current best time complexity as those of existing algorithms~\cite{chen2013iboat,wu2017fast,liu2020online} for the trajectory or subtrajectory detection task, and can largely meet practical needs for online scenarios as shown in our experiments.

\noindent\textbf{22 Nov-Cheng: For the delay technique, the description is not precise. Is it the same as a post-processing step which convert some 0's to 1's very D steps?}

==> method3.tex <==
\section{METHODOLOGY}
\label{sec:method}

\subsection{Overview of \texttt{RL4OASD}}

%  review what you mentioned about it in Introduction, 
%  I want you to highlight how to handle the issues in the method section.
% corresponding to introduction
As we mentioned in section~\ref{sec:problem}, the task of online anomalous trajectory detection is modelled via a supervised learning method, which fails to utilize in real applications, as it needs a large amount of labelled data. In addition, determining an ongoing trajectory is anomalous or not is a decision-making process, which could be modelled as a as a Markov decision process (MDP)~\cite{puterman2014markov}. We propose a weakly supervised framework, namely RL4OASD via the reinforcement learning. The framework consists of three components, namely data preprocessing, RSRNet and ASDNet(see Figure~\ref{fig:rl4oasd}). 

In data preprocessing, data preprocessing aims to provide noisy labelled data for training RSRNet. In particular, we conduct map-matching on raw trajectories, mapping them onto road networks and obtain the map-matched trajectories. The map-matching trajectory is denoted as a sequence of road segments. Then to save more efforts and provide more information for following phases, we design a noisy labelling method to label each road segment as 0 representing normal and 1 representing abnormal via counting each transition frequency from historical trajectories. The noisy labels are then used to train the Road Segment Representation Network (RSRNet) in weakly supervised manner(section~\ref{sec:weakly}). Also, we \emph{manually labelled} 1,688 (resp.1,057) SD pairs, which correspond to 558,098 (resp. 163,027) raw trajectories before map-matching for Chengdu (resp. Xi’an), which is utilized as test data to evaluate the performance of our method.
% In particular, counting each transition frequency from historical trajectories and then comparing the transition frequency with the setting threshold is utilized to setting the each road segment 0 or 1.


In RSRNet, RSRNet aims to provide representations of road segments as the state for the MDP in ASDNet, which provide a method to model subtrajectories and take advantage of road networks. We capture two types of representations. One is to capture the traffic context feature representation by Toast~\cite{chen2021robust}. Another is to capture normal route feature by calculating the fraction of the each road segment involved in the map-matched trajectories for each SD pair. Those embeddings are fed into the Anomalous Subtrajectory Detection  Network (ASDNet) as the state, to provide observations for labeling anomalous subtrajectories. We also implement the RSRNet with RNN, which is able to capture the sequential information of trajectories (Section~\ref{sec:RSRNet}).

In ASDNet, we build a road network enhanced environment, which provides a more effective way to label each road segment as normal or not. The task is modeled as a \emph{Markov decision process}~\cite{puterman2014markov}, whose policies are learned via a policy gradient method~\cite{silver2014deterministic} (Section~\ref{sec:ASDNet}). 

Note that the ASDNet outputs refined labels of road segments, which are further used to train RSRNet again, and then RSRNet provides better observations for ASDNet to train better policies. The process iterates and we call the resulting algorithm combined RSRNet and ASDNet as RL4OASD (Section~\ref{sec:RL4OASD}).



\subsection{Data Preprocessing for Noisy Labels}
\label{sec:weakly}
% Our RL4OASD model consists of two networks (i.e., RSRNet and ASDNet), where RSRNet is essentially to capture the features of each road segment. However, labeled data (i.e., the labeled anomalous subtrajectories in a detected trajectory) is usually not available in the datasets, which makes it a challenge to learn good representations. 
We explore the network training in a weakly supervised setting (i.e., using noisy labels), and take the spatial and temporal factors into consideration. More specifically, the process of obtaining noisy labels includes four steps.

\underline{Step-1}: we group historical trajectories in a dataset wrt different SD-Pairs and time slots. Here, we have 24 time slots if we partition one day with one hour granularity, and we say a trajectory falls into a time slot if its starting travel time is within the slot. e.g., in Figure~\ref{fig:example}, we have three map-matched trajectories $T_1$, $T_2$ and $T_3$ under the source $e_1$ and destination $e_{10}$. Assuming the starting travel times of $T_1$, $T_2$ and $T_3$ are 9:00, 17:00, and 9:10, respectively. Therefore, $T_1$ and $T_3$ are in the same group (denoted by Group-1) because they are within the same time slot with one hour granularity, and $T_2$ is in the other group (denoted by Group-2).

\underline{Step-2}: we then capture the fraction of \emph{transitions} (we defined in section~\ref{sec:problem}) wrt all trajectories in each group, e.g., in Group-1 (i.e., $T_1$ and $T_3$), suppose that there are 9 trajectories traveling the same route as $T_1$ and only one trajectory traveling traveling route as $T_3$, the fraction of \emph{transition} $<e_1,e_2>$ is calculated by $1/10=0.1$ since it appears only once in all 10 trajectories.

\underline{Step-3}: for each trajectory, we refer to the group it belongs to
and map it to a sequence of \emph{transition} fractions wrt each road segment. {\color{blue}{E.g., for a trajectory travelling the route as $T_3$, its mapped \emph{transition} sequence is $<<*,e_1>, <e_1,e_2>, <e_2,e_4>, <e_4, e_{11}>, <e_{11}, e_{12}>, <e_{12}, e_{13}>, <e_{13}, e_{14}>, <e_{14}, e_{15}>, <e_{15}, e_{10}>>$, where we pad the initial transition as $<*,e_1>$, and the corresponding fraction sequence is $<1.0,0.1,0.1,0.1,0.1,0.1,0.1,0.1,0.1,1.0>$}. Note that the fractions on the source $e_1$ (corresponding to $<*,e_1>$) and the destination $e_{10}$ (corresponding to $<e_{15}, e_{10}>$) are always set to 1.0, since the source and destination road segments are definitely travelled within its group.}

\underline{Step-4}: the noisy labels can be obtained with a threshold is given, denoted by $\alpha$, e.g., the noisy labels of $T_3$ is $<0,1,1,1,1,1,1,1,1,0>$ given $\alpha=0.1$, where 0 denotes a normal road segment, whose fraction is larger than $\alpha$ meaning that the road segment is frequently traveled, and 1 otherwise. 
%
The noisy labels are then utilized in the training of RSRNet. Compared with manually labeling~\cite{zhang2011ibat,chen2013iboat, lv2017outlier}, such noisy labels can be obtained more easily.

 
\subsection{Road Segment Representation Network (RSRNet)}
\label{sec:RSRNet}
RSRNet aims to provide representations of road segments as the state for the MDP in ASDNet, {\color{blue}{which provides a method to model subtrajectories and take advantage of road networks.}} To design RSRNet, we adopt LSTM~\cite{hochreiter1997long} structure, which accepts trajectories with different lengths and captures the sequential information behind trajectories. In addition, we embed two types of features into representations, one is to capture the traffic context on road networks, and the other one is to capture the normal routes for a given SD-Pair. 

\noindent \textbf{Traffic Context Feature (TCF).} A map-matched trajectory corresponds to a sequence of road segments and each road segment is naturally in the form of the token (i.e., the road segment id). We pre-train each road segment in the embedding layer of RSRNet as a vector, which embeds traffic context features (e.g., driving speed, trip duration, road type) into it. To do this, we employ Toast~\cite{chen2021robust} to learn road segments, which is the state-of-the-art road network representation learning model to support road segment based applications. The learned road segment representations will be used to initialize the embedding
layer in RSRNet, and those embeddings can still be further optimized with the model training. Other road network representation models~\cite{jepsen2019graph,wang2019learning} are also applicable for the task.

\noindent \textbf{Normal Route Feature (NRF).} Given an SD-Pair in a time slot, we first infer the normal routes within it. Intuitively, the normal trajectories are often followed the same route. If a trajectory contains some road segments that are rarely traveled by others, and it probably contains anomalies. Therefore, we infer a route as the normal route by calculating the fraction of the trajectories passing through the route wrt all trajectories within its SD-Pair. The inferred results are obtained via comparing a threshold (denoted by $\delta$) with the fraction of each road segment, i.e., a route is inferred as the normal if the fraction is larger than the threshold, vice versa.
%
For example, given $\delta=0.4$, recall that the Group-1 with the trajectory $T_1$ (appearing 9 times) and $T_3$ (appearing 1 time) in Figure~\ref{fig:example}, we infer $T_1$ as the normal route, because its fraction ($9/10=0.9$) is larger than the threshold $\delta$.
%
Based on the inferred normal routes, we then extract the features of a detected trajectory. For example, given a detected trajectory followed the route as $T_3$, we partition the trajectory into a sequence of transitions, and we detect whether a road segment in a detected trajectory is normal (i.e., 0) if the transition on that road segment occurs in the inferred normal routes; 1 otherwise. For example, the extracted normal features of $T_3$ are $<0,1,1,1,1,1,1,1,0>$, where the feature on the road segment $e_2$ is 1 since the transition $<e_1,e_2>$ does not occur in the normal route $T_1$. {\Comment{Note that the extracted normal features of the source and destination road segments are always 0 (i.e., normal). 
%We notice normal route features and noisy labels are both in the form of 0-1 vectors. We use the former as input features since they are fine-grained to recognize the normal or abnormal information on each road segment via discovering the normal routes, and remains unchanged during the training; however, noisy labels are coarse-grained as the initialized labels for the training, and be will be refined by ASDNet latter.
%
After obtaining the normal route features that are in the form of tokens, we then obtain a vector for the feature by embedding the tokens as one-hot vectors. We call the obtained vectors embedded normal route features.
%
}}

\noindent \textbf{Training RSRNet.} Figure~\ref{fig:rl4oasd} illustrates the architecture of RSRNet. In particular, given a sequence of embedded traffic context features $\mathbf{x_i}^{t}$ ($1 \leq i \leq n$), where $n$ denotes the trajectory length, and the LSTM obtains the hidden states $\mathbf{h_i}$ at each road segment, accordingly. We then concatenate $\mathbf{h_i}$ with the embedded normal route feature $\mathbf{x_i}^{n}$, denoted by $\mathbf{z}_i=[\mathbf{h}_i;\mathbf{x}_i^{n}]$. {\Comment{Note that the two parts $\mathbf{h}$ and $\mathbf{x}^{n}$ capture the sequential trajectory information and normal route information, respectively. They are concatenated and further used to denote the state of RL in ASDNet. Note that we do not let $\mathbf{x}^{n}$ go through the LSTM since it preserves the normal route feature at each road segment.
}}
RSRNet is trained using the noisy labels, and we adopt cross-entropy loss to train RSRNet between the predicted label $\hat{y}_i$ based on the $\mathbf{z}_i$ and the noisy label $y_i$, i.e.,
\begin{equation}
\label{eq:entropy}
\mathcal{L}=\frac{1}{n}\sum_{i=1}^{n}\mathcal{H}(y_i,\hat{y}_i),
\end{equation}
where $\mathcal{H}$ denotes the cross-entropy operator. 
%The trained $\mathbf{z}_i$ is then fed into ASDNet as the state representation in ASDNet.
%, and the parameters in RSRNet will be optimized during the joint training of RSRNet and ASDNet.

 


\subsection{Anomalous Subtrajectory Detection Network (ASDNet)}
\label{sec:ASDNet}
We implement ASDNet with reinforcement learning (RL). Consider the task of online anomalous subtrajectory detection is to sequentially scan an ongoing trajectory and for each road segment, it decides whether an anomaly happened at that position. This motivates us to model the process as an MDP, involving actions, states, transitions
and rewards. {\Comment{In addition, we utilize the graph structure of a road network to build an environment for conducting the MDP, which reduces the cases of making decisions and facilitates the effectiveness.

\noindent \textbf{Road Network Enhanced Environment (RNEE).} Consider a transition $<e_{i-1},e_i>$ ($1 < i \leq n$) between two road segments $e_{i-1}$ and $e_i$. Based on the graph structure of road networks, we denote the out degree and in degree of a road segment $e_{i}$ as $e_{i}.out$ and $e_{i}.in$, respectively. $e_{i}.l$ denotes the label of the road segment $e_{i}$, where 0 denotes the normal and 1 denotes the abnormal.
\if 0
\begin{lemma}
\label{lemma:1}
Given $e_{i-1}.out=1$ and $e_{i}.in=1$, we have $e_{i}.l=e_{i-1}.l$.
\end{lemma}
\begin{proof}
The transition is smooth without any road turns can be involved, and thus the labels on $e_{i-1}$ and $e_{i}$ maintain the same.
\end{proof}

\begin{lemma}
\label{lemma:2}
Given $e_{i-1}.out=1$ and $e_{i}.in>1$, we have $e_{i}.l=0$, if $e_{i-1}.l=0$.
\end{lemma}
\begin{proof}
This can be proved by contradiction. Suppose $e_{i}.l=1$ when $e_{i-1}.l=0$, it implies that an anomaly happened on the road segment $e_{i}$, whose movement do not follow the normal road, denoted by $e'_{i}$. This contradicts the fact that $e_{i-1}.out=1$. Hence, the lemma holds.
\end{proof}

\begin{lemma}
\label{lemma:3}
Given $e_{i-1}.out>1$ and $e_{i}.in=1$, we have $e_{i}.l=1$, if $e_{i-1}.l=1$.
\end{lemma}
\begin{proof}
We also prove it by contradiction. Suppose $e_{i}.l=0$ when $e_{i-1}.l=1$, it indicates that an anomaly finished on the road segment $e_{i}$, which is definitely associated with a normal road $e'_{i-1}$ that is traveled. This contradicts the fact that $e_{i}.in=1$. Hence, the lemma holds. 
\end{proof}

\begin{lemma}
\label{lemma:4}
Given $e_{i-1}.out>1$ and $e_{i}.in>1$, $e_{i-1}.l$ and $e_{i}.l$ are arbitrary, i.e., $e_{i}.l=e_{i-1}.l$ or $e_{i}.l \neq e_{i-1}.l$.
\end{lemma}
\begin{proof}
The lemma directly follows the observation.
\end{proof}
\fi
\begin{figure}
  \centering
  \includegraphics[width=\linewidth]{figures/rule.pdf}
  \vspace{-3mm}
  \caption{Illustrating three cases for deterministic labeling.}
  \label{fig:rule}
  \vspace{-3mm}
\end{figure}

We build an environment (called RNEE) for conducting the MDP, where a decision for labeling a road segment is deterministic in one of three cases. We illustrate the three cases in Figure~\ref{fig:rule} 
\begin{enumerate}
    \item If $e_{i-1}.out=1$, $e_{i}.in=1$, then $e_{i}.l=e_{i-1}.l$.
    \item If $e_{i-1}.out=1$, $e_{i}.in>1$ and $e_{i-1}.l=0$, then $e_{i}.l=0$.
    \item If $e_{i-1}.out>1$, $e_{i}.in=1$ and $e_{i-1}.l=1$, then $e_{i}.l=1$.
\end{enumerate}

We explain the three rules as follows. The common intuition behind them is the label on  $e_{i}$ can be determined in some cases when we know the road network structure and the previous label on $e_{i-1}$. 
%
For (1), the case can be seen as a ``smooth transition'' without any road turns, and thus the label on $e_{i}$ is the same as $e_{i-1}$. For (2) and (3), both two cases can be shown by contradiction. Suppose $e_{i}.l=1$ (resp. $e_{i}.l=0$) given $e_{i-1}.l=0$ (resp. $e_{i-1}.l=1$) in Case 2 (resp. Case 3), it implies that an anomaly happened on the road segment $e_{i}$ (resp. $e_{i-1}$), whose movement does not follow a normal road on $e'_{i}$ (resp. $e'_{i-1}$), where $e'_{i} \neq e_{i}$ (resp. $e'_{i-1} \neq e_{i-1}$). This contradicts the fact that $e_{i-1}.out=1$ (resp. $e_{i}.in=1$). 

The RNEE brings at least two advantages. First, the efficiency is improved since the time of taking actions in some cases is saved via checking the rules instead of calling the RL model.
%
Second, as many cases have been pruned with deterministic decisions, the RL model is light to train for only tackling the otherwise cases, and some potential wrong decisions can therefore be avoided. 
%
Based on the RNEE, we define the MDP as follows.
}}

\noindent \textbf{Actions.} We denote an action of the MDP by $a$, which is to label each road segment as normal or not. Note that an anomalous subtrajectory boundary can be identified when the labels of two adjacent road segments are different, and the action is only conducted by the RL model for the cases that are not in the aforementioned three cases.

\noindent \textbf{States.} The state $\mathbf{s}_i$ ($1 < i \leq n$) is represented by the concatenation of $\mathbf{z}_i$ and $\mathbf{v}(e_{i-1}.l)$, i.e., $\mathbf{s}_i=[\mathbf{z}_i;\mathbf{v}(e_{i-1}.l)]$, where $\mathbf{z}_i$ is obtained from RSRNet and $\mathbf{v}(e_{i-1}.l)$ denotes a vector of the label on the previous road segment $e_{i-1}.l$ by embedding its token (i.e., 0 or 1). The rationale for the state design is to capture the features from three aspects, i.e., traffic context, normal routes and the previous label.

\noindent \textbf{Transitions.} We take an action $a$ to produce a label on a road segment at a state $\mathbf{s}$, it then would label the next road segment. There are two cases: (1) the label can be determined based on the RNEE at the next road segment. In this case, the process continues for the next; {\Comment{(2) In the other case, let $\mathbf{s}'$ denote a new state, which corresponds to the next state of $\mathbf{s}$ after the action is taken.}}

\noindent \textbf{Rewards.} We design the reward in terms of two aspects. One is called \emph{local reward}, which aims to capture the local continuity of labels of road segments. The rationale is that normal road segments or anomalous road segments are usually continued for several times, and the labels would not be changed frequently. {\Comment{The other one is called \emph{global reward}, which aims to indicate the quality of the refined labels. Intuitively, with high-quality refined labels, we will obtain a lower cross-entropy loss as computed by Equation~\ref{eq:entropy} from RSRNet. We take the loss as some feedback to guide the training of ASDNet.
}}
%During the training, we check the model performance based on the task of online anomalous subtrajectory detection (OASD). 

The local reward is an intermediate reward, which encourages the continuity of the labels on road segments. It is defined as 
\begin{equation}
r_i^{local}=\text{sign}(e_{i-1}.l=e_{i}.l)\text{cos}(\mathbf{z}_{i-1},\mathbf{z}_{i}),
\end{equation}
where the $\text{sign}(e_{i-1}.l=e_{i}.l)$ returns 1 if the condition $e_{i-1}.l=e_{i}.l$ is true and -1 otherwise; $\text{cos}(\mathbf{z}_{i-1},\mathbf{z}_{i})$ denotes the consine similarity between $\mathbf{z}_{i-1}$ and $\mathbf{z}_{i}$, which are obtained from RSRNet. {\Comment{We choose the consine similarity because it outputs a normalized value between 0 and 1, which corresponds to the same output range (i.e., between 0 and 1) of the global reward.
}}

{\Comment{The global reward is designed to measure the quality of refined labels by ASDNet. To obtain the reward, we feed the refined labels into RSRNet, and compute the global reward as 
\begin{equation}
    r^{global}= \frac{1}{1+\mathcal{L}},
\end{equation}
where $\mathcal{L}$ denotes the cross-entropy loss in Equation~\ref{eq:entropy}. We notice this reward has the range between 0 and 1, and makes the objective of RSRNet well aligned with ASDNet (a smaller loss $\mathcal{L}$ means a larger global reward). 
% For the former, it is to minimize the $\mathcal{L}$, and  for the latter, it is to maximize the global reward $\frac{1}{1+\mathcal{L}}$ of ASDNet.
}}

\noindent \textbf{Policy Learning on the MDP.} 
The core problem of an MDP is to learn a policy, which guides an agent to choose actions based on the constructed states such that the cumulative reward, denoted by $R_n$, is maximal. We learn the policy via a policy gradient method~\cite{silver2014deterministic}, called the REINFORCE algorithm~\cite{williams1992simple}. To be specific, let $\pi_{\theta}(a|\mathbf{s})$ denote a stochastic policy, which is used to sample an action $a$ for a given state $\mathbf{s}$ via a neural network, whose parameters are denoted by $\theta$. Then, the gradients wrt the network parameters $\theta$ are estimated as
\begin{equation}
\label{eq:policy}
\nabla_{\theta}J(\theta) = \sum_{i=2}^{n}R_n\nabla_{\theta}\ln\pi_{\theta}(a_i|s_i),
\end{equation}
which can be optimized using an optimizer (e.g., Adam stochastic gradient ascent). Here, $R_n$ is the expected cumulative reward for a trajectory, which is defined as follows.
\begin{equation}
R_n=\frac{1}{n-1}\sum_{i=2}^{n}r_i^{local}+r^{global}.
\end{equation}

\noindent \textbf{Joint Training of RSRNet and ASDNet.} We jointly train the two networks (e.g., RSRNet and ASDNet). First, we map raw trajectories on road networks and generate the noisy labels as explained in Section~\ref{sec:weakly}. Then, we randomly sample 200 trajectories to pre-train the RSRNet and ASDNet, separately. {\Comment{In particular, for the RSRNet, we train the network in a supervised manner with the noisy labels. For the ASDNet, we specify its actions as the noisy labels, and train the policy network via a gradient ascent step as computed by Equation~\ref{eq:policy}. The pre-training provides a warm-start for the two networks, where the parameters of the two networks have incorporated some information captured from the normal routes before joint training.
}}
%
During the joint training, we randomly sample 10,000 trajectories, and for each trajectory, we generate 5 epochs to iteratively train the RSRNet and ASDNet. In particular, we apply the learned policy from ASDNet to 
refine the noisy labels, and the refined labels are used to train the RSRNet to obtain the better representation $\mathbf{z}_i$ on each road segment. Then, $\mathbf{z}_i$ is used to construct the state to learn better policy in ASDNet. Since the learned policy can further refine the labels, and the two networks are jointly trained with the best model is chosen during the process.
 
 
\subsection{The RL4OASD Algorithm}
\label{sec:RL4OASD}
Our \texttt{RL4OASD} algorithm is based on the learned policy for detecting anomalous subtrajectories. The process is presented in Algorithm~\ref{alg:rl4oasd}. Specifically, \texttt{RL4OASD} accepts an ongoing trajectory in an online fashion for labeling each road segment as the normal (i.e., 0) or not (i.e., 1) (lines 1-12). It first labels the source or destination road segment as normal by definitions (lines 2-3). It then validates the three deterministic cases. If so, it labels the current road segment with the label on the previous road segment (lines 4-5). If not, it 
constructs a state via calling RSRNet (lines 7-8), and samples an action to label the road segment based on the learned policy in ASDNet (lines 9-10). Finally, it returns the anomalous subtrajectories which involve the abnormal labels (i.e., 1) on the road segments.

We further develop a technique (called labeling with delay) for boosting the effectiveness. \texttt{RL4OASD} forms an anomalous subtrajectory whenever its boundary is identified, i.e., the boundary is identified at $e_{i-1}$ if $e_{i-1}.l = 1$ and $e_{i}.l=0$. Intuitively, it looks a bit rush to form an anomalous subtrajectory and may produce many short fragments from a detected trajectory. {\Comment{
%Therefore, we consider a delay mechanism, which is to scan $D$ more road segments that follow $e_{i-1}$, and we form a subtrajectory by extending its boundary to the last one with label 1 if that road segment is contained among those $D$ road segments. 
Therefore, we consider a delay technique as a post-processing step. Specifically, it scans $D$ more road segments that follow $e_{i-1}$ when forming an anomalous subtrajectory. Among the $D$ road segments, we choose the final position $j$ ($i-1<j \leq i-1+D$) where the road segment is with label 1, and then convert some 0's to 1's between the position $i-1$ and $j$.
%
It could be verified the labeling with delay does not incur much time cost, and offer a better continuity to avoid forming too many fragments instead.
}}
\begin{algorithm}[t!]
	\caption{The \texttt{RL4OASD} algorithm}
	\label{alg:rl4oasd}
		\KwIn{
		A map-matched trajectory $T = <e_1, e_2, ..., e_n>$ which is inputted in an online manner}
		\KwOut{
		The anomalous subtrajectories}
        \For{$i=1,2,...,n$}{
			\uIf{$i=1$ \textbf{or} $i=n$}{
			$e_{i}.l \leftarrow 0$;
			}
            \uElseIf{Case 1, 2 or 3 is valid}{
			$e_{i}.l \leftarrow e_{i-1}.l$;
			}
           \Else{
           Call RSRNet for obtaining a representation $\mathbf{z}_{i}$;\\
		   Construct a state $\mathbf{s}_i=[\mathbf{z}_i;\mathbf{v}(e_{i-1}.l)]$;\\
		   Sample an action (i.e., 0 or 1), $a_i \sim \pi_{\theta}(a|s)$;\\
		   $e_{i}.l \leftarrow a_i$;\\
        }

}
\textbf{Return} anomalous subtrajectories consisting of the road segments with the label 1;\\
\end{algorithm}

\noindent \textbf{Time complexity.} The time complexity of the \texttt{RL4OASD} algorithm is $O(n)$, where $n$ denotes the length of a detected trajectory. The time is dominated by two networks, i.e., RSRNet and ASDNet. We analyze them as follows. In RSRNet, the time cost of one road segment consists of (1) that of obtaining embeddings of TCF and NRF, which are both $O(1)$ and (2) that of obtaining the $\mathbf{z}$ via a classic LSTM cell, which is $O(1)$. In ASDNet, the time cost of one road segment consists of (1) that of constructing a state, where the part $\mathbf{z}$ has been computed in RSRNet and the part $\mathbf{v}(e.l)$ is obtained via an embedding layer, which is $O(1)$ and (2) that of sampling an action via the learned policy, which is $O(1)$. As we can see in Algorithm~\ref{alg:rl4oasd}, the two networks are called at most $n$ times. Therefore, the time complexity of the \texttt{RL4OASD} is $O(n)\times O(1)=O(n)$. We note that the $O(n)$ time complexity maintains the current best time complexity as those of existing algorithms~\cite{chen2013iboat,wu2017fast,liu2020online} for the trajectory or subtrajectory detection task, and can largely meet practical needs for online scenarios as shown in our experiments.

 


























==> problem.tex <==
\section{PROBLEM DEFINITION}
\label{sec:problem}
\if 0
\smallskip\noindent
\emph{\textbf{Problem Definition.}}
Trajectories are collected from the trace of the moving objects by GPS. A trajectory of taxi consists of a sequence of GPS points including latitude, longitude and timestamp, denoted as $T = <p_1, p_2, .....p_n>$, each point is represented as $t_i = (lat_i, lon_i, t_i)$.
In our work, a taxi moves from a source point $s$ to a destination point $d$ in a road network referring to a SD pair. There are a lot of trajectories in each SD pair. The trajectory occur with high probability is denoted as normal routes. 
In this paper, we use the taxi trajectory datasets of \emph{Xi'an} and \emph{Chengdu}. Figure ~\ref{} shows the trajectories from a source to a destination.

\emph{Definition 1: Raw Trajectory.} A trajectory $T$ consists of a sequence of GPS points, which is represented as $T = <p_1, p_2, .....p_n>$, where $p_i$ represents a GPS point, denoted as $P_i = (lat_i, lon_i, t_i)$. Here, $lat_i,lon_i, t_i$ denote the latitude, the longitude and the timestamp of the point $p_i$ respectively.

\emph{Definition 2: Road network.} A road network is represented as a directed graph $G(V,E)$, where $V$ represents a vertex set referring to crossroads and $E$ represents a edge set referring to road segments. 

\emph{Definition 3: Edge Trajectory.} A edge trajectory refers a route $R = <s_1, s_2, .....s_n>$ consists of sets of road segments recording the result of a raw trajectory $T$ after map matching. 

\emph{\textbf{Problem statement:}} Given an SD pair and an ongoing trajectory $T$, the ongoing trajectory $T$ is anomalous if it rarely occurs and is different from the reference trajectories in the SD pair.
Besides, we want to identify the anomalous sub-trajectory of the ongoing trajectory. 
\fi

\smallskip
\noindent \textbf{(1) Raw Trajectory.} A raw trajectory $T$ consists of a sequence of GPS points, i.e., $T = <p_1, p_2,...,p_n>$, where a GPS point $P_i$ is in the form of a triplet, i.e., $P_i = (x_i, y_i, t_i)$, to record a moving object is located on $(x_i, y_i)$ at timestamp $t_i$, and $n$ represents the length of the trajectory $T$.

\smallskip
\noindent \textbf{(2) Road Network.} A road network is represented as a directed graph $G(V,E)$, where $V$ represents a vertex set referring to crossroads or intersections, and $E$ represents an edge set referring to road segments, and for each edge $e$, it connects two vertexes $u$ and $v$ on the road network, denoted as $e=(u,v)$.

\smallskip
\noindent \textbf{(3) Map-matched Trajectory.} A map-matched trajectory refers to a trajectory generated by a moving object on road networks, which corresponds to a sequence of road segments after map-matching~\cite{yang2018fast}, i.e., $T = <e_1, e_2,...,e_n>$. 

For simplicity, {\Comment{we use $T$ to denote a map-matched trajectory, and we refer to map-matched trajectories as trajectories or routes interchangeably in the rest of the paper.}}


\smallskip
\noindent \textbf{(4) Subtrajectory and Transition.} A subtrajectory $T[i,j]$ corresponds to a portion of the trajectory $T = <e_1, e_2,...,e_n>$ from $e_i$ to $e_j$, $1 \leq i \leq j \leq n$. A transition is defined as a special case of a subtrajectory, which only consists of two adjacent road segments to capture the road turn of a moving object, i.e., $<e_{i-1}, e_{i}>$, where $1< i \leq n$.

\smallskip
\noindent \textbf{(5) Online Anomalous Subtrajectory Detection (OASD).} We study the problem of online anomalous subtrajectory detection. Given a source $S$ and destination $D$ pair (SD-pair) with a set of trajectories $\mathcal{T}$ between them. Intuitively, a trajectory $T$ can be considered as the \emph{normal} if it follows the route traveled by the most of trajectories in $\mathcal{T}$. Based on this, we denote an \emph{anomalous} subtrajectory representing a part of a trajectory, whose route \emph{do not} follow the normal routes within the SD-pair. We formulate the problem as follows.

\begin{figure*}
  \centering
  \includegraphics[width=0.85\linewidth]{figures/model2.pdf}
  \vspace{-3mm}
  \caption{Overview of \texttt{RL4OASD}, where $\bigoplus$ denotes the concatenation operation.}
  \label{fig:rl4oasd}
  \vspace{-3mm}
\end{figure*}

\begin{problem}[OASD] Given an ongoing trajectory $T=<e_1,e_2,...e_n>$ that is generated from its source $S_T$ to destination $D_T$ in an online fashion, {\Comment{where the points come one by one, and the future points are not
accessible in advance.
OASD problem aims to identify which parts of a trajectory (i.e., subtrajectories) are anomalous if $T$ contains the anomalous subtrajectories,
while T is sequentially generated.}}
\label{prob:oasd}
\end{problem} 

 


==> related.tex <==
\section{RELATED WORK}
\label{sec:related}
\subsection{Online Anomalous Trajectory Detection}

Existing studies of anomalous trajectory detection are divided into two categories with respect to whether the target trajectory is complete: online anomalous trajectory detection methods and offline anomalous trajectory detection methods.
Online anomalous trajectory detection methods refer to detecting the partial trajectory.
%The first category is usually based on detecting anomalous trajectories with generating trajectory points. There are two steps in the first category:
%1) the first step is to define the normal routes and give representative normal routes and 2) comparing the object trajectory with the representative normal trajectories based on metric-based methods or learning-based methods.
For example, A recent study which is a learning-based method ~\citet{liu2020online} proposes to detect anomalous trajectories by detection-via-generation scheme using gaussian mixture distribution to represent the normal routes, which could represent different kinds of normal routes
and detect anomalous trajectories effectively and efficiently; however, this method cannot detect which part of the trajectory is anomalous. Another learning-based method is introduced in ~\cite{wu2017fast}, which proposes to model the distribution of driving behaviours by probabilistic model without access to historical trajectories in database. However, the linearity of the model of this method makes it hard to get the complex information data behind the trajectories and ignores the sequential context information of trajectories. And another recent study which is learning-based~\cite{zhang2020continuous} proposes a method to calculate the estimation deviation to detect the anomalous trajectory, which is efficient to detect the anomalous trajectories. Neverless, this method requires a reference trajectory for each source-destination (SD) pair, which has a large effect on the performance of the method. Besides, this method cannot detect the which part of the trajectory is anomalous.

One metric-based online anomalous trajectory detection study ~\cite{chen2013iboat} which is designed to detect the anomalous trajectory and the detour part which is similar to our work proposes to maintain a adaptive working window of the latest ongoing trajectory points to compare against the set of the historical trajectories in the working set to better detect anomalousness of the ongoing trajectory. The specific idea is as a new ongoing trajectory point is added into the adaptive working window, some of historical trajectories in the working set are removed by certain trajectory which is inconsistent with the subtrajectory in adaptive working window, new points are added into the adaptive working window until the support value of the subtrajectory in the adaptive working window below the threshold $theta$, the adaptive working window is reduced to contain the latest coming points, which is more likely  to be anomalous point. And then the adaptive working window will not increase until the next anomalous point. In this iteration until the end of the trajectory, the set of the points in the adaptive working window is the anomalous points in the trajectory. Thus, the limitations of this method include: 1) the method needs to maintain a adaptive working window to record the latest points and the working set to record the historical trajectories to be compared with the ongoing part of the trajectory, which is time-consuming and not efficient enough to detect anomalous trajectories. 2) this method consider trajectories in freespace, which is not effective enough without the road network constraints for anomalous trajectories detection. Our work ....
%Anomalous trajectories are isolated from a lot of normal trajectories; thus, the larger variance represents the larger probability the route is the anomaly. This method needs access to historical trajectories which cannot support anomalous trajectory detection efficiently. time-consuming and not efficient enough for detecting anomalous trajectories

\subsection{Other Anomalous Trajectory Detection Studies}
Offline anomalous trajectory detection methods refer to detect the anomalous trajectory based on a complete trajectory. All online methods can handle complete trajectories' detection. There are some methods are proposed for detecting anomalous trajectories based on complete trajectories. Offline trajectory detection methods based on the complete trajectory are usually based on distance or density metrics. A study based on distance metrics ~\cite{lee2008trajectory} proposes to detect anomalous trajectory segments by calculating the distance of each segment of the target trajectory to each segments in other trajectories. Another study~\cite{zhang2011ibat} proposes to detect anomalous trajectories via checking the isolation from normal trajectories in the same iteration. This method needs to compare the target trajectory with historical trajectories in database, which is time-consuming. Some literatures, such as ~\cite{zhu2015time,lv2017outlier} propose other distance metrics to detect anomalous trajectories via mining trajectory patterns. One learning-based offline anomalous trajectory detection study ~\cite{song2018anomalous} consider context information of trajectories using Recurrent neural network (RNN) for anomalous detection. However, this method is supervised method, which uses labeled data that is not available in real anomaly detection appliance. Another learning-based work~\cite{gray2018coupled} propose to use adversarial learning to do anomalous trajectory detection, which has a major limit that this method can only apply for detecting trajectories with the same length. Thus these two recent studies are not applicable to real anomalous trajectory detection. Other studies ~\cite{ge2010top,yu2014detecting,banerjee2016mantra}are other types of anomalous trajectory detection,such as detect time-series anomalous trajectories, which will be discussed further.


%These two categories of anomalous trajectory detection have the following drawbacks: Firstly, these methods cannot detect which part of a trajectory is detour.
%Secondly, all methods set different thresholds for different trajectories, which is time-consuming and cannot support efficient online detection.



\subsection{Deep Reinforcement Learning}

In recent years, reinforcement learning is introduced into anomaly detection in ~\cite{oh2019sequential}, which propose a method to do sequential anomaly detection; and ~\citet{huang2018towards} proposes a method based on reinforcement learning to do temporally anomalous detection.
Our work is very different from them in that (i) our work focuses anomalous subtrajectory detection and output the detour avoiding to access historical trajectories in database. (ii) our work detect anomalous trajectories detection with road network constraints, which is the same as the real application. (iii) our work uses deep reinforcement learning to refine the noise labels that we used. (iv) our work contributes a dataset of the anomalous trajectories.

%\noindent \textbf{(1) Sports Data Analytics.}


%\noindent \textbf{(2) Measuring Pointsets Similarity.}
% From the technical perspective, our problem is related to the problem of measuring the similarity between two pointsets. Although the pointsets similarity has been studied extensively, billiards layouts have several characteristics, e.g., a layout is composed of one cue (white) ball and some object (colored) balls on a billiards table with six pockets, which make them unique and differ from existing studies.
%


==> related2.tex <==
\section{RELATED WORK}
\label{sec:related}
\subsection{Online Anomalous Trajectory Detection}
Many recent studies are proposed for online anomalous trajectory detection.
Online anomalous trajectory detection methods aim to detect a trajectory which is ongoing in an online manner. We discuss these studies in terms of two categories: heuristic-based methods~\cite{ge2010top,yu2014detecting,chen2013iboat,zhang2020continuous} and learning-based methods~\cite{wu2017fast,liu2020online}.

For heuristic-based methods, 
%an early effort~\cite{ge2010top} proposes to detect an evolving trajectory in an accumulating way to count outlying scores, by considering direction-based outlier scores and density-based outlier scores.
%
%Yu et al.~\cite{yu2014detecting} further propose a new trajectory outlier definition by introducing neighboring trajectories into detection in the large-scale trajectory streams.
%
Chen et al.~\cite{chen2013iboat} study the online anomalous trajectory detection with the isolation-based method, which aims to check which parts of a detected trajectory that can be isolated from the reference (i.e., normal) trajectories with the same source and destination routes.
%
Recently, Zhang et al.~\cite{zhang2020continuous} propose to monitor the trajectory similarity based on discrete Frechet distance between a given reference route and the current partial route at each timestamp. If the deviation threshold exceeds a given threshold at any timestamp, and the system alerts that an outlier event of detouring is detected. Our work differs from these studies in that it is based on a road network-enhanced policy learned via reinforcement learning instead of the hand-crafted heuristic with many predefined parameters (e.g., the deviation threshold) for detecting anomalies.

For learning-based methods, a recent study~\citet{liu2020online} proposes to detect anomalous trajectories via a generation scheme, it uses Gaussian mixture distribution to represent different kinds of normal routes and detect those anomalous trajectories that cannot be well-generated based on the given representations of normal routes. Another learning-based method is introduced in~\cite{wu2017fast}, which proposes a probabilistic model to detect trajectory outliers via modeling the distribution of driving behaviours from historical trajectories. The method considers many potential features that are associated with driving behaviour modeling, including road level and turning angle, etc. In our work, we target a more finer-grained setting, i.e, detecting which part of an anomalous trajectory, namely subtrajectory, is responsible for its anomalousness in an online manner. In contrast, subtrajectory detection is not their focus in these studies.

\subsection{Offline Anomalous Trajectory Detection}
Other proposals on anomalous trajectory detection detect the anomalous trajectory by assuming full access to the whole trajectory data (i.e., offline anomalous trajectory detection), and we review the literature in terms of the heuristic-based methods~\cite{lee2008trajectory,zhang2011ibat,zhu2015time,lv2017outlier,banerjee2016mantra} and learning-based methods~\cite{gray2018coupled,song2018anomalous} as follows.

For heuristic-based methods, some distance or density metrics are usually proposed for detecting anomalies. For example, an early study~\cite{lee2008trajectory} proposes to partition the trajectories and detect the anomalous trajectory segments by computing the distance of each segment in a detected trajectory to the segments in other trajectories. Further, Zhu et al.~\cite{zhu2015time} and Lv et al.~\cite{lv2017outlier} adopt the edit distance based metrics to detect anomalies via mining normal trajectory patterns. Another study~\cite{zhang2011ibat} proposes to cluster the trajectories crossing the same itinerary and detect anomalous trajectories via checking the isolation from the cluster. In addition, Ge et al~\cite{ge2011taxi} develop a taxi driving fraud system, which is equipped with both distance and density metrics to identify fraud driving activities. 

Other studies are proposed to detect anomalous trajectories with learning-based methods. Song et al~\cite{song2018anomalous} adopt recurrent neural network (RNN) to capture the sequential information of trajectories for detection. However, the proposed model needs to be trained in a supervised manner, and the labeled data is usually unavailable in real applications.
%
Another learning-based work~\cite{gray2018coupled} aims at detecting anomalous trajectories by new moving subjects (i.e., new taxi driver detection) with an adversarial model (i.e., GAN) is adapted.
%
It is clear that the methods proposed in this line of research cannot be adopted for the online detection scenario. Again, we target the detection in a finer-grained setting, i.e., subtrajectory anomaly detection via reinforcement learning.

\subsection{Other Orthogonal Work}
Some works~\cite{banerjee2016mantra, li2009temporal, ge2010top, yu2014detecting} focus on other types of anomalous trajectory detection, which are orthogonal to ours. We review them as follows. Banerjee et al.~\cite{banerjee2016mantra} study temporal anomaly detection, it employs travel time estimation and traverses some potential subtrajectories in a detected trajectory, where the anomalies are identified if the travel time largely deviates from the expected time. Li et al.~\cite{li2009temporal} detect temporal outliers and a method using historical similarity trends is studied. In addition, Ge et al.~\cite{ge2010top} study the Top-K evolving outliers and Yu et al.~\cite{yu2014detecting} detect anomalous trajectories in large-scale trajectory streams.

\subsection{Deep Reinforcement Learning}
Deep reinforcement learning aims to guide an agent on how to make sequential decisions to maximize a cumulative reward~\cite{sutton2018reinforcement}, where the agent interacts with a specific environment, which is usually modeled as a Markov decision process (MDP)~\cite{puterman2014markov}. In recent years, reinforcement learning has received much research attention. For example, Oh et al.~\cite{oh2019sequential} explore
inverse reinforcement learning for sequential anomaly detection, and Huang et al.~\cite{huang2018towards} design a deep RL powered anomaly detector for time series detection. Wang et al.~\cite{wang2020efficient} propose to use RL-based algorithms to accelerate subtrajectory similarity search. In this paper, we model a novel road network-enhanced MDP for online anomalous subtrajectory detection (called RL4OASD), and a policy gradient method~\cite{sutton2000policy} is involved for solving the problem. To our best knowledge, this is the first deep reinforcement learning based solution of its kind.


\noindent\textbf{22 Nov-Cheng: Comments on the related work. 1. In Section 2.2, [1] is mentioned but not described; 2. Better to use the word "related" to replace "orthogonal".}

==> related3.tex <==
\section{RELATED WORK}
\label{sec:related}
% then you proceed to rewrite "related" work, whenever possible, refer to the issues you talk about (e.g. 
% 1. either they are offline cannot be used for online detection, 
% 2. don't give subtrajectories, require labelled data, 
% 3. modelling of subtrajectories is not good, 
% 4. or work on some other problems, not exactly ours), got it?
We review the related studies which can be categoried into four groups. The first group is online anomalous trajectory detection, the second group is offline anomalous trajectory detection, the third group is other types of anomalous trajectory detection, such as temporal anomalous trajectory detection, and the last group is about deep reinforcement learning, which is utilized in this paper. 

\subsection{Online Anomalous Trajectory Detection}
Online anomalous trajectory detection aims to detect the ongoing trajectory in online manner. Existing studies propose many methods for online anomalous trajectory detection and involve two categories: heuristic-based methods~\cite{ge2010top,yu2014detecting,chen2013iboat,zhang2020continuous} and learning-based methods~\cite{wu2017fast,liu2020online}. 


For heuristic methods, ~\citet{chen2013iboat} investigates the detecting anomalous trajectories in online manner via 
the isolation-based method, which aims to check which parts of trajectories are isolated from the reference (i.e., normal) trajectories with the same source and destination routes. {\Comment{This method aims to detect the anomalous subtrajectories via ongoing trajectories, which is similar to our paper. However, this method models reference trajectories based on many parameters. Besides, the performance of this method is evaluated on a small manually labelled dataset with 9 SD pair only, which fail to reflect the generalization of this method.}}
% Chen et al.~\cite{chen2013iboat} study the online anomalous trajectory detection with the isolation-based method, which aims to check which parts of a detected trajectory that can be isolated from the reference (i.e., normal) trajectories with the same source and destination routes.
%
A recent work ~\cite{zhang2020continuous} propose to calculate the trajectory similarity via discrete Frechet distance between a given reference route and the current partial route at each timestamp. If the deviation threshold exceeds a given threshold at any timestamp, and the system alerts that an outlier event of detouring is detected. {\Comment{There are many predefined parameters involved in this method. Besides, the method of modelling a reference route is not given, which has a direct impact on the task. Our work differs from these heuristic-based studies in that it is based on a road network-enhanced policy learned via reinforcement learning instead of the hand-crafted heuristic with many predefined parameters (e.g., the deviation threshold) for detecting anomalies. Besides, we evaluate the performance of our method on \textbf{a large dataset.}}}


For learning-based methods, a recent study~\citet{liu2020online} proposes to detect anomalous trajectories via a generation scheme, it utilizes the Gaussian mixture distribution to represent different kinds of normal routes and detect those anomalous trajectories that cannot be well-generated based on the given representations of normal routes. {\Comment{This method aims to detect whether the ongoing trajectory is anomalous or not.}} Another learning-based method ~\cite{wu2017fast} proposes a probabilistic model to detect trajectory outliers via modeling the distribution of driving behaviours from historical trajectories. The method involves many potential features that are associated with driving behaviour modeling, including road level and turning angle, etc. {\Comment{ This method also only targets whether the online trajectory is anomalous or not}}. In our work, we target a more finer-grained setting, i.e, detecting which part of an anomalous trajectory, namely subtrajectory, is responsible for its anomalousness in an online manner. Nevertheless, subtrajectory detection is not the focus in these studies.
 


\subsection{Offline Anomalous Trajectory Detection}
Offline anomalous trajectory detection refers to detecting the target trajectory which is complete in offline manner. Also there are two types of studies. One type is heuristic-based methods~\cite{lee2008trajectory, zhang2011ibat,zhu2015time,lv2017outlier,banerjee2016mantra} and another type is learning-based methods~\cite{gray2018coupled,song2018anomalous} as follows.


For heuristic-based methods, some heuristic metrics involving distance or density metrics are usually utilized to detect anomalous trajectories. For example, an early study ~\cite{lee2008trajectory} proposes a partition and detect mechanism to conduct anomalous trajectory detection. The main idea is to partition the trajectories and detect the anomalous trajectory segments by computing the distance of each segment in a detected trajectory to the segments in other trajectories. Further, ~\citet{zhu2015time} and ~\citet{lv2017outlier} utilize edit distance metrics to detect anomalous trajectory based on mining the normal trajectory patterns. Another study~\cite{zhang2011ibat} proposes to cluster trajectories based on the same itinerary and further detect anomalous trajectories via checking whether the target trajectory is the isolated from the the cluster. In addition, ~\cite{ge2011taxi} proposes a system which is utilized to detect fraud taxi driving. The main idea of this method is to detect anomalous trajectories via combining distance and density metrics. 

% some distance or density metrics are usually proposed for detecting anomalies. For example, an early study~\cite{lee2008trajectory} proposes to partition the trajectories and detect the anomalous trajectory segments by computing the distance of each segment in a detected trajectory to the segments in other trajectories.
% Further, Zhu et al.~\cite{zhu2015time} and Lv et al.~\cite{lv2017outlier} adopt the edit distance based metrics to detect anomalies via mining normal trajectory patterns. Another study~\cite{zhang2011ibat} proposes to cluster the trajectories crossing the same itinerary and detect anomalous trajectories via checking the isolation from the cluster. In addition, Ge et al~\cite{ge2011taxi} develop a taxi driving fraud system, which is equipped with both distance and density metrics to identify fraud driving activities. 

Other studies are proposed to detect anomalous trajectories with learning-based methods. Song et al~\cite{song2018anomalous} adopt recurrent neural network (RNN) to capture the sequential information of trajectories for detection. However, the proposed model needs to be trained in a supervised manner, and the labeled data is usually unavailable in real applications.
%
Another learning-based work~\cite{gray2018coupled} aims at detecting anomalous trajectories by new moving subjects (i.e., new taxi driver detection) with an adversarial model (i.e., GAN) is adapted.
%
{\Comment{It is clear that these methods proposed in this line of research can not be utilized for the online detection scenario. Again, we target the online anomalous subtrajectory detection in a finer-grained setting, i.e., subtrajectory anomaly detection via reinforcement learning.}}


\subsection{{\Comment{Other Types of Anomalous Detection Studies}}}
Some works~\cite{banerjee2016mantra, li2009temporal, ge2010top, yu2014detecting} focus on other types of anomalous trajectory detection, which are related to ours. We review them as follows. Banerjee et al.~\cite{banerjee2016mantra} study temporal anomaly detection, which employs travel time estimation and traverses some potential subtrajectories in a detected trajectory, where the anomalies are identified if the travel time largely deviates from the expected time. ~\citet{li2009temporal} detect temporal outliers and a method utilizing historical similarity trends is studied. In addition, ~\citet{ge2010top} investigates the Top-K evolving outliers and ~\citet{yu2014detecting} detects anomalous trajectories in large-scale trajectory streams.



\subsection{Deep Reinforcement Learning}
Deep reinforcement learning aims to guide an agent to make sequential decisions to maximize a cumulative reward~\cite{sutton2018reinforcement}, as the agent interacts with a specific environment, which is usually modeled as a Markov decision process (MDP)~\cite{puterman2014markov}. In recent years, reinforcement learning has attracted much research attention. For example, ~\citet{oh2019sequential} explores inverse reinforcement learning for sequential anomaly detection, and ~\citet{huang2018towards} designs a deep RL based anomaly detector for time series detection. ~\citet{wang2020efficient} proposes to use RL-based algorithms to accelerate subtrajectory similarity search. {\Comment{In this paper, we model a novel road network-enhanced MDP for online anomalous subtrajectory detection (called RL4OASD), and a policy gradient method~\cite{sutton2000policy} is adopted for solving the problem. To our best knowledge, this is the first deep reinforcement learning based solution for online anomalous subtrajectories detection.}}
% its kind
% online anomalous subtrajectories detection











==> response.tex <==

\newpage

\noindent
{\large
\textbf{Response to Review Report of Paper Titled ``Online Anomalous Subtrajectory Detection on Road Networks with Deep Reinforcement Learning'' (ICDE 2023 Paper ID = 95)}}
%\label{sec:response}

\smallskip\noindent Dear ICDE Meta-reviewer and Reviewers,

\smallskip
First, we would like to thank you for your constructive and inspiring comments. We have gone through these comments carefully and revised our draft accordingly. Below we summarize the major changes.

\begin{enumerate}
  \item We have included a new evaluation metric to show the genericity of our method (Table~\ref{tab:baselines} in Section~\ref{sec:experiment}).
  \item We have reported the computational cost of data preprocessing, including the phases of map-matching and noisy labeling (Table~\ref{tab:train_time} in Section~\ref{sec:experiment}).
  \item We have {\CHENG conducted experiments for cases where} the historical trajectories are not sufficient (i.e., it corresponds to a cold-start problem) {\CHENG and show the results} (Table~\ref{tab:droprate} in Section~\ref{sec:experiment}).
  \item We have discussed and evaluated the selection of a proper length of time period for online learning (Figure~\ref{fig:traffic} in Section~\ref{sec:experiment}).
  \item We have added more clarifications and explanations for both methodology and experiments as requested by reviewers.
  \item We have put some experimental results {\CHENG (namely some parameter study results and case study results)} in the technical report~\cite{TR}.
\end{enumerate}
%}

% These major changes are highlighted in blue in the revised paper.
% Appended please find our detailed responses to both the reviewers' and meta-reviewer's comments.
% Thank you for your time reading them.

We highlight the major changes with the blue color in the revised manuscript. Appended please find our detailed responses to both the reviewers' and meta-reviewer's comments. We really appreciate your feedback and time.

\smallskip\noindent Yours sincerely, \\
Qianru, Zheng, Cheng, Chao, Siu-Ming, Yiding, Gao and Jieming

%----------------
%\newpage
\section{Response to Reviewer 1's Comments}
\label{subsec:reviewerOneReport}

% \begin{comment1}\em
% ``O1. Although the idea of utilizing reinforcement learning for online sub-trajectory anomalous detection is interesting, the technical novelty is unclear. Many methods used in the paper can be seen in previous studies. The proposed framework mainly features two modules: RSRNet and ASDNet. However, the former is based on the widely used LSTM model and another existing Toast model; the latter is leveraging the process of MDP for the model training. Such a direct combination or a simple extension of learning techniques with trajectory mining tasks makes it hard to determine the technical novelty.''
% \end{comment1}

\begin{comment1}\em
``O1. Further clarification of the model technical novelty.''
%motivations for model design
\end{comment1}

\noindent\textbf{Response.} Thanks for this valuable comment. We highlight the technical novelty of this work from two aspects.
%
\underline{First}, we are among the pioneering work to develop a deep reinforcement learning based model that enables online anomalous subtrajectory detection. Our proposed model 1) is capable of automatically identifying anomalous subtrajectories without the large efforts on generating hand-crafted features and pre-defined rubrics; 2) does not largely rely on the limited labeled data and can effectively discover the abnormal trajectory patterns under data scarcity. This marks a significant improvement in the methodology to overcome {\CHENG those issues suffered by existing methods (as summarized in Table~\ref{tab:summary})}.
% 1) is capable of detecting anomalous subtrajectories, 2) is data-driven without hand-crafted features and/or pre-defined rubrics for the detection, and 3) does not largely rely on the limited labeled data. This marks a significant improvement in the methodology to overcome {\CHENG those issues suffered by existing methods (as summarized in Table~\ref{tab:summary})}.

% these challenges, especially given that detecting anomalous trajectories is an important problem, for which a rich set of techniques have been developed but very few works can address all challenges as summarized in Table~\ref{tab:summary}.
%
% \underline{Second}, our model is a weakly supervised learning paradigm, where the proposed RSRNet learns better road segment observations to define the states of MDP in ASDNet, and ASDNet provides refined labels of road segments to train RSRNet. They {\CHENG iteratively improve} each other, and run in a positive loop to produce superior results. To our best knowledge, the weakly supervised paradigm is the first of its kind.

\underline{Second}, our model is a weakly supervised learning paradigm, where the proposed RSRNet learns accurate road segment observations to define the states of MDP in ASDNet. ASDNet provides refined labels of road segments to train RSRNet. They {\CHENG iteratively improve} each other, and run in a positive loop to produce superior results. To our best knowledge, the weakly supervised paradigm is the first of its kind.
%
% \underline{Third}, we study the concept drift of anomalous trajectories, our model can handle the issue via online learning, which makes our technique more complete to meet practical needs for varying traffic conditions, and we perform extensive experiments to verify the results, while very few of existing techniques can achieve this.
%
% In summary, our novelty lies in providing an all-around solution that can tackle the challenges of the problem. 
%\underline{Third}, our method \texttt{RL4OASD} solves three challenges effectively, namely the difficulty of detecting anomalous subtrajectories, non-data driven and lacking of sufficient supervision labels. \texttt{RL4OASD} consists of three components, including data preprocessing, RSRNet and ASDNet. RSRNet provides better observations for ASDNet via noise labels, which solves the second and third challenges. ASDNet outputs refined labels that are further used to train RSRNet again, which solves the first, second and third challenges. 

% The techniques are not straightforward as they look in the paper, which require many rounds of efforts for analyzing, adjusting, and testing many possibilities of designing different components.
% the MDP (including states, actions, transitions and rewards) 
With the effective model design, we can achieve better detection performance and competitive efficiency (especially for the online detection task which requires real-time response). %We tried to provide intuitions and discussions for our design as much as possible, but they reflect only a fraction of our efforts devoted to the design task.

% \begin{comment1}\em
% ``O2. The presentation can be improved. In Section IV-C (Normal Route Feature), it is better to clarify how to calculate the fraction of $T_1$ and $T_2$. The noisy labels keep being updated, which is also unclear.''
% \end{comment1}

\begin{comment1}\em
``O2. Clarifications of i) the calculation for $T_1$ and $T_2$; ii) the process of updating noisy labels.''
\end{comment1}

\noindent\textbf{Response.} Thanks for the detailed comment. We have revised the presentation to make it clear. 
The changes are highlighted in blue {\ICDERevision{in Section~\ref{sec:RSRNet}}}. {\CHENG 1) We clarify the fraction calculations. Consider an example where there are 5 trajectories traveling along $T_1$, 4 along $T_2$, and only 1 along $T_3$. Then the fractions of $T_1$ and $T_2$ are calculated as $5/10=0.5$ and $4/10=0.4$, respectively. 2) We clarify that the noisy labels are only utilized to pre-train the representations in RSRNet, which would then provide a warm-start for ASDNet, and the noisy labels are not being updated.}

% \begin{comment1}\em
% ``O3. The experiments are not sufficient. 1) There is only a single evaluation metric, which cannot show the genericity of the methods. 2) It is unfair to adopt the inference time as the efficiency performance metric, compared with non-learning methods, as the learning-based models also rely on the training process. 3) It would be better top report the preprocessing cost is also not reported.''
% \end{comment1} 

\begin{comment1}\em
``i) O3. Performance evaluation with more metrics. ii) Model efficiency study with the preprocessing cost.''
\end{comment1} 

\noindent\textbf{Response.} Thanks for the comment. 1) We have included a variant of $F_1$-score, {\CHENG called $TF_1$-score, as a new metric. The intuition of $TF_1$-score is to count only those detected anomalous subtrajectories which are aligned with real anomalous subtrajectories sufficiently.}
% via a threshold, to control the quality of the recognized anomalous subtrajectories, . 
% Specifically, based on Equation~\ref{eq:jac}, we involve a threshold $\phi$. If the Jaccard similarity $\mathcal{J}_i(C_{g,i},C_{o,i})$ is above the $\phi$, it is set to 1, and 0 otherwise, then we compute the $F_1$-score by Equation~\ref{eq:f1}. 
The detailed definition is described {\ICDERevision{in Section~\ref{sec:setup}}} and the corresponding results are included {\ICDERevision{in Table~\ref{tab:baselines}}}. 
% Based on the results, it still performs similar trends as $F_1$-score, 
{\CHENG The results based on $TF_1$-score and those based on $F_1$-score show similar trends,}
which shows the genericity of our methods. 
2) The inference time is widely adopted by existing learning-based methods including~\cite{wu2017fast,liu2020online,song2018anomalous,li2007roam} for efficiency evaluation. Normally, the training cost is an one-time cost, i.e., once a policy is learned, we can use it for detecting many trajectories online. In this revised paper, we have included some experimental results of the training time and the effects of the size of the training dataset on the performance of RL4OASD in Table~\ref{tab:train_time}. In general, it takes only around 0.2 hours to learn a satisfactory model. 
3) In the revised paper, we have reported the preprocessing cost involving map-matching and noisy labeling {\ICDERevision{in Table~\ref{tab:train_time}}}. Overall, it takes less than two minutes to preprocess the dataset, which again is an one-time process.

\section{Response to Reviewer 2's Comments}
\label{subsec:reviewerTwoReport}

% \begin{comment2}\em
% ``O1. Cold-start problem is not studied or discussed. As the anomalous subtrajectories are defined as unpopular parts, then how to detect when the historical trajectories are not sufficient or even not exist at the beginning, which should be discussed and tested in experiments.''
% \end{comment2}

\begin{comment2}\em
``O1. Discussion about the cold-start settings of anomalous subtrajectory detection.''
\end{comment2}

\noindent\textbf{Response.} Thank you for the insightful comment. Our method relies on the historical trajectories for defining the normal route feature. The feature is calculated as a relative fraction between 0 and 1. Specifically, the feature of a route is defined to be the number of trajectories along the route over the total number of trajectories within the SD pair.
% is not affected by the data sparsity much. For example, 
{\CHENG We have conducted experiments} by varying the number of historical trajectories within the SD pairs {\ICDERevision{in Table~\ref{tab:droprate}}}. {\CHENG The results show that our model is robust against sparse data, e.g., its effectiveness} only degrades by 6\% even if 80\% of historical trajectories are dropped. The cold-start problem in anomalous trajectory/subtrajectory detection looks very interesting. We believe that some generative methods, e.g., to generate some routes within the sparse SD pairs, can possibly be leveraged to overcome the issue, which we plan to explore as future work.

% \begin{comment2}\em
% ``O2. Using online learning strategy to capture the varying traffic condition is a practical method, but the details seem not well studied. How to select a proper length of time period to start a new training on that part of data is also very important. Currently, the authors only simply divide one day into 4 parts, which is lack of discussion.''
% \end{comment2}

\begin{comment2}\em
``O2. Clarifications of selecting the proper length of time period for new training parts.''
\end{comment2}

\noindent\textbf{Response.} Thank you for the comment. In the revised paper, we have studied the effect of the length of time period for the training and provided the detailed discussion {\ICDERevision{in Section~\ref{sec:concept_exp}}}. Specifically, we follow the setup in~\cite{liu2020online}, and first study how to select a proper length of time period to start the training with a parameter $\xi$. For example, when $\xi$ is set to 4, it partitions one day into 4 parts, and the proposed online learning model \texttt{RL4OASD-FT} is first trained on Part 1, and kept updating on the other parts of data. 
% To set , we 
We vary $\xi$ from 1 to 24, and report the average $F_1$-score over all parts and the corresponding training time {\ICDERevision{in Figure~\ref{fig:traffic}(a) and (b)}}, respectively. Based on the results, we observe that when $\xi$ is set to 8 (i.e., training the model every $24/8=3$ hours), it leads to the best effectiveness with $F_1$-score=0.867, and the average training time less than 0.04 hours, which is much smaller than the duration of a time period (i.e., 3 hours). Under the setting of $\xi=8$, we further report the $F_1$-score and training time for each part {\ICDERevision{in Figure~\ref{fig:traffic}(c) and (d)}}, respectively. We note that our online learning strategy can tackle the issue of concept drift in varying traffic conditions.

% \begin{comment2}\em
% ``O3. The design of framework and models lack of insights and explanation. The paper mainly introduces how to build the RL4OASD and the small components of it. Using learning models to solve the problem also needs to provide the overall insights of the effectiveness of the model. I suggest to provide some explanation in Section IV-A.''
% \end{comment2}

\begin{comment2}\em
``O3. Further explanations of the effectiveness of individual components in the proposed RL4OASD model.''
\end{comment2}

\noindent\textbf{Response.} Thank you for the comment. In the revised paper, we have included {\CHENG some explanations on the effectiveness of our method.}
% the overall insights and explanations. 
Please refer to the texts highlighted in blue {\ICDERevision{in Section~\ref{sec:overview_rl4oasd}}}. 
{\CHENG We copy the explanations below for the ease of reference.} First, in RSRNet, 
%we  carefully define the state such that 
both traffic context features (e.g., driving speed, trip duration) and normal route features that are associated with the anomalies are well captured into the model. Second, in ASDNet, the task of labeling anomalous subtrajectories is formulated as a MDP, whose policy is learned in a data-driven manner, instead of using heuristics (e.g., some pre-defined parameters) as the existing studies do.
% , those are hard to cover all possible situations. 
%
Third, 
% we design a weakly supervised framework to deploy the model, where 
RSRNet is first trained with noisy labels for dealing with the cold-start problem.
Then, RSRNet and ASDNet are trained iteratively and collaboratively, where RSRNet uses ASDNet's outputs as labels and ASDNet uses the outputs of RSRNet as features.
% Specifically, the effectiveness of the model is mainly in three aspects. First, in RSRNet, we carefully define the state such that both traffic context features (e.g., driving speed, trip duration) and normal route features that are associated with the anomalies are well captured into the model.
% %
% Second, in ASDNet, the task of labeling anomalous subtrajectories is formulated as a MDP, whose policy is learned in a data-driven manner, instead of using heuristics (e.g., some pre-defined parameters) as the existing studies, those are hard to cover all possible situations.
% %
% Third, we design a weakly supervised framework to deploy the model, where RSRNet and ASDNet can mutually refine each other, and run in a positive loop to produce better results.
%

\section{Response to Reviewer 3's Comments}
\label{subsec:reviewerThreeReport}

% \begin{comment3}\em
% ``O1. While I found the OASD problem interesting, I am confused with the problem formalization, especially the criteria about "anomalous road segments".
% - O1.1. Can I understand that a subtrajectory is anomalous if the subtrajectory is a detour?
% - O1.2. It seems that the paper uses the "transition frequency" as the supervision signal. This may not be reasonable, as some infrequent segments in a subtrajectory may not indicate the subtrajectory is a detour or being anomalous.''
% \end{comment3}

\begin{comment3}\em
O1. Further description of the problem formalization and the criteria for anomalous road segments.
\end{comment3}

\noindent\textbf{Response.} Thanks for the comment. 1) {\CHENG Yes, a detour would be probably labeled to be anomalous since it deviates from others within the same SD pair}. 2) First, we emphasize that the transition frequency is only used to construct the noisy labels, which are further used to pre-train the model as a warm-start, but are not used to train the model as the supervision signal during the joint training of RSRNet and ADSNet. In addition, based on the ablation study in Table~\ref{tab:ablation}, 
% we observe that the transition frequency incorporates some information captured from the normal routes in general, e.g., 
{\CHENG with the transition frequency used, it improves the overall effectiveness by around 36\%.}
% , which provides a necessary warm-start for improving the performance of around 36\%.

% \begin{comment3}\em
% ``O2. The RL4OASD approach seems solid. However, it would be better if the authors discuss more on the generalizability of the approach. For example, why does the learned policy can make good decisions on the trajectories, which are not seen during the training phase.''
% \end{comment3}

\begin{comment3}\em
``O2. The discussion on the generalizability of the approach.''
\end{comment3}

\noindent\textbf{Response.} Thanks for the comment. We discuss the generalizability of the approach in two aspects. {\underline{First}}, our {\texttt{RL4OASD}} is a data-driven approach, where we capture two types of features, namely the representations of road segments based on traffic context (e.g., driving speed) and the information captured from the normal routes. These two types of features can be generalized to other trajectories, and captured by the model trained in a data-driven manner. 
% Compared with the existing methods that are not data driven~\cite{chen2013iboat, zhang2020continuous}, they rely on some manually defined parameters and/or rules for the detection as discussed in Section~\ref{sec:introduction}. However, the parameters are hard to set appropriately, and not general enough to cover all possible situations (e.g., for some trajectories that are not seen). 
{\underline{Second}}, our model can be deployed with an online learning strategy, where the model continues to be refined with newly recorded trajectory data.
% , and thus keeps its policy updated for those unseen trajectories. 
The effects of online learning are shown in Figure~\ref{fig:traffic}. 

% \begin{comment3}\em
% ``O3. The authors invite 5 participants to label anomalous subtrajectories. During this process, it is not clear how to instruct the participants about the criteria about what is "anomalous". Thus, it would be good if the authors provide the detailed instruction to the participants.''
% \end{comment3}

\begin{comment3}\em
``O3. The description of the criteria details for labeling anomalous subtrajectories by participants.''
\end{comment3}

\noindent\textbf{Response.} Thanks for the comment. We have provided the detailed instruction to the participants, and please refer to the text highlighted in blue {\ICDERevision{in Section~\ref{sec:setup}}}.

% \begin{comment3}\em
% ``O4. The arrows in Fig. 2 are sometimes confusing. For example, arrows from $x_i$ to $h_i$ indicate connections with weights, while arrows from $x_i^{n}$ do not have the same meaning as indicated in Section IV-C. Moreover, it is unclear about how to get $\hat{y}_{i}$ from $z_i$.
% ''
% \end{comment3}

\begin{comment3}\em
``O4. The clarification of the  arrows in Fig. 2 and the derivation process of $\hat{y}_{i}$ based on $z_i$.''
\end{comment3}

\noindent\textbf{Response.} Thank you for the comment. {\CHENG We have revised {\ICDERevision{Figure~\ref{fig:rl4oasd}}} in the revised paper. To be specific, we use different arrows with annotations to distinguish the operations represented by the arrows. In addition, $\hat{y}_{i}$ is computed from $z_i$ via Softmax.} 
% We have annotated the arrows used in in the figure.

% \begin{comment3}\em
% ``O5. More justifications are needed for the evaluation metrics. Take recall as an example and consider two outputs $C_{o_1}$ and $C_{o_2}$. Suppose that $C_{o_1}$ matches 5 trajectories in $C_{g}$ where each has a Jaccard similarity 0.2. Also, suppose that $C_{o_2}$ only matches 1 trajectory in $C_{g}$ with a Jaccard similarity 1. In this case, we can see that these two outputs have the same recall, which is counter-intuitive.''
% \end{comment3}

\begin{comment3}\em
``O5. Further justifications of the evaluation metrics.''
\end{comment3}

\noindent\textbf{Response.} 
% Please refer to our response to Reviewer 1's Comment 3. 
In the revised paper, we have included a new metric called $TF_1$-score, {\CHENG which counts only those Jaccard similarities above a threshold $\phi$}. 
% For example, when $\phi$ is set to 0.5, the 5 subtrajecories with Jaccard similarities 0.2 will be set to 0, and the 1 subtrajecory with a Jaccard similarity 1 is still set to 1. Then, these two outputs are with different recall, which is in line with our intuition (e.g., $C_{o_2}$ should be better). 
We have included the new results based on this additional new metric $TF_1$-score {\ICDERevision{in Table~\ref{tab:baselines}}}, which show that our solution outperforms the existing baselines under this new metric.
% in similar trends as $F_1$-score.

\section{Response to Meta-Reviewer's Report}

We have addressed all revision items, and our responses to required changes
\begin{itemize}
    \item \textbf{Reviewer 1: O1, O2, O3}, can be found in our responses to  
    Reviewer 1's Comment 1, 2 and 3, respectively.
    \item \textbf{Reviewer 2: O1, O2}, can be found in our responses to Reviewer 2's Comment 1 and 2, respectively.
    \item \textbf{Reviewer 3: O1, O2, O5}, can be found in our responses to Reviewer 3's Comment 1, 2 and 5, respectively. 
\end{itemize}
and optional changes
\begin{itemize}
    \item \textbf{Reviewer 2: O3}, can be found in our responses to Reviewer 2's Comment 3.
    \item \textbf{Reviewer 3: O3, O4}, can be found in our responses to Reviewer 3's Comment 3 and 4, respectively.
\end{itemize}



